Multidimensional coupling: A variationally consistent approach to fiber-reinforced materials

A novel mathematical model for fiber-reinforced materials is proposed. It is based on a 1-dimensional beam model for the thin fiber structures, a flexible and general 3-dimensional elasticity model for the matrix and an overlapping domain decomposition approach. From a computational point of view, this is motivated by the fact that matrix and fibers can easily meshed independently. Our main interest is in fiber reinforce polymers where the Young's modulus are quite different. Thus the modeling error from the overlapping approach is of no significance. The coupling conditions acknowledge both, the forces and the moments of the beam model and transfer them to the background material. A suitable static condensation procedure is applied to remove the beam balance equations. The condensed system then forms our starting point for a numerical approximation in terms of isogeometric analysis. The choice of our discrete basis functions of higher regularity is motivated by the fact, that as a result of the static condensation, we obtain second gradient terms in fiber direction. Eventually, a series of benchmark tests demonstrate the flexibility and robustness of the proposed methodology. As a proof-of-concept, we show that our new model is able to capture bending, torsion and shear dominated situations.

==> preamble.tex <==
% !TeX root = MAIN.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{amsfonts,amsmath,amsthm,amssymb}
\usepackage{mathtools}
\usepackage{hyperref}
\usepackage{autonum}
%\usepackage[normalem]{ulem}
%\usepackage{ulem}
\usepackage{hhline}
\usepackage{array}
%\usepackage{gensymb}
\usepackage{diagbox}
\usepackage{tcolorbox}
\usepackage{mdframed}
\usepackage{multicol}
\usepackage{subcaption}
%\usepackage[labelfont=bf,font=sf]{caption}
\usepackage{moreverb}
\usepackage{bbm}
\usepackage{placeins}
\usepackage{enumerate}


%\usepackage{todonotes}
\allowdisplaybreaks
%\usepackage[breaklinks=true]{hyperref}
%\usepackage{breakcites}


% --- biblio ----

%\usepackage[doi=false,isbn=false,url=false]{natbib}
%\usepackage{natbib}
%%	\bibliographystyle{ieeetr}
%\bibliographystyle{abbrvnat}	
%\setcitestyle{authoryear, square}
%\renewcommand{\cite}[1]{((\citet{#1}))}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TIKZ
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{tikz}
\usetikzlibrary{decorations.pathmorphing} % for snake lines
\usetikzlibrary{matrix} % for block alignment
\usetikzlibrary{arrows} % for arrow heads
\usetikzlibrary{calc} % for manimulation of coordinates
\usetikzlibrary{shapes}
\usetikzlibrary{shapes.geometric}

% TikZ styles for drawing
\tikzstyle{block} = [draw,rectangle,thick,minimum height=2em,minimum width=2em]
\tikzstyle{sum} = [draw,circle,inner sep=0mm,minimum size=2mm]
\tikzstyle{connector} = [->,thick]
\tikzstyle{line} = [thick]
\tikzstyle{branch} = [circle,inner sep=0pt,minimum size=1mm,fill=black,draw=black]
\tikzstyle{guide} = []
\tikzstyle{snakeline} = [connector, decorate, decoration={pre length=0.2cm,
	post length=0.2cm, snake, amplitude=.4mm,
	segment length=2mm},thick, magenta, ->]

\usepackage{pgfplots}
%%\usepackage{pgffor}
%\usepackage{pgfplotstable}
%\usepgfplotslibrary{colorbrewer}
%\usepgfplotslibrary{groupplots}
%%\pgfplotsset{compat=1.15}
%\pgfplotsset{compat=newest}
%\usepackage{tikz}
%\usetikzlibrary{external}
%\tikzexternalize[prefix=tikz/]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Notations 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% math
\newcommand{\X}{\vec{X}}
\newcommand{\x}{\vec{x}}
\newcommand{\y}{\vec{y}}
\newcommand{\z}{\vec{z}}
\newcommand{\Id}{\operatorname*{Id}}
\newcommand{\sign}{\operatorname*{sign}}
\newcommand{\op}[1]{\operatorname*{#1}}
\newcommand{\eps}{\varepsilon}
\newcommand{\J}{\mathcal{J}}
\newcommand{\dev}[1]{\text{dev}\left[#1\right]}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\dt}{\Delta t}
\newcommand{\dx}{\Delta x}
\newcommand{\sgn}[1]{\ \text{sgn}\left(#1\right) }
\newcommand{\sca}[2]{\langle #1, \; #2 \rangle}
\newcommand{\frc}[2]{{\textstyle\frac{#1}{#2}}}
\newcommand{\minus}{\scalebox{0.7}[1.0]{\( - \)}}
\newcommand{\inv}{^{\scalebox{0.7}[1.0]{\( - \)}1}}%{^{-1}}
\newcommand{\tp}{^\intercal}
\newcommand{\tpc}{^*}
\renewcommand{\exp}[1]{e^{#1}}
\newcommand{\Exp}[1]{\operatorname*{Exp}\left(#1\right)}
\renewcommand{\i}{\mathrm{i}}
\renewcommand{\d}{\operatorname{d}\!}
\newcommand{\tr}{\operatorname{tr}}
\renewcommand{\Re}{\mathfrak{Re}}
\renewcommand{\Im}{\mathfrak{Im}}
\newcommand{\B}{\lbrace -1, 1\rbrace}
\newcommand{\Ind}{\mathbbm{1}}
\renewcommand{\O}{\mathcal{O}}

% vectors and matrices
\newcommand{\mat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\diag}{\operatorname{diag}}
\renewcommand{\vec}[1]{\pmb{#1}}
\newcommand{\vct}[1]{\vec{#1}}
\newcommand{\ten}[1]{\pmb{#1}}
\newcommand{\tns}[1]{\ten{#1}}
\newcommand{\tnsfour}[1]{\pmb{#1}}

% parantheses
\newcommand{\bbc}[1]{\left( #1 \right)}
\newcommand{\rbc}[1]{\left[ #1 \right]}

% differentiation
\newcommand{\drv}[2]{\frac{\partial #1}{\partial #2}} %{\partial_{#1} #2}
\newcommand{\D}[2]{\partial_{#1} #2}
\renewcommand{\div}{\nabla\cdot}
\newcommand{\grad}{\nabla}
\newcommand{\gradS}{\nabla\!_s}
\newcommand{\Jac}[2][]{ \operatorname*{D_{#1}}\! #2  }
\newcommand{\Hess}[1]{ D^2#1  }


% integral transforms
\newcommand{\La}[1]{\mathfrak{L}\lbrace #1 \rbrace }
\newcommand{\Lai}[1]{\mathfrak{L}\inv\lbrace #1 \rbrace }
\newcommand{\F}{\mathcal{F}} % Fourrier transform
\newcommand{\Fi}{\mathcal{F}^{-1}} % inverse Fourrier transform
\newcommand{\FFT}[1]{\operatorname{FFT}\left\lbrace #1 \right\rbrace} % Discrete (Fast) Fourrier Transform
\newcommand{\IFFT}[1]{\operatorname{IFFT}\left\lbrace #1 \right\rbrace} % inverse Discrete (Fast) Fourrier Transform

% Sets
\newcommand{\Z}{\mathbb{Z}} % integer
\newcommand{\R}{\mathbb{R}} % real
\newcommand{\C}{\mathbb{C}} % complex
\newcommand{\N}{\mathbb{N}} % natural

% Matrix groups
\newcommand{\SymM}[1][3]{\op{S}^{#1}} % Symmetric matrices
\newcommand{\PSD}[1][3]{\SymM[#1]_+} % Symmetric positive semi-definite matrices
\newcommand{\PD}[1][3]{\SymM[#1]_{++}}  % Symmetric positive definite matrices
\newcommand{\SO}[1]{\operatorname{SO}_{#1}}  % Symmetric positive definite matrices

% Spaces
\newcommand{\HS}{\mathcal{H}} % Hilbert space
\newcommand{\K}{\mathcal{K}} % Krylov subspace
\renewcommand{\L}[1]{\op{L}^{\!#1}} % Lesbegues space
\newcommand{\W}[2]{\op{W}^{#1,#2}} % Sobolev space
\renewcommand{\H}[1]{\op{H}^{#1}} % Sobolev space
\newcommand{\Cn}[1]{\op{C}^{#1}} % Sobolev space
%\newcommand{\M}{\mathbb{M}} % Space of matrices
\newcommand{\vspan}{\op{span}} % convex hull (span)

% Probability
\newcommand{\E}[1]{\operatorname{\mathbb{E}}\rbc{#1}}
\newcommand{\Prob}[1]{\operatorname{\mathbb{P}}\rbc{#1}}
\newcommand{\Var}[1]{\operatorname{Var}\rbc{#1}}
\newcommand{\Gaussian}{\mathcal{N}}
\newcommand{\Cov}{\tns{C}}
\newcommand{\WN}{\mathcal{W}} % White noise
\newcommand{\WNhat}{\hat{\mathcal{W}}} % Fourier of White noise


% Special functions
\newcommand{\BesselJ}[1]{\mathcal{J}_{#1}}
\newcommand{\BesselK}[1]{\mathcal{K}_{#1}}
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\erfc}{\operatorname{erfc}}
\newcommand{\hypTwoOne}{{\;}_{2}F_{1}}


% raccourcis
\newcommand{\MatLab}{MatLab R2016b}

% formating
\newcounter{rownumber}
\newcommand{\rownumber}{\stepcounter{rownumber}\therownumber}


% Elasticity problem
\newcommand{\dir}{\vec{e}}
\newcommand{\disp}{\vec{u}}
\newcommand{\strain}{\tns{\varepsilon}}
\newcommand{\stress}{\tns{\sigma}}
\newcommand{\Macrostrain}{\tns{E}}%{\bar{\strain}}
\newcommand{\Macrostress}{\tns{\Sigma}}%{\bar{\stress}}
\newcommand{\dv}{\tns{s}}
\newcommand{\nbhd}{O}
\newcommand{\thickness}{t}
\newcommand{\bulk}{K}
\newcommand{\shear}{G}
\newcommand{\Stiffness}{\tnsfour{C}}
\newcommand{\QoI}{Q}


% Fiber coupling
\newcommand{\stiffnessC}{\ten{C}}%{\ten{\mathfrak{C}}}
\newcommand{\stiffnessD}{\ten{D}}%{\ten{\mathfrak{D}}}
\newcommand{\ds}[1]{\drv{#1}{s}} % derivative along fiber
\newcommand{\axl}{\operatorname{axl}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Theorem envs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{rmk}{Remark}
\newtheorem{lemma}{Lemma}
%\newdefinition{}{Remark}
%\newtheorem{corollary}{Corollary}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Revision
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\myRed}{\color{red!70!black}}
\newcommand{\rev}[1]{{\color{red} #1}}








==> sections/sec_CollocationIGA.tex <==
% !TeX root = ../MAIN.tex

\newcommand{\TrialSpace}{V^h}
\newcommand{\TestSpace}{\hat{V}^h}
\newcommand{\CollocSet}{\mathcal{S}}



Let us consider the following strain energy function for fibers:
\begin{equation}\label{eq:fiber:StrainEnergyDensity}
	\Psi_{F}(\grad\vec{u}_{F}(\x), \ten{R}_{F}(\x))
	=
 	\frac{1}{2}\left(
 		\vec{\eps}\tp\,\stiffnessC\,\vec{\eps} + \vec{\kappa}\tp\,\stiffnessD\,\vec{\kappa}
 	\right)
\end{equation}
where
\begin{equation}\label{key}
	\vec{\eps} = \ten{R}_{F}\tp\left(\drv{\vec{r}}{s} - \vec{d}_1\right),
	\qquad
	\vec{\kappa} = 
	-\mat{
		\vec{d}_3\tp\,\partial_{s}{\vec{d}_2} \\
		\vec{d}_1\tp\,\partial_{s}{\vec{d}_3} \\
		\vec{d}_2\tp\,\partial_{s}{\vec{d}_1}
	},
\end{equation}
with $\vec{r} = \vec{x} + \vec{u}_{F}$, $\x\in\Omega_{F}$, and $\ten{R}_{F} 
=
\mat{\vec{d}_1, \vec{d}_2, \vec{d}_3}$.
The corresponding stiffness tensors are
\begin{equation}\label{eq:stifnessTensors}
	\stiffnessC = \mat{EA &&\\ & k_1 GA &\\ && k_2 GA},
	\qquad
	\stiffnessD = \mat{GJ &&\\ & EI_1 &\\ && EI_2},
\end{equation}
where $E$ is Young's modulus, $G=\frac{E}{2\,(1+\nu)}$ is shear modulus with Poissonratio~$\nu$, $A$ is cross area, $I_j$ are second moments of area (planar), $J$ torsion constant (polar second moment \rev{?}), $k_j$ are shear correction factors.
Typically $J = I_1 + I_2$ and $k_1=k_2=\frac{5}{6}$.


From~\eqref{eq:fiber:StrainEnergyDensity}, we have
\begin{equation}\label{key}
\vec{N} = \drv{\Psi_{F}}{\grad\vec{u}_F} = \ten{R}_{F}\,\stiffnessC\,\vec{\eps},
\end{equation}
The fiber cross-section orientation is a tensor field $\ten{R}_{F}: [0,L] \to \SO{3}$ and can be represented as
\begin{gather}\label{key}
	\ten{R}_{F}(\x) = \Exp{\sum\limits_{j=1}^{3}\theta_j(\x)\,\ten{L}_j},\\
	\ten{L}_1 = \mat{0&0&0\\ 0&0&-1 \\0&1 &0}, 
	\qquad
	\ten{L}_2 = \mat{0&0& 1\\ 0&0&0\\ -1 &0&0}, 
	\qquad
	\ten{L}_3 = \mat{0& -1 &0\\ 1 &0&0\\0&0&0}.
\end{gather}
Thus, we have the variation $\ten{\delta R}_{F} = \sum\limits_{j=1}^{3}\ten{R}_{F}\,\ten{L}_j\,\delta\theta_j$, and hence we have
\begin{align}\label{key}	
\int_{0}^{L}\ten{Q}:\ten{\delta R} \d s
&=
\int_{0}^{L}\drv{\Psi_{F}}{\ten{R}_{F}}:\ten{\delta R}\d s \\
&=
\int_{0}^{L}\drv{\Psi_{F}}{\ten{R}_{F}}:\sum\limits_{j=1}^{3}\ten{R}_{F}\,\ten{L}_j\,\delta\theta_j\d s \\
&=
\int_{0}^{L}\left(\vec{\delta\theta}\tp\left(\drv{\vec{r}}{s}\times\left(\ten{R}_{F}\,\stiffnessC\,\vec{\eps}\right)\right) - \drv{\vec{\delta\theta}}{s}\tp\ten{R}_{F}\,\stiffnessD\,\vec{\kappa}\right)\d s \\
&= \int_{0}^{L}\left(\drv{\vec{M}}{s} + \drv{\vec{r}}{s}\times\vec{N}\right)\cdot\vec{\delta\theta}\d s - \left(\vec{M}\cdot\vec{\delta\theta}\right)\bigr|_{0}^{L},
\end{align}
where we denoted $\vec{M} = \ten{R}_{F}\,\stiffnessD\,\vec{\kappa}$.

Let us introduce the quaternion parametrization of the rotational matrix~$\ten{R}_{F}$ using vector $\vec{q}\in\R^4$:
\begin{equation}\label{key}
\ten{R}_{F} 
=
\mat{\vec{d}_1, \vec{d}_2, \vec{d}_3}
=
\mat{
	q_1^2 - q_2^2 - q_3^2 + q_4^2 &
	2\,(q_1\,q_2 - q_3\,q_4) &
	2\,(q_1\,q_3 + q_2\,q_4)
	\\
	2\,(q_1\,q_2 + q_3\,q_4) &
	-q_1^2 + q_2^2 - q_3^2 + q_4^2 &
	2\,(q_2\,q_3 - q_1\,q_4)
	\\
	2\,(q_1\,q_3 - q_2\,q_4) &
	2\,(q_2\,q_3 + q_1\,q_4) &		
	-q_1^2 - q_2^2 + q_3^2 + q_4^2
}
\end{equation}
Given the normalized directors~$\vec{d}_j$, the vector~$\vec{q}$ is normalized:
\begin{equation}\label{key}
\abs{\vec{d}_j} = 1
\qquad
\Leftrightarrow
\qquad
q_1^2 + q_2^2 + q_3^2 + q_4^2 = 1.
\end{equation}

\subsection{Discretization}
%\paragraph{Discretization.} 
Let us consider a Petrov-Galerkin type approximation.
We approximate the solution with
$\vec{u}_{M}\in \TrialSpace_{M}$, $\vec{u}_{F}\in \TrialSpace_{F}$, $\vec{q}\in \TrialSpace_{q}$, $\vec{\lambda}\in \TrialSpace_{\lambda}$, such that
\begin{equation}
\begin{aligned}\label{eq:sys:PG}
\int\limits_{\Omega} \ten{P}_{M}\!\left(\grad\vec{u}_{M}\right):\grad\vec{\phi}_{M} \d\x 
+
\!\!\int\limits_{\Omega} \vec{f}_{vol}\cdot\vec{\phi}_{M} \d\x
+
\!\!\int\limits_{\Gamma_N} \vec{t}_{ext}\cdot\vec{\phi}_{M} \d\x
&+
\!\!\int\limits_{0}^{L}\vec{\lambda}\cdot\vec{\phi}_{M}\d s
+
\!\!\!\!\sum_{\hat{s}\in\{0,L\}} \!\!\!\!\vec{\hat{\lambda}}_{\hat{s}}\cdot\vec{\phi}_{M}(\hat{s})
= 0,
\\
\int\limits_{0}^{L}\left(
\drv{\vec{N}}{s}
+
\vec{\lambda}
-
\vec{\bar{f}}_{vol}
\right)\cdot\vec{\phi}_{F} \d s
&= 0,
\qquad
\vec{N}(0) = \vec{\hat{\lambda}}_{0}, \qquad \vec{N}(L) = \vec{\hat{\lambda}}_{L}, 
\\	
\int\limits_{0}^{L}\left(\drv{\vec{M}}{s} + \drv{\vec{r}}{s}\times\vec{N}\right)\cdot\vec{\phi}_{\theta}\d s &= 0,
\qquad
\vec{M}(0) = \vec{0}, \qquad \vec{M}(L) = \vec{0}, 
\\
\int\limits_{0}^{L} (\vec{u}_{M}-\vec{u}_{F})\cdot\vec{\phi}_{\lambda}\d s &= 0,
\end{aligned}
\end{equation}
for all $\vec{\phi}_{M}\in\TestSpace_{M}$, $\vec{\phi}_{F}\in\TestSpace_{F}$, $\vec{\phi}_{\theta}\in\TestSpace_{\theta}$, $\vec{\phi}_{\theta}\in\TestSpace_{\lambda}$.


Let $\CollocSet = \{s_k, \; k=1..n\}$ be a set of $n$ points on $[0,L]$, such that $s_k\notin\{0,L\}$, and let us consider
$$\TestSpace_{F} = \TestSpace_{\theta} = \TestSpace_{\lambda} = \TrialSpace_{\lambda} = \vspan\{\delta(s-s_k), \; s_k\in\CollocSet\}^3,$$ 
where $\delta(s)$ denotes Dirac $\delta$-function.
That is, $\vec{\lambda}(s) = \sum_{k=1}^{n}\vec{\lambda}_k\,\delta(s-s_k)$, $\vec{\lambda}_k\in\R^3$.
%Then, the system~\eqref{eq:sys:PG} reduces to
%\begin{equation}
%\begin{aligned}\label{eq:sys:PG}
%\int\limits_{\Omega} \ten{P}_{M}\!\left(\grad\vec{u}_{M}\right):\grad\vec{\phi}_{M} \d\x 
%+
%\!\!\int\limits_{\Omega} \vec{f}_{vol}\cdot\vec{\phi}_{M} \d\x
%+
%\!\!\int\limits_{\Gamma_N} \vec{t}_{ext}\cdot\vec{\phi}_{M} \d\x
%&+
%\!\!\int\limits_{0}^{L}\vec{\lambda}\cdot\vec{\phi}_{M}\d s
%+
%\!\!\!\!\sum_{\hat{s}\in\{0,L\}} \!\!\!\!\vec{\hat{\lambda}}_{\hat{s}}\cdot\vec{\phi}_{M}(\hat{s})
%= 0,
%\\
%\drv{\vec{N}}{s}
%+
%\vec{\lambda}
%-
%\vec{\bar{f}}_{vol}
%&= 0
%\quad\;\;\text{ in }\CollocSet,
%\qquad
%\vec{N}(0) = \vec{\hat{\lambda}}_{0}, \qquad \vec{N}(L) = \vec{\hat{\lambda}}_{L}, 
%\\	
%\drv{\vec{M}}{s} + \drv{\vec{r}}{s}\times\vec{N} &= 0
%\quad\;\;\text{ in }\CollocSet,
%\qquad
%\vec{M}(0) = \vec{0}, \qquad \vec{M}(L) = \vec{0}, 
%\\
%\vec{u}_{F} &= \vec{u}_{M} \quad\text{in }\CollocSet.
%\end{aligned}
%\end{equation}
Then, assuming $\TrialSpace_{M}=\TestSpace_{M}$, $\TrialSpace_{F}$, $\TrialSpace_{q}$ to be appropriate spline spaces with the knots~$\CollocSet\cup\{0,L\}$, we end up with isogeometric collocation method proposed in~\cite{Weeger2017}.
As in~\cite{Weeger2017}, in order to avoid locking, we consider $\vec{N}$ and $\vec{M}$ as additional unknowns living in appropriate spline spaces $\TrialSpace_{N}$ and $\TrialSpace_{Q}$ respectively.
In what follows, we assume $\TrialSpace_{F} = \TrialSpace_{N} = \TrialSpace_{Q}$.
Thus, from~\eqref{eq:sys:PG} we obtain eventually the system for the unknowns $\vec{u}_{M}\in \TrialSpace_{M}$, $\vec{r}\in \TrialSpace_{F}$, $\vec{q}\in \TrialSpace_{q}$, $\vec{N}\in \TrialSpace_{N}$, $\vec{M}\in \TrialSpace_{Q}$:
\begin{equation}
\begin{aligned}
\int\limits_{\Omega} \ten{P}_{M}\!\left(\grad\vec{u}_{M}\right):\grad\vec{\phi}_{M} \d\x 
+
\!\!\int\limits_{\Omega} \vec{f}_{vol}\cdot\vec{\phi}_{M} \d\x
+
\!\!\int\limits_{\Gamma_N} \vec{t}_{ext}\cdot\vec{\phi}_{M} \d\x
+&
\sum_{k=0}^{n+1}\vec{\lambda}_k\cdot\vec{\phi}_{M}(s_k)
%+
%\!\!\!\!\sum_{\hat{s}\in\{0,L\}} \!\!\!\!\vec{\hat{\lambda}}_{\hat{s}}\cdot\vec{\phi}_{M}(\hat{s})
= 0,
\qquad\forall\vec{\phi}_{M}\in\TestSpace_{M},
\\
\drv{\vec{N}}{s}
+
\vec{\lambda}_k
-
\vec{\bar{f}}_{vol}
= 0
\quad&\text{ in }\CollocSet,
\qquad
\vec{N}(0) = \vec{\lambda}_{0}, \qquad \vec{N}(L) = \vec{\lambda}_{n+1}, 
\\	
\drv{\vec{M}}{s} + \drv{\vec{r}}{s}\times\vec{N} = 0
\quad&\text{ in }\CollocSet,
\qquad
\vec{M}(0) = \vec{0}, \qquad \vec{M}(L) = \vec{0}, 
\\
\vec{r} = \vec{x} + \vec{u}_{M} \quad&\text{ in }\CollocSet,
\\
\vec{q}\cdot\vec{q} = 1 \quad&\text{ in }\CollocSet,
\\
\vec{N} = \ten{R}_{F}(\vec{q})\,\stiffnessC\,\ten{R}_{F}(\vec{q})\tp\left(\drv{\vec{r}}{s} - \vec{d}_1(\vec{q})\right) \quad&\text{ in }\CollocSet\cup\{0,L\},\\
%\quad&\text{ and }\quad
\vec{M} = \ten{R}_{F}(\vec{q})\,\stiffnessD\,\vec{\kappa}(\vec{q}) \quad&\text{ in }\CollocSet\cup\{0,L\},
\end{aligned}
\end{equation}
where $s_0=0$, $s_{n+1}=L$, $\vec{\lambda}_0=\vec{\hat{\lambda}}_0$, $\vec{\lambda}_{n+1}=\vec{\hat{\lambda}}_L$ (remind that $\vec{\lambda}_0$ and $\vec{\lambda}_{n+1}$ have units different from those of $\vec{\lambda}_k$, $k=1..n$).
The Lagrange multipliers~$\vec{\lambda}_k$ can be condensed, so that we obtain
\begin{equation}
\begin{aligned}\label{eq:sys:IGAcollocation}
\int\limits_{\Omega} \ten{P}_{M}\!\left(\grad\vec{u}_{M}\right):\grad\vec{\phi}_{M} \d\x 
+
\!\!\int\limits_{\Omega} \vec{f}_{vol}\cdot\vec{\phi}_{M} \d\x
+
\!\!\int\limits_{\Gamma_N} \vec{t}_{ext}\cdot\vec{\phi}_{M} \d\x
+&
\sum_{k=1}^{n}\left(\vec{\bar{f}}_{vol}-\drv{\vec{N}}{s}\right)(s_k)\cdot\vec{\phi}_{M}(s_k)
+
\!\!\!\!\sum_{\hat{s}\in\{0,L\}} \!\!\!\!\vec{N}(\hat{s})\cdot\vec{\phi}_{M}(\hat{s})
= 0,
\\	
\drv{\vec{M}}{s} + \drv{\vec{r}}{s}\times\vec{N} = 0
\quad&\text{ in }\CollocSet,
\qquad
\vec{M}(0) = \vec{0}, \qquad \vec{M}(L) = \vec{0},
\\
\vec{r} = \vec{x} + \vec{u}_{M} \quad&\text{ in }\CollocSet, 
\\
\abs{\vec{q}}^2 = 1 \quad&\text{ in }\CollocSet,
\\
\vec{N} = \ten{R}_{F}(\vec{q})\,\stiffnessC\,\ten{R}_{F}(\vec{q})\tp\left(\drv{\vec{r}}{s} - \vec{d}_1(\vec{q})\right) \quad&\text{ in }\CollocSet\cup\{0,L\},\\
%\quad&\text{ and }\quad
\vec{M} = \ten{R}_{F}(\vec{q})\,\stiffnessD\,\vec{\kappa}(\vec{q}) \quad&\text{ in }\CollocSet\cup\{0,L\},
\end{aligned}
\end{equation}
for all $\forall\vec{\phi}_{M}\in\TestSpace_{M}$.

==> sections/sec_Coupling.tex <==
In the next step, we aim at to embed a number of fibers into the matrix material. The coupling can be established using two general approaches, namely boundary fitted methods and immersed methods. In some sense, this is similar to the discussions on Fluid-Structure Interaction problems, although we assume here that the relative position of the fiber to the matrix does not change. Since we assume that the fibers are thin and written in terms of beam strain measures, we follow an immersed approach, to be interpreted as overlapping domain decomposition method, see [???hesch2014c] for a detailed discussion on this topic in the context of FSI. This allows us to embed the fibers independent of the mesh of the matrix material.

\subsection{Beam-Matrix interaction}
The coupling between the fiber and the matrix material can be establish first on the position field, where we assume
\begin{equation}\label{eq:phi1}
\vec{\Phi}_1(\vec{\varphi},\tilde{\vec{\varphi}}) := \vec{\varphi} - \tilde{\vec{\varphi}}\;\text{in}\;\Omega_t\cap\tilde{\Omega}_t,
\end{equation}
must remain valid to enforce congruent positions during the deformation. Note that we restrict $\tilde{\Omega}_t$ to the centerline of the beam. To satisfy this constraint requires the introduction of a suitable vector valued Lagrange multiplier field $\vec{\lambda}$ with admissible variations $\delta\vec{\lambda}$, defined with the functional space
\begin{equation}
\mathcal{M} = \left\{\delta\vec{\lambda}\in\mathcal{L}^2\left(\Omega_t\cap\tilde{\Omega}_t\right)\right\}.
\end{equation}
Here, the Lagrange multipliers  $\vec{\lambda}$ can be considered as force field to ensure the non-slip condition between fiber and matrix. Additionally, we have to link the rotations $\tilde{\vec{R}}$ of the beam to the rotational part $\vec{R}$ of the deformation gradient $\vec{F}$ of the matrix material
\begin{equation}\label{eq:phi2}
\vec{\Phi}_2(\tilde{\vec{R}},\vec{\varphi}) := \op{skew}(\tilde{\vec{R}}^T\vec{F}(\vec{\varphi})),
\end{equation}
where we make use of the formulation proposed by Hughes et al. [???]. For the second set of constraints, we apply a penalty method, as the rotation of the beam axis within the matrix material depend on the adhesive properties between the components, in contrast to the position field. Thus, we reformulate \eqref{eq:phi2}
\begin{equation}
\begin{aligned}
\Psi_2(\tilde{\vec{R}},\vec{\varphi}) :&= \epsilon\op{skew}(\tilde{\vec{R}}^T\vec{F}(\vec{\varphi}):\op{skew}(\tilde{\vec{R}}^T\vec{F}(\vec{\varphi}),\\
&= \frac{\epsilon}{2}\left(\vec{F}(\vec{\varphi}):\vec{F}(\vec{\varphi})-\tilde{\vec{R}}^T\vec{F}(\vec{\varphi}):\vec{F}(\vec{\varphi})\tilde{\vec{R}}^T\right)
\end{aligned}
\end{equation}
where $\epsilon$ is a prescribed penalty factor to account for the adhesive properties.  The constraints $\vec{\Phi}_1$ can directly be inserted into an augmented energy functional
\begin{equation}
\Pi(\vec{\varphi},\tilde{\vec{\varphi}},\mathfrak{q},\vec{\lambda}) = \Pi^{int}(\vec{F}(\vec{\varphi})) + \Pi^{ext}(\vec{\varphi}) + 
\Pi^{fib,int}(\tilde{\vec{\varphi}},\mathfrak{q}) + \Pi^{fib,ext}(\tilde{\vec{\varphi}},\mathfrak{q}) + 
\Pi^{con}(\vec{\varphi},\tilde{\vec{\varphi}},\mathfrak{q},\vec{\lambda}).
\end{equation}
The last term on the right hand side reads
\begin{equation}
\Pi^{con}(\vec{\varphi},\tilde{\vec{\varphi}},\mathfrak{q},\vec{\lambda}) = \int\limits_{\tilde{\Omega}_0}\vec{\lambda}\cdot\vec{\Phi}_1(\vec{\varphi},\tilde{\vec{\varphi}}) + \Psi_2(\tilde{\vec{R}},\vec{\varphi})\,\text{d}V.
\end{equation}
and the variation
\begin{equation}
\begin{aligned}
\delta\Pi^{con}(\vec{\varphi},\tilde{\vec{\varphi}},\mathfrak{q},\vec{\lambda}) = &\int\limits_{\tilde{\Omega}_0}\delta\vec{\lambda}\cdot\vec{\Phi}_1(\vec{\varphi},\tilde{\vec{\varphi}})\,\vec{\varphi})+
\delta\vec{\varphi}\cdot\vec{\lambda} -\delta\tilde{\vec{\varphi}}\cdot\vec{\lambda} + \\
&\delta\vec{\theta}\cdot\epsilon\operatorname{axl}\left((\tilde{\vec{R}}\vec{F}^T)^2)\right) + \nabla_{\vec{X}}(\delta\vec{\varphi}):\epsilon\left(\vec{F}-\tilde{\vec{R}}\vec{F}^T\tilde{\vec{R}}\right)
\,\text{d}V
\end{aligned}
\end{equation}
Note that only the Lagrange multipliers correlating to the constraints $\vec{\Phi}_1$ are added to the system. We will remove them along with the centerline position vector $\tilde{\vec{\varphi}}$ using a suitable discrete Null-Space reduction scheme, once we have discretised the whole system.

\textcolor{red}{Link to IFEM, reduction of the stiffness as usual for overlapping domains.}




==> sections/sec_Coupling2.tex <==
% !TeX root = ../MAIN.tex

\section{\rev{I don't know where to put this section, so I put it in the end for the time being.}}

\subsection{3D-beam/3D-matrix system}



Let us consider a Lipschitz convex bounded domain~$\Omega\subset\R^3$, such that $\Omega = \Omega_{M}\cup\Omega_{F}$, where $\Omega_{M}$ corresponds to the material matrix and $\Omega_{F}\subset\R^3$ to the fiber.


The subdomains $\Omega_{M}$ and $\Omega_{F}$ are closed and their intersection $\Gamma = \Omega_{M}\cap\Omega_{F}$ is the fiber/matrix interface.
Let $\partial\Omega_{N}$ be a part of the boundary~$\partial\Omega$ associated to Neumann boundary conditions.
The matrix and the fiber are presented respectively as Cauchy and Cosserat continua.
The displacement field is
\begin{equation}\label{key}
	\x_{glo}(\X) =
	\begin{cases}
	\mtx{\x}(\X), & \text{ in } \Omega\setminus\Omega_{F}, \\
	\fib{\x}(\X), & \text{ in } \Omega_{F}, \\
	\end{cases}
\end{equation}
where $\mtx{\x}(\X)$ and $\fib{\x}(\X)$ denote deformation fields of matrix and fiber respectively.
Besides, $\fib{\ten{R}}(\X)$, $\X\in\Omega_{F}$, is orthogonal matrix of directors of the fiber. 
The total energy of the matrix/fiber system is
\begin{equation}\label{eq:Total_Energy}
%	W = \Pi_{M} + \Pi_{F} + \Pi_{interact} + \Pi_{ext},
	\Pi = \Pi_{M} + \Pi_{F} + \Pi_{C},
\end{equation}
where $\Pi_{M}$ and $\Pi_{F}$ stand for the internal energy of the matrix and the fiber respectively, and $\Pi_{C}$ is the coupling term:
\begin{align}\label{key}
	\Pi_{M} &= \int\limits_{\Omega_{M}} \Psi_{M} \d V
	+
	\int\limits_{\Omega_{M}} \vec{f}_{vol}\cdot\left(\mtx{\x}-\X\right) \d V
	+
	\int\limits_{\partial\Omega_{N}} \vec{t}_{ext}\cdot\left(\mtx{\x}-\X\right) \d V
	, \\
	\Pi_{F} &= \int\limits_{\Omega_{F}} \Psi_{F} \d V
	+
	\int\limits_{\Omega_{F}} \vec{f}_{vol}\cdot\left(\fib{\x}-\X\right) \d V
	, \\
	\Pi_{C} &= \int\limits_{\Gamma}  \left(\mtx{\x}-\fib{\x}\right)\cdot\vec{\mu}\d S
	- \int\limits_{\Gamma}  \frac{\alpha}{2}\,\vec{\mu}^2\d S
	, \label{eq:fib:FreeEnergy}
\end{align}
where $\Psi_{M}$ and $\Psi_{F}$ denote internal free energy densities of the matrix and the fiber respectively,
%where $\mtx{\x}$ and $\fib{\x}$ denote displacement fields of matrix and fiber respectively, and $\fib{\ten{R}}$ is the directors matrix of the fiber.
%where $\ten{\eps}_{F} = \ten{\eps}_{F}(\nabla\fib{\x}, \fib{\ten{R}})$ is the Green--Lagrange strain tensor and $\ten{\kappa}_{F} = \ten{\kappa}_{F}(\nabla\fib{\x}, \fib{\ten{R}})$ is the curvature tensor, $\ten{C}$ and $\ten{D}$ are the corresponding stiffness higher order tensors.
%The fiber is presented as Cosserat media described by the displacement~$\fib{\x}$ and rotation tensor~$\fib{\ten{R}}$.
%Above, $\Pi_{interact}$ is the work of matrix/fiber interaction forces:
%\begin{align}\label{key}
%	\Pi_{interact} &= \int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{t}_{int} \cdot(\mtx{\x}-\fib{\x})\d V,\\
%	\Pi_{ext} &= 
%	\int\limits_{\Omega_{M}\cup\Omega_{F}} \!\!\!\!\vec{f}_{vol}\cdot\vec{u} \d V
%	+
%	\int\limits_{\partial\Omega_{N}} \vec{t}_{ext}\cdot\vec{u} \d V,
%\end{align}
%where 
%$\rho_{M}$ and $\rho_{F}$ stand for the corresponding mass densities,
%$\mtx{\vec{u}} = \mtx{\x}-\X$ and $\fib{\vec{u}} = \fib{\x}-\X$ are the displacement fields of the matrix and the fiber respectively,
$\vec{f}_{vol}$ and $\vec{t}_{ext}$ are respectively volumetric force density and external load applied on~$\partial\Omega_{N}$, 
and $\vec{\mu}$ is a Lagrange multiplier associated to the surface load on the matrix/fiber interface.
The coupling term~$\Pi_{C}$ in this form defines the fiber/matrix interaction of spring type:
the coefficient~$\alpha\ge0$ corresponds to the inverse spring stiffness.
In what follows we are going to consider the case~$\alpha=0$ (infinite stiffness), which corresponds to displacement continuity constraint on the interface.
%and $\vec{t}_{int}$ is the surface load on the matrix/fiber interface.
%and is also unknown, along with displacement field and the fiber directors.
%The form of the interface load~$\vec{t}_{int}$ is defined by the type of matrix/fiber coupling.
%For example, in case of soft coupling of spring type it writes as $\vec{t}_{int} = k\cdot(\mtx{\x}-\fib{\x})$, with $k$ being the stiffness.
%In what follows, we consider hard coupling implying displacement continuity constraints: $k\to\infty$, $\abs{\vec{t}_{int}}<\infty$, so that $\vec{t}_{int}$ plays role of Lagrange multiplier.
%The form of such multiplier also defines type of constraint.
%For example, the interface load of the form $\vec{t}_{int} = \alpha\cdot\vec{n}$, with a scalar Lagrange multiplier~$\alpha$ and $\vec{n}$ being a normal to the interface, corresponds to a non-penetration constraint.
%%and $\vec{t}_{int}$ is the interaction force density between matrix and fiber surfaces.

Thus, we have a saddle point optimization problem to solve:
\begin{equation}\label{key}
\inf\limits_{\x_{glo},\fib{\ten{R}}} \; \sup\limits_{\vec{\mu}} \; \Pi(\x_{glo},\fib{\ten{R}},\vec{\mu}).
\end{equation}
The corresponding Euler-Lagrange equation writes
\begin{multline}\label{eq:Euler-Lagrange}
\int\limits_{\Omega_{M}} \drv{\Psi_{M}}{\mtx{\ten{F}}}:\ten{\delta \mtx{F}} \d V
+
\int\limits_{\Omega_{F}} \drv{\Psi_{F}}{\fib{\ten{F}}}:\ten{\delta\fib{F}} \d V
%+
%\int\limits_{\Omega_{F}} \ten{G}_{F}:\ten{\delta\fib{R}} \d V
%	+
%	\int\limits_{\Omega_{F}} \left(\ten{\eps}_{F}:\ten{C}:\ten{\delta\eps}_{F} + 	\ten{\kappa}_{F}:\ten{D}:\ten{\delta\kappa}_{F}\right) \d V
+\\
+
\!\!\!\!\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\mu} \cdot(\vec{\delta\mtx{x}}-\vec{\delta\fib{x}})\d S
+
\!\!\!\!\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\delta\mu} \cdot(\mtx{\x}-\fib{\x})\d S
%	+
%	\!\!\!\!\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\mu} \cdot(\vec{\delta u}_{M}-\vec{\delta\fib{\varphi}})\d V
%	+
%	\!\!\!\!\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\delta f}_{interact} \cdot(\mtx{\x}-\fib{\x})\d V
+ \\
+
\int\limits_{\Omega} \vec{f}_{vol}\cdot\vec{\delta x}_{glo} \d V
+
\int\limits_{\partial\Omega_{N}} \vec{t}_{ext}\cdot\vec{\delta x}_{glo} \d S
= 0.
\end{multline}
%where $\ten{P}_M$ and $\ten{P}_{F}$ are the $1$st Piola-Kirchhoff stress tensors of the matrix and the fiber respectively, and $\ten{G}_{F}$ is \rev{(What is $\ten{G}_{F}$ ??)}.
%, and $\ten{F}=\nabla\vec{u}$ is the deformation gradient.
Without loss of generality, we assume $\vec{f}_{vol}=0$ in what follows. 


\subsection{Thin rigid fiber model.}
Let us consider a thin, geometrically exact 3D beam with rigid cross-section.
Let $[\vec{D}_1,\,\vec{D}_2,\,\vec{D}_3]$ be an orthonormal triad, where $\vec{D}_{\alpha}$ ($\alpha=1,\,2$) span the plane cross section of the beam.
Then, the fiber domain~$\Omega_{F}\subset\Omega$ is defined as
\begin{equation}%\label{eq:fib:position_ref}
\Omega_{F} = \big\{ \vec{X}(\theta^{\alpha},s) = \vec{X}_c(s) + \theta^{\alpha}\vec{D}_{\alpha}(s) \big\},
% \vec{X}(\theta^{\alpha},s) = \vec{X}_c(s) + \theta^{\alpha}\vec{D}_{\alpha}(s),
\end{equation}
parameterized in terms of arclength~$s\in [0,\,L]$ along the center line~$\vec{X}_c(s)$ of the beam of length $L$,
%Moreover, an orthonormal triad $[\vec{D}_1,\,\vec{D}_2,\,\vec{D}_3]$ with
and convective coordinates
$\theta^{\alpha}\in[-r,r]$ ($\alpha=1,\,2$), 
%$\theta^i = (\theta^{\alpha},s)\in\Omega_{F}$ $(i=1,\,2,\,3;\,\alpha=1,\,2)$ 
%is introduced, were $\vec{D}_{\alpha}$ span the plane cross section of the beam.
the radius~$r$ being much less than the problem characteristic length.
The deformation field is
\begin{equation}%\label{eq:fib:position}
\tilde{\vec{x}}(\theta^{\alpha},s) = \fib{\vec{\varphi}}(s) + \theta^{\alpha}\vec{d}_{\alpha}(s).
\end{equation}
Here, the orthonormal triad $\vec{d}_i$ is related to the reference triad via the rotation tensor $\fib{\ten{R}}\in SO(3)$, i.e. $\fib{\ten{R}} = \vec{d}_i\otimes\vec{D}_i$.
Above and further, Einstein summation convention is used.

%We assume the fiber to be thin enough to be modeled as a rigid cross-section beam.
%That is, we assume $r<<L$, where $r$ is the radius of the fiber cross-section, and $L$ is the fiber length.
%Then, from~\eqref{eq:fib:position_ref} and \eqref{eq:fib:position}, the fiber deformation field is
%\begin{equation}\label{eq:u_fib}
%\fib{\x}\!\left(\theta^\alpha,s\right) = \fib{\vec{\varphi}}(s) + \theta^{\alpha}\vec{d}_{\alpha}(s)
%\quad\text{ in }\Omega_{F}.
%\end{equation}
%Then, from~\eqref{eq:fib:position_ref} and \eqref{eq:fib:position}, the fiber deformation field is
%\begin{equation}\label{eq:u_fib}
%	\fib{\x}\!\left(\fib{\X}(\theta^\alpha,s)\right) = \fib{\vec{\varphi}}(s) + \fib{\ten{R}}(s)\left(\fib{\X}-\fib{\X}_c(s)\right)
%	\quad\text{ in }\Omega_{F},
%\end{equation}
%where 
%%$\ten{R}_0$ is the reference fiber orientation \rev{(it can depend on $s$)}, and 
%$\fib{\X}_c(s)$ is the coordinates of the centerline point corresponding to the arc-length~$s\in[0,L]$.
%%Without loss of generality, we assume that $\abs{\drv{\x_c}{s}}=1$.
%%By abuse of notation, in what follows. we denote $\fib{\x}(s) = \fib{\x}(\x_c(s))$.

%\begin{proof}
%	We have
%	\begin{equation}\label{eq:kin1}
%	\tilde{\vec{X}}(\theta^{\alpha},s) = \tilde{\vec{X}}_0(s) + \theta^{\alpha}\vec{D}_{\alpha}(s),
%	\end{equation}
%	and
%	\begin{equation}\label{eq:kin2}
%	\tilde{\vec{x}}(\theta^{\alpha},s) = \tilde{\vec{\varphi}}(s) + \theta^{\alpha}\vec{d}_{\alpha}(s).
%	\end{equation}	
%	From~\eqref{eq:kin1}, it holds
%	\begin{align}
%		\theta^1 &= \vec{D}_{1}(s)\cdot(\tilde{\vec{X}}(\theta^{\alpha},s) - \tilde{\vec{X}}_0(s))\\
%		\theta^2 &= \vec{D}_{2}(s)\cdot(\tilde{\vec{X}}(\theta^{\alpha},s) - \tilde{\vec{X}}_0(s))\\
%		0 &=\vec{D}_{3}(s)\cdot\left(\tilde{\vec{X}}(\theta^{\alpha},s) - \tilde{\vec{X}}_0(s)\right)
%	\end{align}	
%	Substituting this to~\eqref{eq:kin2}, we obtain
%	\begin{align}
%	\fib{\x}\!\left(\fib{\X}(\theta^\alpha,s)\right) &= \fib{\vec{\varphi}}(s) + \sum_{i=1}^{3}\vec{d}_i\otimes\vec{D}_i\left(\fib{\X}-\fib{\X}_c(s)\right)\\
%	&=  \fib{\vec{\varphi}}(s) + \fib{\ten{R}}(s)\left(\fib{\X}-\fib{\X}_c(s)\right).
%	\end{align}
%	
%\end{proof}


\input{tikz/fiber3D/fiber3D}

Let us denote by $A(s)$ and $C(s)$ respectively the fiber cross-section and its boundary corresponding to the arc-length~$s$.
Then, taking in account that
\begin{equation}\label{eq:zero_integrals}
	\int\limits_{A(s)}\theta^{\alpha}\vec{d}_{\alpha}(s)\d A = \int\limits_{C(s)}\theta^{\alpha}\vec{d}_{\alpha}(s)\d C = 0.
\end{equation}
%we can write
%\begin{align}
%	\int\limits_{A(s)}\fib{\x}\d A
%	&=
%	\int\limits_{A(s)}\biggl(\fib{\vec{\varphi}}(s) + \fib{\ten{R}}(s)\left(\theta^{\alpha}\vec{D}_{\alpha}(s)\right)\biggr)\d A
%	=
%	\abs{A}\,\fib{\vec{\varphi}}(s),
%	\label{eq:integralA_uF}\\
%%\intertext{and}
%	\int\limits_{C(s)}\fib{\x}\d C
%	&=
%	\int\limits_{C(s)}\biggl(\fib{\vec{\varphi}}(s) + \fib{\ten{R}}(s)\left(\theta^{\alpha}\vec{D}_{\alpha}(s)\right)\biggr)\d C
%	=
%	\abs{C}\,\fib{\vec{\varphi}}(s),
%	\label{eq:integralC_uF}
%\end{align}
%where $\abs{A}$ and $\abs{C}$ are respectively the area of the fiber cross-section and the length of the fiber circumference.
%Likewise, the corresponding variation writes
%\begin{gather}
%	\vec{\delta\fib{x}}(\X)
%	=
%	\vec{\delta\fib{\varphi}}(s) + \ten{\delta\fib{R}}(s)\left(\theta^{\alpha}\vec{D}_{\alpha}(s)\right),\\	
%	\int\limits_{A(s)}\vec{\delta\fib{x}}\d A
%	=
%	\abs{A}\,\vec{\delta\fib{\varphi}}(s), 
%	\qquad
%	\int\limits_{C(s)}\vec{\delta\fib{x}}\d C
%	=
%	\abs{C}\,\vec{\delta\fib{\varphi}}(s).
%\end{gather}


\paragraph{Lagrange multipliers (interface load).} Lagrange multipliers~$\vec{\mu}$ can be decomposed into mean and fluctuation parts:
\begin{align}\label{key}
	\vec{\mu}\big|_{\Circ(s)} &= \vec{\bar{\mu}}(s) + \vec{\tilde{\mu}}(\theta^{\alpha}),
	\quad\text{where}\quad
	\vec{\bar{\mu}}(s) = \int\limits_{C(s)}\vec{\mu}\d C,
	\quad
	\int\limits_{C(s)}\vec{\tilde{\mu}}\d C = 0,
	\\
	\vec{\mu}\big|_{\Area_{0,L}} &= \vec{\bar{\mu}}_{0,L} + \vec{\tilde{\mu}}_{0,L}(\theta^{\alpha}),
	\quad\text{where}\quad
	\vec{\bar{\mu}}_{0,L} = \int\limits_{\Area_{0,L}}\vec{\mu}\d C,
	\quad
	\int\limits_{\Area_{0,L}}\vec{\tilde{\mu}}_{0,L}\d C = 0,
\end{align}
where the average term~$\vec{\bar{\mu}}$ corresponds to the resulting force applied to the cross-section, while the zero-mean term~$\vec{\tilde{\mu}}$ contains the hydrostatic pressure terms and force couples and is thus associated to the pressure, shear and coupling torque. 
%In what follows, due to the assumption that the fiber radius~$r$ is small, we neglect the torques, i.e. $\vct{\mu}=\vec{\bar{\mu}}$.
Taking in account~\eqref{eq:zero_integrals}, we have
\begin{align}\label{eq:LM_decomposition}
	\int\limits_{C(s)}\fib{\x}\cdot\vec{\delta\mu}\d C
	&=
	\abs{C}\,\fib{\vec{\varphi}}(s)\cdot\vec{\delta\bar{\mu}}(s)
	+
	\int\limits_{C(s)}\theta^{\alpha}\vec{d}_{\alpha}\cdot\vec{\delta\tilde{\mu}}\d C, \\	
	\int\limits_{\Area_{0,L}}\fib{\x}\cdot\vec{\delta\mu}\d C
	&=
	\abs{A}\,\fib{\vec{\varphi}}(s_{0,L})\cdot\vec{\delta\bar{\mu}}_{0,L}
	+
	\int\limits_{\Area_{0,L}}\theta^{\alpha}\vec{d}_{\alpha}\cdot\vec{\delta\tilde{\mu}}\d C.
\end{align}
Hence, we obtain
\begin{align}\label{key}
\!\!\!\!\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\delta\mu} \cdot(\mtx{\x}-\fib{\x})\d V
%&=
%\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\delta\mu} \cdot\biggl(\mtx{\x}-\fib{\vec{\varphi}} - \fib{\ten{R}}\left(\X-\X_{c}\right)\biggr)\d V \\
&=
\int\limits_{\partial\Omega_{F,3}} \vec{\delta\mu} \cdot(\mtx{\x}-\fib{\x})\d V
+
\int\limits_{\partial\Omega_{F,1/2}} \vec{\delta\mu} \cdot(\mtx{\x}-\fib{\x})\d V
\\
&=
\abs{C}\!\int\limits_{0}^{L}\vec{\delta\bar{\mu}} \cdot\left(\frac{1}{\abs{C}}\!\int\limits_{C(s)} \mtx{\x}\d C - \fib{\vec{\varphi}}(s)\right)\d s \\
&+
\abs{A}\!\!\sum_{s\in\{0,L\}} \vec{\delta\bar{\mu}}_{0,L}(s) \cdot\left(\frac{1}{\abs{A}}\!\!\int\limits_{A(s)} \mtx{\x}\d A -\fib{\vec{\varphi}}(s) \right)\\
&+
\int\limits_{0}^{L}\int\limits_{C(s)}\vec{\delta\tilde{\mu}}\cdot\bigg(\mtx{\x}-\theta^{\alpha}\vec{d}_{\alpha}\bigg)\d C\d s
+
\int\limits_{A_{0,L}}\vec{\delta\tilde{\mu}}_{0,L}\cdot\bigg(\mtx{\x}-\theta^{\alpha}\vec{d}_{\alpha}\bigg)\d A,
\end{align}
and
\begin{align}\label{key}
\!\!\!\!\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\mu} \cdot\vec{\delta\fib{\varphi}}\d V
&=
\abs{C}\!\int\limits_{0}^{L}\vec{\bar{\mu}} \cdot \vec{\delta \fib{\varphi}}\d s
+
\abs{A}\!\!\sum_{s\in\{0,L\}} \vec{\bar{\mu}}_{0,L}(s) \cdot\vec{\delta \fib{\varphi}}(s) +\\
&+
\int\limits_{0}^{L}\int\limits_{C(s)}\vec{\tilde{\mu}}\tp\,\ten{\delta\fib{R}}\,\left(\theta^{\alpha}\vec{D}_{\alpha}\right)\d C \d s +
\int\limits_{A_{0,L}}\vec{\tilde{\mu}}_{0,L}\tp\,\ten{\delta\fib{R}}\,\left(\theta^{\alpha}\vec{D}_{\alpha}\right)\d A.
%\\
%&=
%\int\limits_{0}^{L}\vec{\delta\lambda} \cdot\left(\frac{1}{\abs{C}}\!\!\int\limits_{C(s)} \mtx{\x}\d C - \fib{\x}(s)\right)\d s
%+
%\sum_{s\in\{0,L\}} \vec{\delta\lambda}(s) \cdot\left(\frac{1}{\abs{A}}\!\!\int\limits_{A(s)} \mtx{\x}\d A -\fib{\x}(\hat{s}) \right),
%\intertext{and}
%\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\mu} \cdot\vec{\delta u}_{M} \d V
%&=
%\int\limits_{0}^{L}\vec{\lambda} \cdot\left(\frac{1}{\abs{C}}\!\!\int\limits_{C(s)} \vec{\delta u}_{M}\d C\right)\d s
%+
%\sum_{s\in\{0,L\}} \!\!\!\vec{\lambda}(s) \cdot\left(\frac{1}{\abs{A}}\!\!\int\limits_{A(s)} \vec{\delta u}_{M}\d A\right).
\end{align}

Thus,
\begin{equation}\label{key}
\begin{aligned}
\delta\Pi_{C}
&=
\int\limits_{\Gamma}\left(\vec{\bar{\mu}} + \vec{\tilde{\mu}}\right)\cdot \vec{\delta \mtx{x}} \d S
+
\abs{C}\!\int\limits_{0}^{L}\vec{\bar{\mu}} \cdot \vec{\delta\fib{\varphi}}\d s
+
\abs{A}\!\!\sum_{s\in\{0,L\}} \vec{\bar{\mu}}_{0,L}(s) \cdot\vec{\delta\fib{\varphi}}(s)
+\\
&+\int\limits_{0}^{L}\int\limits_{C(s)}\vec{\tilde{\mu}}\tp\,\ten{\delta\fib{R}}\,\left(\theta^{\alpha}\vec{D}_{\alpha}(s)\right)\d C\d s +
\int\limits_{A_{0,L}}\vec{\tilde{\mu}}_{0,L}\tp\,\ten{\delta\fib{R}}\,\left(\theta^{\alpha}\vec{D}_{\alpha}(s)\right)\d A
+\\
&+\int\limits_{0}^{L}\vec{\delta\bar{\mu}} \cdot\left(\fib{\vec{\varphi}}(s)-\frac{1}{\abs{C}}\!\int\limits_{C(s)} \mtx{\x}\d C\right)\d s
+
\!\!\sum_{s\in\{0,L\}}\!\!\vec{\delta\bar{\mu}}(s)\cdot\left(\fib{\vec{\varphi}}(s) - \frac{1}{\abs{A}}\!\!\int\limits_{A(0)} \mtx{\x}\d A\right)
+\\
&+\frac{1}{\abs{C}}\!\int\limits_{\partial\Omega_{F, 3}}\vec{\delta\tilde{\mu}}\cdot\bigg(\mtx{\x}-\theta^{\alpha}\vec{d}_{\alpha}\bigg) \d S
+
\frac{1}{\abs{A}}\!\int\limits_{\Area_{0,L}}\!\!\vec{\delta\tilde{\mu}}_{0,L}\cdot\bigg(\mtx{\x}-\theta^{\alpha}\vec{d}_{\alpha}\bigg)\d A.
\end{aligned}
\end{equation}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Reduced model
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Reduced problem}

Let us consider a natural continuation of matrix solution inside the fiber domain~$\Omega_{F}$.
Such continuation of the solution will produce an error which depends on fiber radius~$r$, see~\cite{Koeppl2017}.
Moreover, under some regularity assumptions, this solution~$\mtx{\x}(\X)$ admits the following expansion in the vicinity of $\mtx{\x}(\X_{c})$:
\begin{equation}\label{eq:expansion}
\mtx{\x}(\theta^{\alpha},s) = \mtx{\x}_{c}(s) + \mtx{\ten{F}}_{c}(s)\cdot\theta^{\alpha}\vec{D}_{\alpha}(s) + \O\left((\theta^{\alpha})^2\right),
\end{equation}
\rev{TODO: rigorous proof of \eqref{eq:expansion} ?}
where we denoted by $\mtx{\x}_{c}(s) = \mtx{\x}(\X_{c}(s))$ and $\mtx{\ten{F}}_{c}(s)=\mtx{\ten{F}}(\X_{c}(s))$ respectively the deformation map and the deformation gradient of the matrix points corresponding to the fiber centerline in the reference configuration.
%\begin{equation}\label{key}
%\mtx{\x}(\theta^{\alpha},s) = \mtx{\x}(\X_{c}(s)) + \mtx{\ten{F}}(\X_{c}(s))\cdot\left(\theta^{\alpha}\vec{D}_{\alpha}(s)\right) + \O\left((\theta^{\alpha})^2\right),
%\end{equation}
%Thus, under thin fiber assumption, we will consider the reduced model with the matrix solution extended into the fiber domain, and the circumference average of the matrix deformation in the coupling condition is replaced by the matrix deformation at the fiber centerline.
Then, taking in account~\eqref{eq:zero_integrals}, we have
\begin{equation}\label{eq:red_pb:pos_cond}
\frac{1}{\abs{C}}\!\int\limits_{C(s)} \mtx{\x}\d C = \mtx{\x}(\X_{c}) +  \O(r^2)
\end{equation}
and, given zero mean of $\vec{\delta\tilde{\mu}}$, we obtain
%\begin{equation}\label{key}
%\frac{1}{\abs{C}}\!\int\limits_{C(s)}\vec{\delta\tilde{\mu}}\cdot\mtx{\x} \d C
%=0
%\end{equation}
\begin{equation}\label{eq:red_pb:rot_cond_1}
\frac{1}{\abs{C}}\!\int\limits_{C(s)}\vec{\delta\tilde{\mu}}\cdot\bigg(\mtx{\x}-\theta^{\alpha}\vec{d}_{\alpha}\bigg) \d C
=
\frac{1}{\abs{C}}\!\int\limits_{C(s)}\vec{\delta\tilde{\mu}}\tp\bigg(\mtx{\ten{F}}_{c}-\fib{\ten{R}}\bigg)\left(\theta^{\alpha}\vec{D}_{\alpha}\right) \d C +  \O(r^2).
\end{equation}

Assume that $\vec{\tilde{\mu}}$ is a combination of torque and pressure (i.e. we neglect the shear):
\begin{equation}\label{key}
\vec{\tilde{\mu}}(\theta^{\alpha},s) = \vec{\mu}_{\tau}(s)\times\ten{\fib{R}}(s)\vec{n}(\theta^{\alpha}) + \mu_{n}(s)\,\ten{\fib{R}}(s)\vec{n}(\theta^{\alpha}),
\end{equation}
where $\vec{n}=\vec{D}_1\,\cos\theta + \vec{D}_2\,\sin\theta$ is the unit outer normal to the interface in the reference configuration.
%\begin{equation}\label{key}
%	\HS_{\tilde{\mu}}(\Gamma) = \left\{ \vec{\tilde{\mu}} \;\big|\; \vec{\tilde{\mu}}(\theta^{\alpha},s) = \vec{\mu}_{\tau}(s)\times\vec{n}(\theta^{\alpha},s) + \mu_{n}(s)\,\vec{n}(\theta^{\alpha},s), \; \vec{\mu}_{\tau}\in\HS_{\vec{\fib{\varphi}}}^\prime([0,L]), \mu_{n}\in\HS_{\mu_{n}}([0,L]) \right\}
%\end{equation}
%with the outer normal unit vector
%\begin{equation}\label{key}
%\vec{n}(\theta^{\alpha},s) = \vec{d}_1(s)\,\cos\theta + \vec{d}_2(s)\,\sin\theta.
%\end{equation}
%\begin{equation}\label{key}
%	\vec{n}(\theta^{\alpha},s) = \fib{\ten{R}}(s)\,\vec{n}_0,
%	\qquad
%	\vec{n}_0 = \left[\begin{array}{l}
%	\cos\theta \\
%	\sin\theta \\
%	0
%	\end{array}\right].
%\end{equation}

\rev{Circle section is considered (however, no loss of generality). TODO: generalize for ellipses. Directors transformation (elongation) can be considered.}


%Let us introduce deformed outer normal $\vec{n}=\fib{\ten{R}}\,\vec{n}_0$.
Then, \eqref{eq:red_pb:rot_cond_1} becomes
\begin{equation}\label{eq:red_pb:rot_cond_2}
\begin{aligned}
\frac{1}{\abs{C}}\!\int\limits_{C(s)}\vec{\delta\tilde{\mu}}\cdot\bigg(\mtx{\x}-\theta^{\alpha}\vec{d}_{\alpha}\bigg) \d C
=&
\frac{1}{2\pi}\,\fib{\ten{R}}\tp\vec{\delta\mu}_{\tau}(s)\cdot\int\limits_{C(s)}\vec{n}\times\bigg(\mtx{\fib{\ten{R}}\tp\ten{F}}_{c}-\ten{\Id}\bigg)\vec{n} \d C \\
&+
\frac{1}{2\pi}\,\delta\mu_{n}(s)\int\limits_{C(s)}\vec{n}\cdot\bigg(\fib{\ten{R}}\tp\mtx{\ten{F}}_{c}-\ten{\Id}\bigg)\vec{n} \d C  \\
&+
\frac{1}{2\pi}\,\vec{\mu}_{\tau}(s)\cdot\int\limits_{C(s)}\ten{\delta\fib{R}}\,\vec{n}\times\bigg(\mtx{\ten{F}}_{c}-\fib{\ten{R}}\bigg)\vec{n} \d C \\
&+
\frac{1}{2\pi}\,\mu_{n}(s)\int\limits_{C(s)}\vec{n}\tp\ten{\delta\fib{R}}\tp\bigg(\mtx{\ten{F}}_{c}-\fib{\ten{R}}\bigg)\vec{n} \d C +  \O(r^2)
\\
=&
\fib{\ten{R}}\tp\vec{\delta\mu}_{\tau}(s)\cdot\frac{1}{2\pi}\!\int\limits_{C(s)}\vec{n}\times\left(\fib{\ten{R}}\tp\mtx{\ten{F}}_{c}\,\vec{n}\right) \d C \\
&+
\delta\mu_{n}(s)\,\left(\frac{1}{2\pi}\!\int\limits_{C(s)}\vec{n}\tp\fib{\ten{R}}\tp\mtx{\ten{F}}_{c}\,\vec{n} \d C-1\right)  \\
&+
\frac{1}{2\pi}\,\vec{\mu}_{\tau}(s)\cdot\int\limits_{C(s)}\ten{\delta\fib{R}}\,\vec{n}\times\mtx{\ten{F}}_{c}\,\vec{n} \d C \\
&+
\frac{1}{2\pi}\,\mu_{n}(s)\int\limits_{C(s)}\vec{n}\tp\ten{\delta\fib{R}}\tp\mtx{\ten{F}}_{c}\vec{n} \d C \\
&-
\frac{1}{\abs{C}}\!\int\limits_{C(s)}\vec{\tilde{\mu}}\tp\,\ten{\delta\fib{R}}\,\left(\theta^{\alpha}\vec{D}_{\alpha}(s)\right)\d C\d s  +  \O(r^2)
\end{aligned}
\end{equation}
That is,
\begin{equation}\label{eq:tildePi_C}
\begin{aligned}
\delta\tilde{\Pi}_{C} 
&= \fib{\ten{R}}\tp\vec{\delta\mu}_{\tau}(s)\cdot\frac{1}{2\pi}\!\int\limits_{C(s)}\vec{n}\times\left(\fib{\ten{R}}\tp\mtx{\ten{F}}_{c}\,\vec{n}\right) \d C \\
&+
\delta\mu_{n}(s)\,\left(\frac{1}{2\pi}\!\int\limits_{C(s)}\vec{n}\tp\fib{\ten{R}}\tp\mtx{\ten{F}}_{c}\,\vec{n} \d C-1\right)  \\
&+
\frac{1}{2\pi}\,\vec{\mu}_{\tau}(s)\cdot\int\limits_{C(s)}\ten{\delta\fib{R}}\,\vec{n}\times\mtx{\ten{F}}_{c}\,\vec{n} \d C \\
&+
\frac{1}{2\pi}\,\mu_{n}(s)\int\limits_{C(s)}\vec{n}\tp\ten{\delta\fib{R}}\tp\mtx{\ten{F}}_{c}\,\vec{n} \d C +  \O(r^2).
\end{aligned}
\end{equation}
%The last two terms go to the equation~\eqref{eq:sys:moments} as the interface torque term.
\rev{TODO: write the results as lemmas, and put all the arithmetics to the appendix.  }

Let us remark that for any matrix $\ten{A}$ one has:
\begin{equation}\label{eq:integral2condition}
\begin{aligned}
\int\limits_{0}^{2\pi} \vec{n}\times\bigl(\ten{A}\,\vec{n} \bigr)\,\d\theta
&= \int\limits_{0}^{2\pi}\begin{vmatrix} \vec{D}_1 & \vec{D}_2 & \vec{D}_3 \\ 
\cos\theta & \sin\theta & 0 \\
\vec{D}_1\tp\ten{A}\vec{n} & \vec{D}_2\tp\ten{A}\vec{n} & \vec{D}_3\tp\ten{A}\vec{n}
\end{vmatrix}\,\d\theta 
\\
&= \left[\vec{D}_1,  \vec{D}_2,  \vec{D}_3\right]\cdot
\int\limits_{0}^{2\pi}
\begin{bmatrix} 
\vec{D}_3\tp\ten{A}\vec{n}\,\sin\theta \\ 
-\vec{D}_3\tp\ten{A}\vec{n}\,\cos\theta  \\
\vec{D}_2\tp\ten{A}\vec{n}\,\cos\theta - \vec{D}_1\tp\ten{A}\vec{n}\,\sin\theta
\end{bmatrix}\,\d\theta
\\
&= \pi\left[\vec{D}_1,  \vec{D}_2,  \vec{D}_3\right]\cdot\begin{bmatrix} 
\vec{D}_3\tp\ten{A}\vec{D}_2 \\ 
-\vec{D}_3\tp\ten{A}\vec{D}_1 \\
\vec{D}_2\tp\ten{A}\vec{D}_1 - \vec{D}_1\tp\ten{A}\vec{D}_2
\end{bmatrix}
\end{aligned}
\end{equation}	
Thus, in \eqref{eq:tildePi_C}
\begin{equation}
\frac{1}{2\pi}\!\int\limits_{C(s)}\vec{n}\times\left(\fib{\ten{R}}\tp\mtx{\ten{F}}_{c}\,\vec{n}\right) \d C
=
\frac{1}{2}\,\left[\vec{D}_1,  \vec{D}_2,  \vec{D}_3\right]\cdot\begin{bmatrix} 
\vec{d}_3\tp\mtx{\ten{F}_{c}}\,\vec{D}_2 \\ 
-\vec{d}_3\tp\mtx{\ten{F}_{c}}\,\vec{D}_1 \\
\vec{d}_2\tp\mtx{\ten{F}_{c}}\,\vec{D}_1 - \vec{d}_1\tp\mtx{\ten{F}_{c}}\,\vec{D}_2
\end{bmatrix}.
\end{equation}

%\begin{equation}
%\begin{aligned}
%\frac{1}{\abs{C}}\!\int\limits_{C(s)}\vec{\delta\tilde{\mu}}\cdot\bigg(\mtx{\x}-\theta^{\alpha}\vec{d}_{\alpha}\bigg) \d C
%&=
%\frac{1}{2}\,\vec{\delta\mu}_{\tau}(s)\cdot\begin{bmatrix} 
%\vec{d}_3\tp\mtx{\ten{F}_{c}}\vec{D}_2 \\ 
%-\vec{d}_3\tp\mtx{\ten{F}_{c}}\vec{D}_1 \\
%\vec{d}_2\tp\mtx{\ten{F}_{c}}\vec{D}_1 - \vec{d}_1\tp\mtx{\ten{F}_{c}}\vec{D}_2
%\end{bmatrix} \\
%&+
%\delta\mu_{n}(s)\,\left( \frac{1}{2}\,\vec{d}_1\tp\mtx{\ten{F}_{c}}\vec{D}_1 + \frac{1}{2}\,\vec{d}_2\tp\mtx{\ten{F}_{c}}\vec{D}_2 - 1\right)  \\
%&+
%\frac{1}{2\pi r}\,\vec{\mu}_{\tau}(s)\cdot\int\limits_{C(s)}\ten{\delta\fib{R}}\left(\theta^{\alpha}\vec{D}_{\alpha}(s)\right)\times\bigg(\mtx{\ten{F}_{c}}\fib{\ten{R}}\tp-\ten{\Id}\bigg)\vec{n} \d C \\
%&+
%\frac{1}{2\pi r}\,\mu_{n}(s)\int\limits_{C(s)}\left(\theta^{\alpha}\vec{D}_{\alpha}(s)\right)\tp\ten{\delta\fib{R}}\tp\bigg(\mtx{\ten{F}_{c}}\fib{\ten{R}}\tp-\ten{\Id}\bigg)\vec{n} \d C +  \O(r^2)
%\end{aligned}
%\end{equation}


Given a thin enough fiber of small radius~$r$, we neglect the higher order in $r$ terms in the expansion.
Thus, \eqref{eq:red_pb:pos_cond} leads to~\eqref{eq:phi1}.
\rev{However, \eqref{eq:red_pb:rot_cond_2} does not leads to \eqref{eq:phi2} (see the following remark). }

\begin{remark}
	In order to obtain condition~\eqref{eq:phi2}, one has to consider a spherical integral in~\eqref{eq:integral2condition} instead with the normal
	\begin{equation}\label{key}
		\vec{n} = \vec{D}_1\,\cos\theta\sin\phi + \vec{D}_2\,\sin\theta\sin\phi + \vec{D}_3\,\cos\phi.
	\end{equation}
	
	\begin{equation}
	\begin{aligned}
	\int\limits_{0}^{2\pi}\int\limits_{-\pi}^{\pi} \vec{n}\times\bigl(\ten{A}\,\vec{n} \bigr)\,\d\theta\d\phi
	&= \int\limits_{0}^{2\pi}\begin{vmatrix} \vec{D}_1 & \vec{D}_2 & \vec{D}_3 \\ 
	\cos\theta\sin\phi & \sin\theta\sin\phi & \cos\phi \\
	\vec{D}_1\tp\ten{A}\vec{n} & \vec{D}_2\tp\ten{A}\vec{n} & \vec{D}_3\tp\ten{A}\vec{n}
	\end{vmatrix}\,\d\theta 
	\\
	&= \left[\vec{D}_1,  \vec{D}_2,  \vec{D}_3\right]\cdot
	\int\limits_{0}^{2\pi}
	\begin{bmatrix} 
	\vec{D}_3\tp\ten{A}\vec{n}\,\sin\theta\sin\phi - \vec{D}_2\tp\ten{A}\vec{n}\,\cos\phi\\ 
	-\vec{D}_3\tp\ten{A}\vec{n}\,\cos\theta\sin\phi  + \vec{D}_1\tp\ten{A}\vec{n}\,\cos\phi\\
	\vec{D}_2\tp\ten{A}\vec{n}\,\cos\theta\sin\phi - \vec{D}_1\tp\ten{A}\vec{n}\,\sin\theta\sin\phi
	\end{bmatrix}\,\d\theta
	\\
	&=
	\pi\left[\vec{D}_1,  \vec{D}_2,  \vec{D}_3\right]\cdot\begin{bmatrix} 
	\vec{D}_3\tp\ten{A}\vec{D}_2 - \vec{D}_2\tp\ten{A}\vec{D}_3 \\ 
	-\vec{D}_3\tp\ten{A}\vec{D}_1 + \vec{D}_1\tp\ten{A}\vec{D}_3\\
	\vec{D}_2\tp\ten{A}\vec{D}_1 - \vec{D}_1\tp\ten{A}\vec{D}_2	
	\end{bmatrix} \\
	&=
	2\pi\,\left[\vec{D}_1,  \vec{D}_2,  \vec{D}_3\right]\cdot\axl\left(\left[\vec{D}_1,  \vec{D}_2,  \vec{D}_3\right]\tp\ten{A}\left[\vec{D}_1,  \vec{D}_2,  \vec{D}_3\right]\cdot\right)
	\end{aligned}
	\end{equation}	
	
%	\begin{equation}
%	\begin{aligned}
%	\frac{1}{2}\,
%	\begin{bmatrix} 
%	\vec{D}_3\tp\fib{\ten{R}}\tp\mtx{\ten{F}_{c}}\vec{D}_2 - \vec{D}_2\tp\fib{\ten{R}}\tp\mtx{\ten{F}_{c}}\vec{D}_3 \\ 
%	-\vec{D}_3\tp\fib{\ten{R}}\tp\mtx{\ten{F}_{c}}\vec{D}_1 + \vec{D}_1\tp\fib{\ten{R}}\tp\mtx{\ten{F}_{c}}\vec{D}_3\\
%	\vec{D}_2\tp\fib{\ten{R}}\tp\mtx{\ten{F}_{c}}\vec{D}_1 - \vec{D}_1\tp\fib{\ten{R}}\tp\mtx{\ten{F}_{c}}\vec{D}_2
%	\end{bmatrix}
%	&=
%	\frac{1}{2}\,
%	\begin{bmatrix} 
%	\vec{d}_3\tp\mtx{\ten{F}_{c}}\vec{D}_2 - \vec{d}_2\tp\mtx{\ten{F}_{c}}\vec{D}_3 \\ 
%	-\vec{d}_3\tp\mtx{\ten{F}_{c}}\vec{D}_1 + \vec{d}_1\tp\mtx{\ten{F}_{c}}\vec{D}_3\\
%	\vec{d}_2\tp\mtx{\ten{F}_{c}}\vec{D}_1 - \vec{d}_1\tp\mtx{\ten{F}_{c}}\vec{D}_2
%	\end{bmatrix}
%	\\
%	&=
%	\axl\big(\left[\vec{d}_1,  \vec{d}_2,  \vec{d}_3\right]\tp\mtx{\ten{F}_{c}}\left[\vec{D}_1,  \vec{D}_2,  \vec{D}_3\right]\big)
%	\end{aligned}
%	\end{equation}	
	
	\begin{equation}
	\begin{aligned}
	skew\big(\left[\vec{D}_1,  \vec{D}_2,  \vec{D}_3\right]\tp\fib{\ten{R}}\tp\mtx{\ten{F}_{c}}\left[\vec{D}_1,  \vec{D}_2,  \vec{D}_3\right]\big)
	&=
	\left[\vec{D}_1,  \vec{D}_2,  \vec{D}_3\right]\tp\, skew(\fib{\ten{R}}\tp\mtx{\ten{F}_{c}}) \,\left[\vec{D}_1,  \vec{D}_2,  \vec{D}_3\right]
	\end{aligned}
	\end{equation}	
\end{remark}




\paragraph{Total system.}
Finally, from~\eqref{eq:Euler-Lagrange}, we obtain the coupled matrix/fiber system for the unknowns $\mtx{\x}\in\HS_{M}(\Omega_{M})$, $\fib{\vec{\varphi}}\in\HS_{\vec{\fib{\varphi}}}([0,L])$, $\fib{\ten{R}}\in\HS_{\fib{\ten{R}}}([0,L])$, $\vec{\bar{\mu}}\in\HS_{\vec{\fib{\varphi}}}^\prime([0,L])$, $\vec{\tilde{\mu}}\in\HS_{\tilde{\mu}}(\Gamma)$:
\begin{align}\label{eq:tot_system}
&\int\limits_{\Omega_{M}} \drv{\Psi_{M}}{\ten{F}}:\nabla\vec{\delta\mtx{x}} \d V
+
%\int\limits_{\Omega_{M}} \!\!\vec{f}_{vol}\cdot\vec{\delta\mtx{x}} \d V
%+
\int\limits_{\partial\Omega_{N}} \!\!\vec{t}_{ext}\cdot\vec{\delta\mtx{x}} \d S
+
\int\limits_{\Gamma}\left(\vec{\bar{\mu}} + \vec{\tilde{\mu}}\right)\cdot \vec{\delta \mtx{x}} \d S
= 0, 
\\
&\int\limits_{0}^{L}\drv{\Psi_{F}}{\fib{\vec{\varphi}}^{\prime}}\cdot\vec{\delta\fib{\varphi}}^{\prime}\, \d s
%+
%\int\limits_{0}^{L} \vec{\bar{f}}_{vol}\cdot\vec{\delta\fib{\varphi}} \d s
-
\abs{C}\!\int\limits_{0}^{L}\vec{\bar{\mu}} \cdot \vec{\delta\fib{\varphi}}\d s
-
\abs{A}\!\!\sum_{s\in\{0,L\}} \vec{\bar{\mu}}_{0,L}(s) \cdot\vec{\delta\fib{\varphi}}(s)
= 0,
\\	
&\int\limits_{0}^{L}\drv{\Psi_{F}}{\fib{\ten{R}}}:\ten{\delta\fib{R}}\, \d s + \int\limits_{0}^{L}\int\limits_{C(s)}\vec{\tilde{\mu}}\tp\,\ten{\delta\fib{R}}\;\theta^{\alpha}\vec{D}_{\alpha}\d C\d s +
\int\limits_{A_{0,L}}\vec{\tilde{\mu}}_{0,L}\tp\,\ten{\delta\fib{R}}\;\theta^{\alpha}\vec{D}_{\alpha}\d A
= 0,  \label{eq:sys:moments}
\\
&\int\limits_{0}^{L}\vec{\delta\bar{\mu}} \cdot\left(\fib{\vec{\varphi}}(s)-\frac{1}{\abs{C}}\!\int\limits_{C(s)} \mtx{\x}\d C\right)\d s
= 0,
\qquad 
\fib{\vec{\varphi}}(s_{0,L}) = \frac{1}{\abs{A}}\!\int\limits_{A_{0,L}} \mtx{\x}\d A,
%\qquad
%\fib{\vec{\varphi}}(L) = \frac{1}{\abs{A}}\!\!\int\limits_{A(L)} \mtx{\x}&\d A,
\\
&\frac{1}{\abs{C}}\!\int\limits_{\partial\Omega_{F, 3}}\vec{\delta\tilde{\mu}}\cdot\bigg(\mtx{\x}-\theta^{\alpha}\vec{d}_{\alpha}\bigg) \d S
=0,
\qquad
\frac{1}{\abs{A}}\!\int\limits_{A_{0,L}}\!\!\vec{\delta\tilde{\mu}}_{0,L}\cdot\bigg(\mtx{\x}-\theta^{\alpha}\vec{d}_{\alpha}\bigg)\d A
=0,
\end{align}
for all $\vec{\delta \mtx{x}}\in\HS_{M}(\Omega_{M})$, $\vec{\delta\fib{\varphi}}\in\HS_{\vec{\fib{\varphi}}}([0,L])$, $\ten{\delta \fib{R}}\in\HS_{\ten{\fib{R}}}([0,L])$, $\vec{\delta\bar{\mu}}\in\HS_{\vec{\fib{\varphi}}}^\prime([0,L])$, $\vec{\delta\tilde{\mu}}\in\HS_{\tilde{\mu}}(\Gamma)$.
%completed with the constitutive laws
%\begin{align}\label{key}
%\ten{P}_{M} & = \drv{\Psi_{M}}{\nabla\mtx{\x}}\left(\nabla\mtx{\x}\right),
%&
%\vec{N} &= \drv{\Psi_{F}}{\left(\drv{\fib{\vec{\varphi}}}{s}\right)}\left(\drv{\fib{\vec{\varphi}}}{s}, \fib{\ten{R}}\right),
%&
%\ten{Q} &= \drv{\Psi_{F}}{\fib{\ten{R}}}\left(\drv{\fib{\vec{\varphi}}}{s}, \fib{\ten{R}}\right).
%\end{align}
%which are defined by the form of the free energy density in~\eqref{eq:fib:FreeEnergy}.



Two kind of errors occurs: due continuation of matrix solution inside the fiber domain and due to truncation of expansion w.r.t.~$r$.
\rev{TO DO: Estimate bounds for this errors. }


%Assume that $\HS_{\tilde{\mu}} = \{ \vec{\tilde{\mu}} \;\big|\; \vec{\tilde{\mu}}(\X) = \sum_{i=1}^{3}\tilde{\mu}_i(s)\,\vec{v}_i(\theta), \; \tilde{\mu}_i\in\HS_{\vec{\fib{\varphi}}}^\prime([0,L]) \}$,
%where
%\begin{equation}\label{key}
%	\vec{v}_i(\theta) = \ten{L}_i\cdot
%	\left[\begin{array}{l}
%		\cos\theta\\
%		\sin\theta\\
%		0
%	\end{array}\right]
%\end{equation}
%Then
%
%\begin{align}\label{key}
%\vec{d}_3\tp\ten{F}\vec{D}_{2} &= 0,\\ 
%\vec{d}_{3}\tp\ten{F}\vec{D}_{1} &= 0, \\
%\vec{d}_{2}\tp\ten{F}\vec{D}_{1} &= \vec{d}_1\tp\ten{F}\vec{D}_{2}.
%\end{align}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\begin{proposition}\label{prop:condensed_sys_avg}
%	If the function $\vec{\bar{u}}_{M}(s)=\int\limits_{C(s)} \mtx{\x}\d A$ lives in $\HS_{c}([0,L])$, then the Lagrange multipliers $\vec{\bar{\mu}}$ can be condensed, and the system~\eqref{eq:tot_system} thus reduces to	
%	\begin{multline}\label{eq:condensed_sys_avg}
%	\int\limits_{\Omega_{M}} \ten{P}_{M}:\nabla\vec{\delta u}_{M} \d V 
%	+
%	\int\limits_{\Omega_{M}} \!\!\vec{f}_{vol}\cdot\vec{\delta u}_{M} \d V
%	+
%	\int\limits_{\partial\Omega_{N}} \!\!\vec{t}_{ext}\cdot\vec{\delta u}_{M} \d V
%	+
%	\int\limits_{\Gamma}\vec{\tilde{\mu}}\cdot \vec{\delta u}_{M} \d V +\\
%	+
%	\int\limits_{0}^{L}\left(\vec{\bar{f}}_{vol}-\vec{N}^{\prime}\right) \cdot\left(\frac{1}{\abs{C}}\!\!\int\limits_{C(s)} \!\!\vec{\delta u}_{M}\d C\right)\d s
%	+
%	\!\!\!\!\sum_{s\in\{0,L\}} \!\!\vec{N}(s) \cdot\left(\frac{1}{\abs{A}}\!\!\int\limits_{A(s)} \!\!\vec{\delta u}_{M}\d A\right)
%	= 0, 
%	\\	
%	\int\limits_{0}^{L}\ten{Q}:\ten{\delta\fib{R}}\, \d s + \int\limits_{0}^{L}\int\limits_{C(s)}\vec{\tilde{\mu}}\tp\,\ten{\delta\fib{R}}\,\left(\theta^{\alpha}\vec{D}_{\alpha}(s)\right)\d C\d s +
%	\int\limits_{A_{0,L}}\vec{\tilde{\mu}}_{0,L}\tp\,\ten{\delta\fib{R}}\,\left(\theta^{\alpha}\vec{D}_{\alpha}(s)\right)\d A
%	= 0,
%	\\
%	\int\limits_{\partial\Omega_{F, 3}}\vec{\delta\tilde{\mu}}\cdot\bigg(\mtx{\x}-\theta^{\alpha}\fib{\ten{R}}\vec{D}_{\alpha}\bigg) \d V
%	=0,
%	\qquad
%	\int\limits_{\partial\Omega_{F, 1/2}}\!\!\!\!\vec{\delta\tilde{\mu}}_{0,L}\cdot\bigg(\mtx{\x}-\theta^{\alpha}\fib{\ten{R}}\vec{D}_{\alpha}\bigg)\d A
%	=0
%	\end{multline}
%	for all $\vec{\delta u}_{M}\in\HS_{M}(\Omega_{M})$, $\ten{\delta R}\in\HS_{\ten{R}}(\Gamma)$, $\vec{\delta\tilde{\mu}}\in\HS_{\tilde{\mu}}([0,L])$, with the constitutive laws
%	
%	\begin{align}\label{key}
%	\ten{P}_{M} & = \drv{\Psi_{M}}{\nabla\mtx{\x}}\left(\nabla\mtx{\x}\right),
%	&
%	\vec{N} &= \drv{\Psi_{F}}{\fib{\vec{\varphi}}^{\prime}}\left(\fib{\vec{\varphi}}^{\prime}, \fib{\ten{R}}\right),
%	&
%	\ten{Q} &= \drv{\Psi_{F}}{\fib{\ten{R}}}\left(\fib{\vec{\varphi}}^{\prime}, \fib{\ten{R}}\right),
%	&\text{where }\;
%	\fib{\vec{\varphi}}(s) = \frac{1}{\abs{C}}\!\int\limits_{C(s)} \mtx{\x}\d C.
%	\end{align}
%\end{proposition}

%\begin{rmk}
%	For example, if $\HS_{M}(\Omega_{M}) = \H{1}(\Omega_{M})$, then $\mtx{\x}\big|_{\Gamma}\in\H{\frac{1}{2}}(\Gamma)$
%\end{rmk}

%\begin{proposition}\label{prop:continuation}
%	Let us consider a continuation of $\mtx{\x}$ inside the subdomain~$\Omega_{F}$, solving a supplementary problem
%	\begin{equation}\label{eq:suppl_pb}
%	\int\limits_{\Omega_{F}}\ten{P}_{M}(\nabla\mtx{\x}):\nabla\vec{\delta u}_{M}\d V
%	+
%	\int\limits_{\partial\Omega_{F}}\vec{\mu}\cdot\vec{\delta u}_{M}\d V
%	+
%	\int\limits_{\Omega_{F}}\vec{g}\cdot\vec{\delta u}_{M}\d V
%	= 0
%	\end{equation}
%	Then, the system~\eqref{eq:condensed_sys_avg} can be written as
%	\begin{align}\label{eq:alt_sys}
%	\int\limits_{\Omega} \ten{P}_{M}:\nabla\vec{\delta u}_{M} \d V 
%	+
%	\int\limits_{\Omega_{M}} \!\!\vec{f}_{vol}\cdot\vec{\delta u}_{M} \d V
%	+&
%	\int\limits_{\partial\Omega_{N}} \!\!\vec{t}_{ext}\cdot\vec{\delta u}_{M} \d V
%	+
%	\int\limits_{\Omega_{F}}\vec{g}\cdot\vec{\delta u}_{M}\d V
%	= 0, \\
%	\int\limits_{\Omega_{F}}\ten{P}_{M}:\nabla\vec{\delta u}_{M}\d V
%	+
%	\int\limits_{\Omega_{F}}\vec{g}\cdot\vec{\delta u}_{M}\d V
%	+
%	\int\limits_{0}^{L}\left(\vec{\bar{f}}_{vol}-\vec{N}^{\prime}\right) \cdot&\left(\frac{1}{\abs{C}}\!\!\int\limits_{C(s)} \!\!\vec{\delta u}_{M}\d C\right)\d s
%	+
%	\!\!\!\!\sum_{s\in\{0,L\}} \!\!\vec{N}(s) \cdot\left(\frac{1}{\abs{A}}\!\!\int\limits_{A(s)} \!\!\vec{\delta u}_{M}\d A\right)
%	= 0, \\	
%	\int\limits_{0}^{L}\ten{Q}:\ten{\delta R}\, \d s &= 0.
%	\end{align}
%	From the second equation of this system, we can notice that
%	\begin{equation}\label{key}
%	\int\limits_{A(s)}\vec{g}\d A
%	= \int\limits_{A(s)}\div\ten{P}_{M}\d A
%	= \int\limits_{C(s)}\ten{P}_{M}\,\vec{n}\d C
%	= -\int\limits_{C(s)}\vec{\mu}\d C
%	= -\vec{\lambda}(s)
%	= \vec{N}^{\prime}-\vec{\bar{f}}_{vol}.
%	\end{equation}
%	\rev{Should we develop this ? Or just cut $\Omega_{F}$ from $\Omega$ is ok ?}
%\end{proposition}




%\subsection{1D-beam/3D-matrix system. Rigid fiber cross-section}
%
%\input{tikz/fiber3D/fiber3D}
%
%%\paragraph{Rigid fiber cross-section.} 
%
%Let us now consider the case of rigid cross-section fiber.
%That is, $\vec{u}(\X)\bigr|_{\Omega_{F}}=\vec{u}(s)$ and $\fib{\ten{R}}(\X)=\fib{\ten{R}}(s)$, where $s\in[0,L]$ is the arc-length of the fiber centerline.
%In what follows, without loss of generality, we assume that $\abs{\drv{\X}{s}}=1$ in $\Omega_{F}$.
%In other words, we have $\fib{\x}\in\HS_{F}([0,L])$, $\fib{\ten{R}}\in\HS_{R}([0,L])$.
%For any test function of the form $\vec{\delta\fib{\varphi}}(\X) = \vec{\phi}(s)$, we have
%\begin{align}\label{eq:fib:N}
%\int\limits_{\Omega_{F}} \ten{P}_{F}:\nabla\vec{\delta\fib{\varphi}} \,\rho_{F}\!\d V
%= \int\limits_{0}^{L}\int\limits_{A(s)} \ten{P}_{F}:\left(\vec{\phi}^{\prime}\,\vec{e}_L\tp\right) \,\rho_{F}\!\d A \d s
%= \int\limits_{0}^{L}\underbrace{\left(\int\limits_{A(s)} \ten{P}_{F}\cdot\vec{e}_L\,\rho_{F}\!\d A\right)}_{\vec{N}(s)}\cdot\drv{}{s}\vec{\phi}(s)\, \d s,
%\end{align}
%where $A(s)$ denotes the fiber cross-section with coordinate~$s$, and $\vec{e}_L$ is the fiber centerline director in the reference frame.
%We also have (see Figure~\ref{fig:fiber3D_ref}):
%\begin{align}\label{eq:fib:f_interact}
%\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\mu}\cdot\vec{\delta\fib{\varphi}}\d V
%&=
%\int\limits_{\partial\Omega_{F,1/2}} \vec{\mu}\cdot\vec{\delta\fib{\varphi}}\d V
%+
%\int\limits_{\partial\Omega_{F,3}} \vec{\mu}\cdot\vec{\delta\fib{\varphi}}\d V\\
%&=
%\sum_{\hat{s}\in\{0,L\}} \underbrace{\left(\int\limits_{A(\hat{s})}\vec{\mu}\d A\right)}_{\vec{\hat{\lambda}}_{0}, \vec{\hat{\lambda}}_{L}} \cdot\vec{\phi}(\hat{s})
%+
%\int\limits_{0}^{L}\underbrace{\left(\int\limits_{C(s)}\vec{\mu}\d A\right)}_{\vec{\lambda}(s)} \cdot\vec{\phi}(s)\,\d s,
%\end{align}
%where $C(s)$ denotes the circumference of the fiber cross-section with coordinate~$s$.
%Here, $\vec{\hat{\lambda}}_{0}$ and $\vec{\hat{\lambda}}_{L}$ are the resulting matrix action forces applied respectively to $\Omega_{F,1}$ and $\Omega_{F,2}$, while $\vec{\lambda}(s)$ is the resulting line load imposed by the matrix to the cross-section~$s$.
%Note that $\vec{\hat{\lambda}}$ and $\vec{\lambda}$ have distinct units.
%Thus, we can write
%\begin{equation}\label{key}
%	\int\limits_{0}^{L}\vec{N}\cdot\vec{\phi}^{\prime}\, \d s
%	-
%	\int\limits_{0}^{L}\vec{\lambda}\cdot\vec{\phi}\,\d s
%	-
%	\sum_{\hat{s}\in\{0,L\}} \vec{\hat{\lambda}}_{\hat{s}}\cdot\vec{\phi}(\hat{s})
%	+
%	\int\limits_{0}^{L} \vec{\bar{f}}_{vol}\cdot\vec{\phi} \d s
%	= 0,
%\end{equation}
%where $\vec{\bar{f}}_{vol}(s) = \int_{A(s)}\vec{f}_{vol}\,\rho_{F}\!\d A$.
%Moreover, for any test function of the form $\ten{\delta\fib{R}}(\X) = \ten{\Phi}(s)$, we have
%\begin{equation}
%\int\limits_{\Omega_{F}} \ten{G}_{F}:\ten{\delta\fib{R}} \,\rho_{F}\!\d V
%%= \int\limits_{0}^{L}\int\limits_{A(s)} \ten{G}_{F}:\left(\vec{\Phi}^{\prime}\,\vec{e}_L\tp\right) \d A \d s
%= \int\limits_{0}^{L}\underbrace{\left(\int\limits_{A(s)} \ten{G}_{F}\,\,\rho_{F}\!\d A\right)}_{\ten{Q}(s)}\cdot\ten{\Phi}(s)\, \d s.
%\end{equation}
%Hence, we obtain the fiber system
%\begin{gather}%\label{key}
%	\int\limits_{0}^{L}\vec{N}^{\prime}\cdot\vec{\phi}\, \d s
%	+
%	\int\limits_{0}^{L}\vec{\lambda}\cdot\vec{\phi}\,\d s
%	-
%	\int\limits_{0}^{L} \vec{\bar{f}}_{vol}\cdot\vec{\phi} \d s
%	= 0,\qquad	
%	\vec{N}(0) = \vec{\hat{\lambda}}_{0}, \qquad \vec{N}(L) = \vec{\hat{\lambda}}_{L},\\	
%	\int\limits_{0}^{L}\ten{Q}(s):\ten{\Phi}(s)\, \d s = 0.
%\end{gather}
%
%\paragraph{Lagrange multipliers.} For the Lagrange multipliers~$\vec{\mu}$, there are two alternatives:
%\begin{enumerate}
%	\item $\vec{\mu}\in\HS_{\mu}(\Omega_{M}\cap\Omega_{F})$,
%	\item $\vec{\mu}\in\HS_{\mu}([0,L])$, i.e. $\vec{\mu}$ is constant on $C(s)$, $s\in[0,L]$.
%\end{enumerate}
%Let us consider in what follows the last case in details.
%In this situation, we have
%\begin{align}\label{key}
%\!\!\!\!\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\delta\mu} \cdot(\mtx{\x}-\fib{\x})\d V
%&=
%\int\limits_{\partial\Omega_{F,3}} \vec{\delta\mu} \cdot(\mtx{\x}-\fib{\x})\d V
%+
%\int\limits_{\partial\Omega_{F,1/2}} \vec{\delta\mu} \cdot(\mtx{\x}-\fib{\x})\d V
%\\
%&=
%\abs{C}\!\int\limits_{0}^{L}\vec{\delta\mu} \cdot\left(\frac{1}{\abs{C}}\!\!\int\limits_{C(s)} \mtx{\x}\d C - \fib{\x}(s)\right)\d s
%+
%\abs{A}\!\!\sum_{s\in\{0,L\}} \vec{\delta\mu}(s) \cdot\left(\frac{1}{\abs{A}}\!\!\int\limits_{A(s)} \mtx{\x}\d A -\fib{\x}(\hat{s}) \right)\\
%&=
%\int\limits_{0}^{L}\vec{\delta\lambda} \cdot\left(\frac{1}{\abs{C}}\!\!\int\limits_{C(s)} \mtx{\x}\d C - \fib{\x}(s)\right)\d s
%+
%\sum_{s\in\{0,L\}} \vec{\delta\lambda}(s) \cdot\left(\frac{1}{\abs{A}}\!\!\int\limits_{A(s)} \mtx{\x}\d A -\fib{\x}(\hat{s}) \right),
%\intertext{and}
%\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\mu} \cdot\vec{\delta u}_{M} \d V
%&=
%\int\limits_{0}^{L}\vec{\lambda} \cdot\left(\frac{1}{\abs{C}}\!\!\int\limits_{C(s)} \vec{\delta u}_{M}\d C\right)\d s
%+
%\sum_{s\in\{0,L\}} \!\!\!\vec{\lambda}(s) \cdot\left(\frac{1}{\abs{A}}\!\!\int\limits_{A(s)} \vec{\delta u}_{M}\d A\right).
%\end{align}
%
%\paragraph{Total system.}
%Thus, we obtain the coupled matrix/fiber system for the unknowns $\mtx{\x}\in\HS_{M}(\Omega_{M})$, $\fib{\x}\in\HS_{F}([0,L])$, $\ten{R}\in\HS_{\ten{R}}([0,L])$, $\ten{\lambda}\in\HS_{F}^\prime([0,L])$:
%\begin{align}\label{eq:system3D}
%\int\limits_{\Omega_{M}} \ten{P}_{M}:\nabla\vec{\delta u}_{M} \,\rho_{M}\!\d V 
%+
%\int\limits_{\Omega_{M}} \!\!\vec{f}_{vol}\cdot\vec{\delta u}_{M} \,\rho_{M}\!\d V
%+&
%\int\limits_{\partial\Omega_{N}} \!\!\vec{t}_{ext}\cdot\vec{\delta u}_{M} \d V \\
%+
%\int\limits_{0}^{L}\vec{\lambda} \cdot&\left(\frac{1}{\abs{C}}\!\!\int\limits_{C(s)} \!\!\vec{\delta u}_{M}\d C\right)\d s
%+
%\!\!\!\!\sum_{s\in\{0,L\}} \!\!\vec{\lambda}(s) \cdot\left(\frac{1}{\abs{A}}\!\!\int\limits_{A(s)} \!\!\vec{\delta u}_{M}\d A\right)
%= 0, \\
%\int\limits_{0}^{L}\vec{N}^{\prime}\cdot\vec{\delta\fib{\varphi}}\, \d s
%+
%\int\limits_{0}^{L}\vec{\lambda}\cdot\vec{\delta\fib{\varphi}}\,\d s
%-
%\int\limits_{0}^{L} \vec{\bar{f}}_{vol}\cdot\vec{\delta\fib{\varphi}} \d s
%&= 0,
%\qquad
%\vec{N}(0) = \vec{\hat{\lambda}}_{0}, \qquad \vec{N}(L) = \vec{\hat{\lambda}}_{L}, \\	
%\int\limits_{0}^{L}\ten{Q}:\ten{\delta R}\, \d s &= 0, \\
%\int\limits_{0}^{L}\vec{\delta\lambda} \cdot\left(\fib{\x}(s)-\frac{1}{\abs{C}}\!\!\int\limits_{C(s)} \mtx{\x}\d C\right)\d s
%&= 0,
%\qquad 
%\fib{\x}(0) = \frac{1}{\abs{A}}\!\!\int\limits_{A(0)} \mtx{\x}\d A,
%\qquad
%\fib{\x}(L) = \frac{1}{\abs{A}}\!\!\int\limits_{A(L)} \mtx{\x}\d A,
%\end{align}
%for all $\vec{\delta u}_{M}\in\HS_{M}(\Omega_{M})$, $\vec{\delta\fib{\varphi}}\in\HS_{F}([0,L])$, $\ten{\delta R}\in\HS_{\ten{R}}([0,L])$, $\ten{\delta\lambda}\in\HS_{F}^\prime([0,L])$,
%completed with fiber constitutive laws in~$[0,L]$:
%\begin{align}\label{key}
%\vec{N} &= \vec{N}(\nabla\fib{\x}, \fib{\ten{R}}), \\	
%\ten{Q} &= \ten{Q}(\nabla\fib{\x}, \fib{\ten{R}}),
%\end{align}
%which are defined by the form of the free energy density in~\eqref{eq:fib:FreeEnergy}.
%
%\begin{proposition}\label{prop:condensed_sys_avg}
%	If the function $\vec{\bar{u}}_{M}(s)=\int\limits_{A(s)} \mtx{\x}\d A$ lives in $\HS_{F}([0,L])$, then the Lagrange multipliers $\vec{\lambda}$ and $\vec{\hat{\lambda}}$ can be condensed, and the system~\eqref{eq:system3D} thus reduces to	
%	\begin{align}\label{eq:condensed_sys_avg}
%	\int\limits_{\Omega_{M}} \ten{P}_{M}:\nabla\vec{\delta u}_{M} \,\rho_{M}\!\d V 
%	+
%	\int\limits_{\Omega_{M}} \!\!\vec{f}_{vol}\cdot\vec{\delta u}_{M} \,\rho_{M}\!\d V
%	+&
%	\int\limits_{\partial\Omega_{N}} \!\!\vec{t}_{ext}\cdot\vec{\delta u}_{M} \d V \\
%	+
%	\int\limits_{0}^{L}\left(\vec{\bar{f}}_{vol}-\vec{N}^{\prime}\right) \cdot&\left(\frac{1}{\abs{C}}\!\!\int\limits_{C(s)} \!\!\vec{\delta u}_{M}\d C\right)\d s
%	+
%	\!\!\!\!\sum_{s\in\{0,L\}} \!\!\vec{N}(s) \cdot\left(\frac{1}{\abs{A}}\!\!\int\limits_{A(s)} \!\!\vec{\delta u}_{M}\d A\right)
%	= 0, \\	
%	\int\limits_{0}^{L}\ten{Q}:\ten{\delta R}\, \d s &= 0,
%	\end{align}
%	for all $\vec{\delta u}_{M}\in\HS_{M}(\Omega_{M})$ and all $\ten{\delta R}\in\HS_{\ten{R}}([0,L])$, with the constitutive laws
%	\begin{gather}\label{key}
%	\vec{P}_{M} = \vec{P}_{M}(\nabla\mtx{\x})  \;\text{ in }\Omega_{M},	
%	\intertext{and}
%	\vec{N} = \vec{N}(\nabla\fib{\x}, \fib{\ten{R}}) \;\text{ and }\;
%	\ten{Q} = \ten{Q}(\nabla\fib{\x}, \fib{\ten{R}}),
%	\quad\text{where }\quad
%	\fib{\x}(s) = \frac{1}{\abs{A}}\!\!\int\limits_{A(s)} \mtx{\x}\d A.
%	\end{gather}
%\end{proposition}
%
%\begin{proposition}\label{prop:continuation}
%	Let us consider a continuation of $\mtx{\x}$ inside the subdomain~$\Omega_{F}$, solving a supplementary problem
%	\begin{equation}\label{eq:suppl_pb}
%	\int\limits_{\Omega_{F}}\ten{P}_{M}(\nabla\mtx{\x}):\nabla\vec{\delta u}_{M}\d V
%	+
%	\int\limits_{\partial\Omega_{F}}\vec{\mu}\cdot\vec{\delta u}_{M}\d V
%	+
%	\int\limits_{\Omega_{F}}\vec{g}\cdot\vec{\delta u}_{M}\d V
%	= 0
%	\end{equation}
%	Then, the system~\eqref{eq:condensed_sys_avg} can be written as
%	\begin{align}\label{eq:alt_sys}
%	\int\limits_{\Omega} \ten{P}_{M}:\nabla\vec{\delta u}_{M} \d V 
%	+
%	\int\limits_{\Omega_{M}} \!\!\vec{f}_{vol}\cdot\vec{\delta u}_{M} \d V
%	+&
%	\int\limits_{\partial\Omega_{N}} \!\!\vec{t}_{ext}\cdot\vec{\delta u}_{M} \d V
%	+
%	\int\limits_{\Omega_{F}}\vec{g}\cdot\vec{\delta u}_{M}\d V
%	= 0, \\
%	\int\limits_{\Omega_{F}}\ten{P}_{M}:\nabla\vec{\delta u}_{M}\d V
%	+
%	\int\limits_{\Omega_{F}}\vec{g}\cdot\vec{\delta u}_{M}\d V
%	+
%	\int\limits_{0}^{L}\left(\vec{\bar{f}}_{vol}-\vec{N}^{\prime}\right) \cdot&\left(\frac{1}{\abs{C}}\!\!\int\limits_{C(s)} \!\!\vec{\delta u}_{M}\d C\right)\d s
%	+
%	\!\!\!\!\sum_{s\in\{0,L\}} \!\!\vec{N}(s) \cdot\left(\frac{1}{\abs{A}}\!\!\int\limits_{A(s)} \!\!\vec{\delta u}_{M}\d A\right)
%	= 0, \\	
%	\int\limits_{0}^{L}\ten{Q}:\ten{\delta R}\, \d s &= 0.
%	\end{align}
%	From the second equation of this system, we can notice that
%	\begin{equation}\label{key}
%	\int\limits_{A(s)}\vec{g}\d A
%	= \int\limits_{A(s)}\div\ten{P}_{M}\d A
%	= \int\limits_{C(s)}\ten{P}_{M}\,\vec{n}\d C
%	= -\int\limits_{C(s)}\vec{\mu}\d C
%	= -\vec{\lambda}(s)
%	= \vec{N}^{\prime}-\vec{\bar{f}}_{vol}.
%	\end{equation}
%	\rev{Should we develop this ? Or just cut $\Omega_{F}$ from $\Omega$ is ok ?}
%\end{proposition}
%
%%\vspace{5ex}
%%On the other hand, for the matrix it holds
%%\begin{equation}\label{key}
%%\int\limits_{\Omega_{M}} \ten{S}_{M}:\ten{\delta \eps}_{M} \,\rho_{M}\!\d V 
%%+
%%\int\limits_{\Omega_{M}} \vec{f}_{vol}\cdot\vec{\delta u}_{M} \,\rho_{M}\!\d V
%%+
%%\int\limits_{\partial\Omega_{N}} \vec{t}_{ext}\cdot\vec{\delta u}_{M} \d V
%%+
%%\!\!\!\!\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\mu} \cdot\vec{\delta u}_{M} \d V
%%= 0
%%\end{equation}
%%For any $\vec{\delta u}_{M}$ such that $\vec{\delta u}_{M}\bigr|_{\Omega_{M}\cap\Omega_{F}} = \vec{\phi}(s)$, we have
%%\begin{equation}\label{key}
%%\int\limits_{\Omega_{M}} \ten{S}_{M}:\ten{\delta \eps}_{M} \,\rho_{M}\!\d V 
%%+
%%\int\limits_{\Omega_{M}} \vec{f}_{vol}\cdot\vec{\delta u}_{M} \,\rho_{M}\!\d V
%%+
%%\int\limits_{\partial\Omega_{N}} \vec{t}_{ext}\cdot\vec{\delta u}_{M} \d V
%%+
%%\int\limits_{\Omega}\left(\vec{\lambda}\,\delta_{(0,L)}(\X) + \sum_{\hat{s}\in\{0,L\}} \vec{\hat{\lambda}}_{\hat{s}}\,\delta_{\hat{s}}(\X)\right)\cdot\vec{\delta u}_{M}\d V
%%= 0,
%%\end{equation}
%%where $\delta_{s}(\X) = \delta(\X - \X_{s})$ is Dirac $\delta$-function ($\X_{s}$ being the point of $\Omega_{F}$ with line coordinate~$s$), and $\delta_{(0,L)}(\X)$ denotes Dirac $\delta$-function in the hyperspace orthogonal to $\vec{e}_L$.
%%
%%Thus, for $\vec{u}\in V = \{\vec{v}\in\HS(\Omega)\; : \; \vec{v}(\X)\bigr|_{\Omega_{F}}=\vec{v}(s)\}$, i.e. rigid cross-section fiber, the complete system looks like
%%\begin{align}\label{eq:system3D}
%%	\int\limits_{\Omega_{M}} \ten{P}_{M}:\nabla\vec{\delta u}_{M} \,\rho_{M}\!\d V 
%%	+
%%	\int\limits_{0}^{L}\vec{\lambda}\cdot\vec{\delta u}_{M}\d s
%%	+
%%	\!\!\!\sum_{\hat{s}\in\{0,L\}} \!\!\!\vec{\hat{\lambda}}_{\hat{s}}\cdot\vec{\delta u}_{M}(\hat{s})
%%	+
%%	\int\limits_{\Omega_{M}} \vec{f}_{vol}\cdot\vec{\delta u}_{M} \,\rho_{M}\!\d V
%%	+
%%	\int\limits_{\partial\Omega_{N}} \vec{t}_{ext}\cdot\vec{\delta u}_{M} \d V
%%	&= 0, \\
%%	\int\limits_{0}^{L}\vec{N}^{\prime}\cdot\vec{\phi}\, \d s
%%	+
%%	\int\limits_{0}^{L}\vec{\lambda}\cdot\vec{\phi}\,\d s
%%	-
%%	\int\limits_{0}^{L} \vec{\bar{f}}_{vol}\cdot\vec{\phi} \d s
%%	&= 0, \qquad \\
%%	\vec{N}(0) = \vec{\hat{\lambda}}_{0}, \qquad \vec{N}(L) &= \vec{\hat{\lambda}}_{L}, \\	
%%	\int\limits_{0}^{L}\ten{Q}(s):\ten{\Phi}(s)\, \d s &= 0, \\
%%	\int\limits_{0}^{L} \vec{\delta\lambda}\cdot(\mtx{\x}-\fib{\x})\d s &= 0,
%%\end{align}
%%completed with fiber constitutive laws in~$[0,L]$:
%%\begin{align}\label{key}
%%	\vec{N} &= \vec{N}(\nabla\fib{\x}, \fib{\ten{R}}), \\	
%%	\ten{Q} &= \ten{Q}(\nabla\fib{\x}, \fib{\ten{R}}),
%%\end{align}
%%which are defined by the form of the free energy density in~\eqref{eq:fib:FreeEnergy}.
%
%%\subsection{Moments coupling}
%%\input{sections/sec_MomentsCoupling}
%
%
%\subsection{1D-beam/3D-matrix system. Thin fiber}
%
%\rev{This section is to be corrected.}
%
%Let us consider the limit when the radius of fiber cross-section goes to zero, preserving however the fiber mass.
%When the radius of the fiber cross-section vanishes, we have $\Omega_{M}\cap\Omega_{F} = \Omega_{F}$ and thus $\Omega = \Omega_{M}$.
%Besides, in the limit case, all $\vec{\delta u}_{M}\bigr|_{\Omega_{M}\cap\Omega_{F}}$ and $\vec{\delta\fib{\varphi}}$ are of the form $\vec{\delta u}(\X)\bigr|_{\Omega_{M}\cap\Omega_{F}}=\vec{\phi}(s)$.
%
%Remark that while the radius~$r$ vanishes, the mass of the fiber remains constant, so the density grows, tending to the Dirac mass density.
%Thus, the integrals in~\eqref{eq:fib:N} and~\eqref{eq:fib:f_interact} do not vanish, since the forces implicitly contain the fiber density.
%
%Thus, from~\eqref{eq:system3D} we obtain the coupled $1$D-fiber/$3$D-matrix system for the unknowns $\mtx{\x}\in\HS_{M}(\Omega)$, $\fib{\x}\in\HS_{F}([0,L])$, $\ten{R}\in\HS_{\ten{R}}([0,L])$, $\ten{\lambda}\in\HS_{F}^\prime([0,L])$:
%\begin{equation}
%\begin{aligned}\label{eq:system1D/3D}
%\int\limits_{\Omega} \ten{P}_{M}(\nabla\mtx{\x}):\nabla\vec{\delta u}_{M} \d V 
%+
%\!\!\int\limits_{\Omega} \vec{f}_{vol}\cdot\vec{\delta u}_{M} \d V
%+
%\!\!\int\limits_{\partial\Omega_{N}} \vec{t}_{ext}\cdot\vec{\delta u}_{M} \d V
%+&
%\int\limits_{0}^{L}\vec{\lambda}\cdot\vec{\delta u}_{M}\d s
%+
%\!\!\sum_{s\in\{0,L\}} \!\!\!\!\vec{\hat{\lambda}}_{s}\cdot\vec{\delta u}_{M}(s)
%= 0, 
%%\quad \forall\;\vec{\delta u}_{M}\in\HS_{M}(\Omega),
%\\
%\int\limits_{0}^{L}\vec{N}^{\prime}\cdot\vec{\delta\fib{\varphi}}\, \d s
%+
%\int\limits_{0}^{L}\vec{\lambda}\cdot\vec{\delta\fib{\varphi}}\,\d s
%-
%\int\limits_{0}^{L} \vec{\bar{f}}_{vol}\cdot\vec{\delta\fib{\varphi}} \d s
%&= 0,
%%\quad \forall\;\vec{\phi}\in\HS_{F}([0,L]), 
%%\\
%\qquad
%\vec{N}(0) = \vec{\hat{\lambda}}_{0}, \qquad \vec{N}(L) = \vec{\hat{\lambda}}_{L}, 
%\\	
%\int\limits_{0}^{L}\ten{Q}:\ten{\delta R}\, \d s &= 0, 
%%\quad \forall\;\ten{\delta R}\in\HS_{\ten{R}}([0,L]),
%\\
%\int\limits_{0}^{L} \vec{\delta\lambda}\cdot(\mtx{\x}-\fib{\x})\d s &= 0,
%%\quad \forall\;\ten{\delta\lambda}\in\HS_{F}^\prime([0,L]),
%\end{aligned}
%\end{equation}
%for all $\vec{\delta u}_{M}\in\HS_{M}(\Omega)$, $\vec{\delta\fib{\varphi}}\in\HS_{F}([0,L])$, $\ten{\delta R}\in\HS_{\ten{R}}([0,L])$, $\ten{\delta\lambda}\in\HS_{F}^\prime([0,L])$.
%%\begin{multline}\label{key}
%%\int\limits_{\Omega} \ten{S}_{M}:\ten{\delta \eps}_{M} \d V
%%+
%%\int\limits_{\Omega}\vec{f}_{vol}\cdot\vec{\delta u} \d V
%%+
%%\int\limits_{\partial\Omega_{N}} \vec{t}_{ext}\cdot\vec{\delta u} \d V
%%+\\
%%+
%%\int\limits_{0}^L\left(\ten{\eps}_{F}:\ten{C}:\ten{\delta\eps}_{F} + \ten{\kappa}_{F}:\ten{D}:\ten{\delta\kappa}_{F}\right) \d s
%%+
%%\int\limits_{0}^L \vec{t}_{int} \cdot(\vec{\delta u}_{M}-\vec{\delta\fib{\varphi}})\d s
%%+
%%\int\limits_{0}^L \vec{\delta f}_{interact} \cdot(\mtx{\x}-\fib{\x})\d s
%%= 0
%%\end{multline}
%
%\begin{proposition}\label{prop:condensed_sys}
%%	The last equation defines the jump on~$\Omega_{F}$ between matrix/fiber displacements, $\mtx{\x}\in\HS_{M}(\Omega)$ and $\fib{\x}\in\HS_{F}([0, L])$ respectively.
%%	Let us consider the case when $\HS_{M}(\Omega)$, $\HS_{F}([0, L])$ and $\HS_{\vec{\lambda}}([0,L])$  are such that
%%	\begin{enumerate}[a)]
%%		\item $\vec{\lambda}\in\HS_{\vec{\lambda}}([0,L]) = \HS_{F}([0, L])$, \rev{That is "hard" coupling. So the case $\HS_{\vec{\lambda}}([0,L]) \ne \HS_{F}([0, L])$ should include "soft" couplings, I suppose.}
%%		\item $\forall \; \vec{v}\in\HS_{M}(\Omega), \quad \vec{v}\bigr|_{\Omega_{F}} \in\HS_{F}([0, L])$.
%%		\rev{We should better formulate this in terms of trace operator. For example, if $\HS_{M}(\Omega)= \H{\alpha}(\Omega)$, $\alpha\ge\frac{3}{2}$, then $\HS_{F}([0, L])=\H{\alpha-1}(\Omega_{F})$. Or should we even show this asymptotically from 3D fiber, where $\partial\Omega_{F}$ is not a degenerated boundary of $\Omega_{M}$ ? }
%%	\end{enumerate}
%%	In this case, the jump equation above becomes a continuity condition on~$\Omega_{F}$, and we have $\fib{\x} = \mtx{\x}\bigr|_{\Omega_{F}}$.
%%	Moreover, the system~\eqref{eq:system1D/3D} reduces to
%%	%Since $\vec{\phi}\in\{ \vec{\hat{\phi}} \; : \; \exists \vec{v}\in\HS(\Omega), \; \vec{v}\bigr|_{\Omega_{F}} = \vec{\hat{\phi}}  \}$, we can write the above system as
%If $\forall \; \vec{v}\in\HS_{M}(\Omega)$ we have $\vec{v}\bigr|_{\Omega_{F}} \in\HS_{F}([0, L])$, then the Lagrange multipliers $\vec{\lambda}$ and $\vec{\hat{\lambda}}$ can be condensed, and the system~\eqref{eq:system1D/3D} thus reduces to	
%	\begin{align}%\label{eq:system1D/3D_lambda_reduced}
%	\int\limits_{\Omega} \ten{P}_{M}:\nabla\vec{\delta u} \d V 
%	+
%	\int\limits_{\Omega} \vec{f}_{vol}\cdot\vec{\delta u} \d V
%	+
%	\int\limits_{\partial\Omega_{N}} \vec{t}_{ext}\cdot\vec{\delta u} \d V
%	-
%	\int\limits_{0}^{L}\left(\vec{N}^{\prime} - \vec{\bar{f}}_{vol}\right)\cdot\vec{\delta u}\d s
%	+
%	\!\!\!\sum_{\hat{s}\in\{0,L\}} \!\!\!\vec{N}(\hat{s})\cdot\vec{\delta u}(\hat{s})
%	&= 0, \label{eq:sys1D/3D:matrix} \\	
%	\int\limits_{0}^{L}\ten{Q}:\ten{\delta R}\, \d s &= 0, \label{eq:sys1D/3D:moments}
%	\end{align}
%	for all $\vec{\delta u}_{M}\in\HS_{M}(\Omega)$ and all $\ten{\delta R}\in\HS_{\ten{R}}([0,L])$, with the constitutive laws
%	\begin{gather}\label{key}
%	\vec{P}_{M} = \vec{P}_{M}(\nabla\vec{u})  \;\text{ in }\Omega, \\
%	\vec{N} = \vec{N}(\nabla\vec{u}, \fib{\ten{R}}) \;\text{ and }\;
%	\ten{Q} = \ten{Q}(\nabla\vec{u}, \fib{\ten{R}}) \; \text{ in }\Omega_{F}.
%	\end{gather}
%	Remind that $\vec{f}_{vol}$ and $\vec{\bar{f}}_{vol}$ are volumetric forces acting on matrix and fiber respectively.
%	
%	Thus, in the system~~\eqref{eq:sys1D/3D:matrix}-\eqref{eq:sys1D/3D:moments}, the presence of the fiber embedded into the material matrix is now formulated simply via additional fiber-induced load~$\ten{N}$ in $\Omega_{F}$, governed by additional equation~\eqref{eq:sys1D/3D:moments}.
%	
%	\rev{We should better formulate this in terms of trace operator.
%		That is, $\mtx{\x}\bigr|_{\Omega_{F}}=\fib{\x}$ means $\fib{\x} = \operatorname{Trace}_{\Omega_{F}}\mtx{\x}$. For example, if $\HS_{M}(\Omega)= \H{\alpha}(\Omega)$, $\alpha\ge\frac{3}{2}$, then $\HS_{F}([0, L])=\H{\alpha-1}(\Omega_{F})$.}
%\end{proposition}
%
%
%
%
%
%%%\subsection{Collocation coupling}
%%
%%\newcommand{\CollocSet}{\mathcal{S}}
%%
%%\begin{proposition}[Collocation coupling]
%%	Let $\CollocSet = \{s_k, \; k=1..n\}$ be a set of $n$ points on $[0,L]$, such that $s_k\notin\{0,L\}$.
%%	Let us return to the system~\eqref{eq:system1D/3D} and consider 
%%	$$\HS_{\vec{\lambda}}=\vspan\{\delta(s-s_k), \; s_k\in\CollocSet\}^3,$$ 
%%	where $\delta(s)$ denotes Dirac $\delta$-function.
%%	Then, from the last equation of~\eqref{eq:system1D/3D} we have $\mtx{\x}\bigr|_{\CollocSet}=\fib{\x}\bigr|_{\CollocSet}$.
%%	Moreover,
%%	$$\vec{\lambda}(s) = \sum_{k=1}^{n}\vec{\lambda}_k\,\delta(s - s_k).$$
%%	Hence, the system~\eqref{eq:system1D/3D} writes
%%	\begin{equation}
%%	\begin{aligned}\label{eq:system1D/3D_collocation}
%%	\int\limits_{\Omega} \ten{P}_{M}:\nabla\vec{\delta u}_{M} \d V 
%%	+
%%	\sum_{k=0}^{n+1}\vec{\lambda}_k\cdot\vec{\delta u}_{M}(\X_{s_k})
%%	%	+
%%	%	\!\!\!\!\sum_{\hat{s}\in\{0,L\}} \!\!\!\!\vec{\hat{\lambda}}_{\hat{s}}\cdot\vec{\delta u}_{M}(\X_{\hat{s}})
%%	+
%%	\!\!\int\limits_{\Omega} \vec{f}_{vol}\cdot\vec{\delta u}_{M} \d V
%%	+
%%	\!\!\int\limits_{\partial\Omega_{N}} \vec{t}_{ext}\cdot\vec{\delta u}_{M} \d V
%%	&= 0, 
%%	\quad \forall\;\vec{\delta u}_{M}\in\HS_{M}(\Omega),
%%	\\
%%	\int\limits_{0}^{L}\vec{N}^{\prime}\cdot\vec{\delta\fib{\varphi}}\, \d s
%%	+
%%	\sum_{k=1}^{n}\vec{\lambda}_k\,\vec{\delta\fib{\varphi}}(s_k)
%%	-
%%	\int\limits_{0}^{L} \vec{\bar{f}}_{vol}\cdot\vec{\delta\fib{\varphi}} \d s
%%	&= 0,
%%	\quad \forall\;\vec{\delta\fib{\varphi}}\in\HS_{F}([0,L]), 
%%	\\
%%	\vec{N}(0) = \vec{\lambda}_{0}, \qquad \vec{N}(L) &= \vec{\lambda}_{n+1}, 
%%	\\	
%%	\int\limits_{0}^{L}\ten{Q}:\ten{\delta R}\, \d s &= 0, 
%%	\quad \forall\;\ten{\delta R}\in\HS_{\ten{R}}([0,L]),
%%	\\
%%	\mtx{\x}(\X_{s_k}) &=\fib{\x}(s_k), \quad s_k\in\CollocSet,
%%	\end{aligned}
%%	\end{equation}
%%	where $s_0=0$, $s_{n+1}=L$, $\vec{\lambda}_0=\vec{\hat{\lambda}}_0$, $\vec{\lambda}_{n+1}=\vec{\hat{\lambda}}_L$.
%%	Such collocation coupling can be used in combination with the isogeometric collocation method~\cite{Weeger2017} for fiber discretization, using $\CollocSet$ as collocation points.
%%	\rev{Note that using the last equation of~\eqref{eq:system1D/3D_collocation} also allows to condense~$\vec{\lambda}_k$.}
%\end{proposition}


==> sections/sec_Coupling3.tex <==
%\subsection{Thin fiber coupling.}





%With regard to (\ref{eq:fib:position_ref}) and (\ref{eq:fib:position}), we reformulate the position field of the matrix in terms of the convective coordinates $(\theta^{\alpha},s)$ as follows
%\begin{equation}\label{eq:expansion_r}
%\vec{\varphi}(\theta^{\alpha},s) = \vec{\varphi}_c(s) + \vec{F}_{c}(s)\,\theta^{\alpha}\,\vec{D}_{\alpha}(s) + \O\left(\abs{\theta^{\alpha}}^2\right),
%\end{equation}
%where $\vec{\varphi}_c(s):=\vec{\varphi}(\tilde{\vec{\varphi}}_0(s))$ and $\vec{F}_c(s):=\vec{F}(\tilde{\vec{\varphi}}_0(s))$.
%% correlates to \ref{eq:deformationgradient}, evaluated at the centerline of the beam, i.e.\ $\vec{X}_{c}(s) \,\hat{=}\,\tilde{\vec{\varphi}}_0(s)$ and $\vec{x}_{c}(s) = \vec{\varphi}(\vec{X}_c(s))$.
%
%In our reduced model, we truncate the expansion~\eqref{eq:expansion_r} after the first two terms yielding a modeling error of order $\O\left(r^2\right)$.

\input{tikz/fiber3D/fiber3D}
\rev{TODO (Ustim): modify the beam picture.}

The coupling conditions have to be evaluated at the surfaces $A_0$, $A_L$ and $\Gamma_C$. Therefore, the virtual work of coupling forces over the whole matrix/beam interface reads
\begin{equation}\label{eq:CouplingTerm}
\Pi_{\Gamma} = \int_{\partial\tilde{\Omega}}\vec{\mu}\cdot\left(\vec{x}-\tilde{\vec{x}}\right)\d A =\Pi_{C} + \Pi_{A},
\end{equation}
\begin{equation}\label{eq:coupling_term_init}
\Pi_{C} = \int\limits_{\mathfrak{C}_0} \int\limits_{C(s)}\vec{\mu}\cdot\left(\vec{x}-\tilde{\vec{x}}\right)\d C\d s,
\qquad
\Pi_{A} = \sum_{s=0,L} \int\limits_{A(s)}\vec{\mu}\cdot\left(\vec{x}-\tilde{\vec{x}}\right)\d A,
\end{equation}
where $A(s)$ and $C(s)$ are respectively the beam cross-section and its boundary corresponding to the arc-length $s$.
Next, we decompose the interface Lagrange multipliers $\vec{\mu}$, physically interpreted as interface load, into mean and fluctuation parts
\begin{equation}\label{eq:LM_mu}
\vec{\mu}\big|_{\Circ(s)} = \bar{\vec{\mu}}(s) + \tilde{\vec{\mu}}(\theta^{\alpha},s),\quad\text{where}\quad
\bar{\vec{\mu}}(s) = \frac{1}{|C(s)|}\int\limits_{C(s)}\vec{\mu}\d C,\quad\int\limits_{C(s)}\tilde{\vec{\mu}}\d C = \vec{0},
\end{equation}
where the average term~$\bar{\vec{\mu}}$ corresponds to the resulting force applied to the cross-section, while the zero-mean term~$\tilde{\vec{\mu}}$ contains the hydrostatic pressure, shear and coupled stresses, produced by the matrix/beam coupling. 
Therefore, we write it in the following form:
\begin{equation}\label{eq:new:mu_tilde}
\tilde{\vec{\mu}}(\theta^{\alpha},s) = \ten{\Sigma}(s)\,\vec{N}(\theta^{\alpha}),
\end{equation}
where $\ten{\Sigma}$ denotes the interface stress tensor, and $\vec{N}=(\theta^{\alpha}\,\vec{D}_{\alpha})/\|\theta^{\alpha}\,\vec{D}_{\alpha}\|\big|_{\Circ(s)}$ is the unit outer normal to the interface in the reference configuration.
This term can be rewritten using $\vec{N}=\vec{D}_1\,\cos\theta + \vec{D}_2\,\sin\theta$, where $\cos\theta = \theta^{1}\,\vec{D}_{1}\cdot\theta^{2}\,\vec{D}_{2}/(\|\theta^{1}\,\vec{D}_{1}\|\|\theta^{2}\,\vec{D}_{2}\|)$.
Note that $\int_{C(s)}\ten{\Sigma}(s)\,\vec{N}(\theta^{\alpha})\d C = \ten{\Sigma}(s)\int_{C(s)}\,\vec{N}(\theta^{\alpha})\d C = 0$.
Besides, $\tilde{\vec{\mu}}$ has six degrees of freedom.
In particular, denoting $\ten{P}_{12} = \vec{D}_{\alpha}\otimes\vec{D}_{\alpha}$ and $\ten{\mathcal{D}}=\vec{D}_j\otimes\vec{e}_j$, we can write
\begin{equation}\label{eq:new:LM_matrix}
\ten{\Sigma}\,\ten{P}_{12} =
\fib{\vec{R}}\,\ten{\mathcal{D}}
\begin{bmatrix}
\tilde{\mu}_{n,1} + \tilde{\mu}_{n,2} & \tilde{\mu}_{n,3} - \tilde{\mu}_{\tau,3} & 0\\
\tilde{\mu}_{n,3} + \tilde{\mu}_{\tau,3} & \tilde{\mu}_{n,1} - \tilde{\mu}_{n,2} & 0\\
-2\,\tilde{\mu}_{\tau,2} &  2\,\tilde{\mu}_{\tau,1} & 0
\end{bmatrix}
\ten{\mathcal{D}}\tp,
\end{equation}
where $\tilde{\mu}_{n,1}$ is associated to the dilatation of the cross-section, $\tilde{\mu}_{n,2}$ and $\tilde{\mu}_{n,3}$ to the shear, $\tilde{\mu}_{\tau,1}$ and $\tilde{\mu}_{\tau,2}$ to the bending, and $\tilde{\mu}_{\tau,3}$ to the torsion.

\rev{Our previous model turns out to be a particular case, where
	one assumes	no shear constraints, that is, $\tilde{\mu}_{n,1}=\tilde{\mu}_{n,2}=0$, or $\sym{\ten{P}_{12}\,\fib{\vec{R}}\tp\,\ten{\Sigma}\,\ten{P}_{12}} = \mu_{n,1}\,\ten{P}_{12}$.}

Representation of the coupling stress~$ \ten{\Sigma} $ is proposed in the following proposition.
\begin{proposition}
	Let $\tilde{\vec{\mu}}_n = \tilde{\mu}_{n,j}\,\vec{d}_j$
	and $\tilde{\vec{\mu}}_\tau = \tilde{\mu}_{\tau,j}\,\vec{d}_j = \axl\left(\ten{\Sigma}\,\ten{P}_{12}\,\fib{\vec{R}}\tp\right)$.	
	Then, we have
	\begin{equation}\label{key}
	\frac{1}{2}\,\ten{\Sigma}\,\ten{P}_{12} = \left(\ten{\mathcal{P}}_{\alpha}\,\tilde{\vec{\mu}}_\tau + \ten{\mathcal{Q}}_{\alpha}\,\tilde{\vec{\mu}}_n\right)\otimes\vec{D}_\alpha,
	\end{equation}
	where
	\begin{align}
	\ten{\mathcal{P}}_1 &= \left(\frac{1}{2}\,\vec{d}_2\otimes\vec{d}_3 - \vec{d}_3\otimes\vec{d}_2\right), &
	\ten{\mathcal{P}}_2 &= \left(-\frac{1}{2}\,\vec{d}_1\otimes\vec{d}_3 + \vec{d}_3\otimes\vec{d}_1\right), \\
	\ten{\mathcal{Q}}_1 &= \frac{1}{2}\left(\vec{d}_1\otimes\vec{d}_1 + \vec{d}_1\otimes\vec{d}_2 + \vec{d}_2\otimes\vec{d}_3\right), &
	\ten{\mathcal{Q}}_2 &= \frac{1}{2}\left(\vec{d}_2\otimes\vec{d}_1 - \vec{d}_2\otimes\vec{d}_2 + \vec{d}_1\otimes\vec{d}_3\right).
	\end{align}	
	Moreover, it holds the following decomposition:
	\begin{equation}\label{eq:new:prop:decomposition}
	\frac{1}{2}\,\ten{\Sigma}\,\ten{P}_{12}
	=
	\left(\ten{I}-\frac{1}{2}\,\fib{\vec{R}}\,\ten{P}_{12}\,\fib{\vec{R}}\tp\right)\underbrace{\skew{\ten{\Sigma}\,\ten{P}_{12}\,\fib{\vec{R}}\tp}}_{\VPTen{\tilde{\vec{\mu}}_\tau}}\fib{\vec{R}}\,\ten{P}_{12}
	+
	\underbrace{\frac{1}{2}\,\fib{\vec{R}}\,\sym{\ten{P}_{12}\,\fib{\vec{R}}\tp\,\ten{\Sigma}\,\ten{P}_{12}}}_{\ten{\mathcal{Q}}_{\alpha}\,\tilde{\vec{\mu}}_n\otimes\vec{D}_\alpha}.		
	\end{equation}
\end{proposition}

\begin{proof}	
%	\begin{equation}\label{key}
%	\begin{aligned}
%	\left(\ten{I}-\frac{1}{2}\,\ten{P}_{12}\right)\skew{\fib{\vec{R}}\tp\,\ten{\Sigma}\,\ten{P}_{12}}\,\ten{P}_{12}
%	&=
%	\frac{1}{2}\,\left(\ten{I}-\frac{1}{2}\,\ten{P}_{12}\right)\fib{\vec{R}}\tp\,\ten{\Sigma}\,\ten{P}_{12}
%	-
%	\frac{1}{4}\,\ten{P}_{12}\,\ten{\Sigma}\tp\,\fib{\vec{R}}\,\ten{P}_{12} \\
%	&=
%	\frac{1}{2}\,\fib{\vec{R}}\tp\,\ten{\Sigma}\,\ten{P}_{12}
%	-
%	\frac{1}{2}\,\sym{\ten{P}_{12}\,\fib{\vec{R}}\tp\,\ten{\Sigma}\,\ten{P}_{12}}.
%	\end{aligned}	
%	\end{equation}	
\begin{equation}
	\begin{aligned}
	\left(\ten{I}-\frac{1}{2}\,\fib{\vec{R}}\,\ten{P}_{12}\,\fib{\vec{R}}\tp\right)\,\skew{\ten{\Sigma}\,\ten{P}_{12}\,\fib{\vec{R}}\tp}\,\fib{\vec{R}}\,\ten{P}_{12}
	&=
	\frac{1}{2}\,\ten{\Sigma}\,\ten{P}_{12}-\frac{1}{4}\,\fib{\vec{R}}\,\ten{P}_{12}\,\left(\ten{\Sigma}\tp\,\fib{\vec{R}}+\fib{\vec{R}}\tp\,\ten{\Sigma}\right)\,\,\ten{P}_{12}\\
	&=
	\frac{1}{2}\,\ten{\Sigma}\,\ten{P}_{12}
	-\frac{1}{2}\,\fib{\vec{R}}\,\sym{\ten{P}_{12}\,\fib{\vec{R}}\tp\,\ten{\Sigma}\,\ten{P}_{12}}.
	\end{aligned}	
	\end{equation}	
\end{proof}

%In particular, it can be decomposed on a spherical part, deviatoric and skew-symmetric parts:
%\begin{equation}\label{key}
%	\ten{\Sigma} = \mu_n\ten{\Id} + \dev{\ten{\Sigma}} + \left[\vec{\mu}_\tau\right]_\times,
%\end{equation}
%where
%\begin{align}\label{key}
%	 \mu_n &= \frac{1}{3}\tr\ten{\Sigma},\\
%	 \dev{\ten{\Sigma}} &= \frac{1}{2}\left(\ten{\Sigma}+\ten{\Sigma}\tp\right)- \mu_n\ten{\Id},\\
%	 \vec{\mu}_\tau &= \axl\ten{\Sigma}.
%\end{align}

\begin{lemma}\label{th:CouplingTerm}
	Given~\eqref{eq:LM_mu} and~\eqref{eq:new:mu_tilde}, the coupling term~\eqref{eq:coupling_term_init} writes
	\begin{equation}\label{eq:coupling_term_lemma}
	\Pi_{C}
	=
	\int\limits_{\mathfrak{C}_0} \bar{\vec{\mu}}\cdot\left(\bar{\vec{\varphi}}-\tilde{\vec{\varphi}}\right) \abs{C}\d s
	+
	\int\limits_{\mathfrak{C}_0} \ten{\Sigma}:\left(\ten{\mathcal{F}}-\frac{1}{2}\,\fib{\vec{R}}\,\ten{P}_{12}\right) \abs{C}\d s
	,
	\end{equation}
	with the circumference length~$ \abs{C} = 2\,\pi\, r $, and
	\begin{equation}
	\bar{\vec{\varphi}} = \frac{1}{\abs{C}}\int\limits_{C(s)}\vec{\varphi}\d C,
	\qquad
	\ten{\mathcal{F}} = \frac{1}{\abs{C}}\int\limits_{C(s)} \vec{\varphi} \otimes \vec{N}\d C.
	\end{equation}
\end{lemma}

\begin{proof}
	From \eqref{eq:LM_mu}, \eqref{eq:new:mu_tilde} and \eqref{eq:coupling_term_init}, it writes
	\begin{equation}\label{eq:coupling_term_proof}
	\Pi_{C}
	=
	\int\limits_{\mathfrak{C}_0}\int\limits_{C(s)}\underbrace{\left(\bar{\vec{\mu}} +  \ten{\Sigma}\,\vec{N}\right)}_{\vec{\mu}}
	\cdot\biggl(\vec{\varphi}-\underbrace{\left(\tilde{\vec{\varphi}}+\theta^{\alpha}\,\vec{d}_{\alpha}\right)}_{\tilde{\vec{x}}}\biggr) \d C\d s
	.
	\end{equation}
	Remark that for the circular cross-section, $\theta^{\alpha}\,\vec{D}_{\alpha}\bigr|_{C(s)}\! = \vec{N}\,r$, 
	and thus $\theta^{\alpha}\,\vec{d}_{\alpha}\bigr|_{C(s)} \!= \fib{\vec{R}}\,\vec{N}\,r$.
	Besides, it is easy to see that
	\begin{equation}\label{eq:int_N}
		\int_{C}\vec{N}\d C = \vec{0}
		\qquad\text{and}\qquad
		\int_{C}\vec{N}\otimes\vec{N}\d C = \pi\,\ten{P}_{12}.
	\end{equation}
	Thus, \eqref{eq:coupling_term_proof} writes
	\begin{equation}
	\begin{aligned}
	\Pi_{C}
	&=
	\int\limits_{\mathfrak{C}_0}\bar{\vec{\mu}}\cdot\int\limits_{C(s)}\left(\vec{\varphi}-\tilde{\vec{\varphi}}\right)\d C\d s
	+ 
	\int\limits_{\mathfrak{C}_0}\int\limits_{C(s)}\ten{\Sigma}:\left(\vec{\varphi}-\fib{\vec{R}}\,\vec{N}\,r\right)\otimes\vec{N} \d C\d s
	\\
	&=
	\int\limits_{\mathfrak{C}_0} \bar{\vec{\mu}}\cdot\left(\int\limits_{C(s)}\vec{\varphi}\d C-\tilde{\vec{\varphi}}\abs{C}\right) \d s
	+
	\int\limits_{\mathfrak{C}_0} \ten{\Sigma}:\left(\int\limits_{C(s)}\vec{\varphi}\otimes\vec{N}\d C - \pi \,r\,\fib{\vec{R}}\,\ten{P}_{12}\right)\d s
	.
	\end{aligned}	
	\end{equation}
	Hence follows the statement.
\end{proof}


\begin{remark}
	Remark that $ \ten{\mathcal{F}} $ corresponds to the first coefficient ($k=1$) in Fourier decomposition of~$ \vec{\varphi} $ on~$C(s)$ as function of the angle~$\theta$.
\end{remark}

\begin{remark}\label{rmk:wellposedness}
	Let us note that if $\vec{\varphi}\in\H{1}(\Omega)^3$, then according to the trace theorem, $\bar{\vec{\varphi}}\in\H{\frac{1}{2}}(\mathfrak{C}_0)^3$ and thus is in~$\L{2}(\mathfrak{C}_0)^3$.
	Likewise, $ \ten{\mathcal{F}} \in \L{2}(\mathfrak{C}_0)^{3\times 3} $.
	Thus, for $ \tilde{\vec{\varphi}}\in\H{1}(\mathfrak{C}_0)^3 $, $ \fib{\vec{R}}\in\H{1}(\mathfrak{C}_0)^{3\times 3}$,  $ \bar{\vec{\mu}}\in\L{2}(\mathfrak{C}_0)^3 $ 
	and $ \ten{\Sigma}\in\L{2}(\mathfrak{C}_0)^{3\times 3}$, the integral in~\eqref{eq:coupling_term_lemma} is defined.
\end{remark}

Analogous to~\eqref{eq:LM_mu}-\eqref{eq:new:mu_tilde}, we define the Lagrange multipliers on the sides~$A_0$ and $A_L$:
\begin{equation}\label{eq:LM_mu_A}
\vec{\mu}\big|_{\Area_s} = \bar{\vec{\mu}}^s + \ten{\Sigma}^s\,\vec{N}(\theta^{\alpha}),\quad\text{where}\quad
\bar{\vec{\mu}}^s(s) = \frac{1}{|A_s|}\int\limits_{A_s}\vec{\mu}\d A,
\end{equation}
with $\vec{N}=\vec{D}_1\,\cos\theta + \vec{D}_2\,\sin\theta$, and where $\ten{\Sigma}^s$ has the same form as in~\eqref{eq:new:LM_matrix}.
Then, similar to Lemma~\ref{th:CouplingTerm}, we have
\begin{equation}\label{eq:coupling_term_lemma_A}
\Pi_{A}
=
\sum_{s=0,L} \left[\bar{\vec{\mu}}^s\cdot\left(\bar{\vec{\varphi}}(s)-\tilde{\vec{\varphi}}(s)\right)
+
\ten{\Sigma}^s:\left(\ten{\mathcal{F}}(s)-\frac{1}{2}\,\fib{\vec{R}}(s)\,\ten{P}_{12}\right)\right] \abs{A_s}.
\end{equation}


\begin{proposition}
	Assuming enough regularity of~$\vec{\varphi}$, we can write
	\begin{equation}\label{eq:expansion_r}
	\vec{\varphi}\bigr|_{C(s)} = \vec{\varphi}_c(s) + \vec{F}_{c}(s)\,\vec{N}(\theta)\,r + \O(r^2),
	\end{equation}
	where $\vec{\varphi}_c(s):=\vec{\varphi}(\tilde{\vec{\varphi}}_0(s))$ and $\vec{F}_c(s):=\vec{F}(\tilde{\vec{\varphi}}_0(s))$.
	% correlates to \ref{eq:deformationgradient}, evaluated at the centerline of the beam, i.e.\ $\vec{X}_{c}(s) \,\hat{=}\,\tilde{\vec{\varphi}}_0(s)$ and $\vec{x}_{c}(s) = \vec{\varphi}(\vec{X}_c(s))$.
	Then, due to~\eqref{eq:int_N}, we have
	\begin{equation}\label{eq:r2_trunc}
		\bar{\vec{\varphi}} = \vec{\varphi}_c + \O(r^2),
		\qquad\text{and}\qquad
		\ten{\mathcal{F}} = \frac{1}{2}\,\vec{F}_{c}\,\ten{P}_{12} + \O(r^2).
	\end{equation}
	
	In our reduced model, we truncate the expansion~\eqref{eq:expansion_r} after the first two terms yielding a modeling error of order $\O\left(r^2\right)$.
	

\end{proposition}

%\rev{TODO (Ustim): show rigorously expansion \eqref{eq:expansion_r}. }

\rev{Note that in the beam constitutive law, the stiffness tensors include area and moments of area, which are of order $\O\left(r^2\right)$ and $\O\left(r^4\right)$, respectively.
	So, it may be important the order of the value $E\,r^2$. 
	@Barbara: Leaving the third term may be very hard to handle.}

\rev{(IMPORTANT)
Here we have to decide about the strategy.
The problem is well-posed in terms of $ \bar{\vec{\varphi}} $ and $ \ten{\mathcal{F}} $ (see integral~\eqref{th:CouplingTerm} and Remark~\ref{rmk:wellposedness}),
however the trace of $\vec{\varphi}\in\H{1}(\Omega)^3$ on $\mathfrak{C}_0$ is not defined, so $\vec{\varphi}_c$ and $\vec{F}_{c} $ are not defined.
There are two possible solutions:
\begin{enumerate}
	\item Consider a second gradient material for the matrix, such that $\vec{\varphi}\in\H{2}(\Omega)^3$, $p>2$.
	So, $\vec{\varphi}_c\in\H{1}(\mathfrak{C}_0)^3$ and $\vec{F}_{c}\in\L{2}(\mathfrak{C}_0)^{3\times 3}$.
	\item Loose consistency in our approach, despite the title ).
	Using Galerkin, we have enough regularity for the projections, so \eqref{eq:r2_trunc} will work fine.
	However, the limit won't be defined.
\end{enumerate}
}


\paragraph{Surrogate model for the coupling term.}

In this work, we propose a reduced surrogate model for the coupling term~\eqref{eq:CouplingTerm} under the following assumption:
\begin{itemize}
	\item[A1.] Matrix continuum is extended inside the fiber.
	This yields a modeling error due to additional stiffness, which depends on the fiber radius and the ratio of the matrix stiffness to the fiber stiffness.
	Such type of modeling error was studied for diffusion problem in~\cite{koppl2018mathematical}, where it was estimated to be of order~$\O\left(r\sqrt{\log r}\right)$.
		
	\CH{We should also consider to remove the matrix stresses within the beam domain. This is something I have to look how we did this in FSI. }
	\item[A2.] Lagrange multiplier~$\vec{\mu}$ are in the form~\eqref{eq:LM_mu}-\eqref{eq:new:mu_tilde}.
	\item[A3.] We assuming enough regularity of~$\vec{\varphi}$ and truncate the expansion~\eqref{eq:expansion_r} after the first two terms yielding a modeling error of order $\O\left(r^2\right)$.
\end{itemize}

Thus, truncating the higher order terms of~\eqref{eq:r2_trunc} in~\eqref{eq:coupling_term_lemma}, we obtain
\begin{equation}
\Pi_C
=
\int\limits_{\mathfrak{C}_0}\left[\bar{\vec{\mu}}\cdot(\vec{\varphi}_{c} -\tilde{\vec{\varphi}})
+
\frac{1}{2}\left[
\big(\vec{F}_c-\fib{\vec{R}}\big)\,\ten{P}_{12}\right]:\ten{\Sigma}
\right]\abs{C}\d s.
\end{equation}
Hence, the associated virtual work is given by
\begin{equation}\label{eq:VirtWork_coupling}
\begin{aligned}
\delta\Pi_C
&=
\int\limits_{\mathfrak{C}_0}\bigl[\delta\bar{\vec{\mu}}\cdot(\vec{\varphi}_{c} -\tilde{\vec{\varphi}})
+
\bar{\vec{\mu}}\cdot(\delta\vec{\varphi}_{c} -\delta\tilde{\vec{\varphi}})\bigr]\abs{C}\d s +
\\
&+
\frac{1}{2}\int\limits_{\mathfrak{C}_0}\left[\left[
\big(\nabla\delta\vec{\varphi}-\left[\delta\vec{\phi}\right]_\times\fib{\vec{R}}\big)\,\ten{P}_{12}\right]:\ten{\Sigma}
+
\left[\big(\vec{F}_{c}-\fib{\vec{R}}\big)\,\ten{P}_{12}\right]:\delta\ten{\Sigma}
\right]\abs{C}\d s.
\end{aligned}
\end{equation}

%For the circular cross-section, it holds that $\theta^{\alpha}\,\vec{D}_{\alpha} = \vec{N}\,r$, and thus we have
%\begin{equation}
%\Pi_{C} = \int\limits_{\mathfrak{C}_0} \int\limits_{C(s)}\left(\bar{\vec{\mu}} + \ten{\Sigma}\,\vec{N}\right)
%\cdot\big( (\vec{\varphi}_{c} + \vec{F}_{c}\,\vec{N}\,r) -(\tilde{\vec{\varphi}} + \fib{\vec{R}}\vec{N}\,r)\big)\d C\d s.
%\end{equation}
%Remind that~$ \int_{C}\vec{N}\d C = \vec{0} $.
%Hence, together with~\eqref{eq:key3}, it yields
%\begin{equation}\label{eq:new:Pi_C}
%\Pi_{C} = \int\limits_{\mathfrak{C}_0}\left[\bar{\vec{\mu}}\cdot(\vec{\varphi}_{c} -\tilde{\vec{\varphi}})\abs{C} + 
%\int\limits_{C(s)} \ten{\Sigma}\,\vec{N}\cdot\big(\vec{F}_{c}-\fib{\vec{R}}\big)\,\vec{N}\,r \d C\right]\d s,
%\end{equation}
%with the circumference length~$ \abs{C} = 2\pi r $.
%The first term in~\eqref{eq:new:Pi_C} enforces the position of the centerline of the beam along its counterpart in the continuum,
%while the second term couples the beam cross-section to the continuum deformation.

%\begin{proposition}
%	Given the outer normal vector
%	$
%	\vec{N} = \vec{D}_1\,\cos\theta + \vec{D}_2\,\sin\theta,
%	$
%	one has for an arbitrary matrix~$\vec{A}$:
%	\begin{equation}\label{eq:axial_int}
%	\begin{aligned}	
%	\int\limits_{0}^{2\,\pi}\vec{N}\cdot\left(\ten{A}\,\vec{N}\right)\d\theta
%	&=
%	\int\limits_{0}^{2\,\pi}(\vec{D}_1\,\cos\theta + \vec{D}_2\,\sin\theta)\cdot\left(\ten{A}\,\vec{D}_1\,\cos\theta + \ten{A}\,\vec{D}_2\,\sin\theta\right)\d\theta \\
%	&=
%	\int\limits_{0}^{2\,\pi}\left(\vec{D}_1\tp\,\ten{A}\,\vec{D}_1\,\cos^2\theta + \vec{D}_2\tp\,\ten{A}\,\vec{D}_2\,\sin^2\theta + (\vec{D}_1\tp\,\vec{A}\,\vec{D}_2 + \vec{D}_2\tp\,\ten{A}\,\vec{D}_1)\,\cos\theta\,\sin\theta\right)\d\theta \\
%	&=
%	\pi\,\left(\vec{D}_1\tp\,\ten{A}\,\vec{D}_1 + \vec{D}_2\tp\,\ten{A}\,\vec{D}_2\right)
%	=
%	\pi\,\tr\left(\ten{A}\ten{P}_{12}\right). \\	
%	\end{aligned}
%	\end{equation}
%\end{proposition}



%According to~\eqref{eq:axial_int}, the second term in~\eqref{eq:new:Pi_C} writes 
%\begin{equation}
%\int\limits_{C(s)} \vec{N}\cdot\ten{\Sigma}\tp\big(\vec{F}_{c}-\fib{\vec{R}}\big)\,\vec{N}\ \d C
%=
%\pi\tr\left(\ten{\Sigma}\tp\big(\vec{F}_{c}-\fib{\vec{R}}\big)\ten{P}_{12}\right).
%\end{equation}
%And thus, the virtual work associated to~\eqref{eq:new:Pi_C} is given by
%\begin{equation}\label{eq:VirtWork_coupling}
%\begin{aligned}
%\delta\Pi_C
%&=
%\int\limits_{\mathfrak{C}_0}\bigl[\delta\bar{\vec{\mu}}\cdot(\vec{\varphi}_{c} -\tilde{\vec{\varphi}})
%+
%\bar{\vec{\mu}}\cdot(\delta\vec{\varphi}_{c} -\delta\tilde{\vec{\varphi}})\bigr]\abs{C}\d s +
%\\
%&+
%\frac{1}{2}\int\limits_{\mathfrak{C}_0}\left[
%\big(\nabla\delta\vec{\varphi}-\left[\delta\vec{\phi}\right]_\times\fib{\vec{R}}\big)\ten{P}_{12}:\ten{\Sigma}
%+
%\big(\vec{F}_{c}-\fib{\vec{R}}\big)\ten{P}_{12}:\delta\ten{\Sigma}
%\right]\abs{C}\d s.
%\end{aligned}
%\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\paragraph{Endpoint constraints.}
Likewise, we derive the virtual work of the coupling term at the endpoints:
\begin{equation}\label{eq:VirtWork_endpoints}
\begin{aligned}
\delta\Pi_A
&=
\sum_{s=0,L}\bigl[\delta\bar{\vec{\mu}}^s\cdot(\vec{\varphi}_{c} -\tilde{\vec{\varphi}})
+
\bar{\vec{\mu}}^s\cdot(\delta\vec{\varphi}_{c} -\delta\tilde{\vec{\varphi}})\bigr]\abs{A_s} +
\\
&+
\frac{1}{2}\sum_{s=0,L}\left[\left[
\big(\nabla\delta\vec{\varphi}-\left[\delta\vec{\phi}\right]_\times\fib{\vec{R}}\big)\,\ten{P}_{12}\right]:\ten{\Sigma}^s
+
\left[\big(\vec{F}_{c}-\fib{\vec{R}}\big)\,\ten{P}_{12}\right]:\delta\ten{\Sigma}^s
\right]\abs{A_s}.
\end{aligned}
\end{equation}


\rev{As it was noticed, the point constraints for an integrable function is in general ill-posed. However, as it will be seen further, we eventually get rid of the endpoint constraints.
So, we should get rid of them earlier, on the level of Lemma~\ref{th:CouplingTerm}, where the analogues of integrals~$\bar{\vec{\varphi}}$ and $\ten{\mathcal{F}}$ in the endpoints are defined.
%Or consider the limit of sequence of smooth test functions.
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Total system.}
Finally, we obtain the principle of virtual work for the  coupled matrix/beam system, hence
\begin{equation}
\delta\Pi^{int} + \delta\Pi^{ext} + \delta\fib{\Pi}^{int} + \delta\fib{\Pi}^{ext} + \delta\Pi_C + \delta\Pi_A = 0,
\end{equation}
with regard to \eqref{eq:pdvA}, \eqref{eq:pdvaBeam} and \eqref{eq:pdvaHW2} along with the virtual work of the coupling forces in \eqref{eq:VirtWork_coupling} and \eqref{eq:VirtWork_endpoints}.
With regard to the matrix material, i.e., the variation with respect to $\delta\vec{\varphi}$, we obtain
\begin{equation}\label{eq:sys:matrix}
\begin{aligned}
&\int\limits_{\mtx{\Omega}_0} \left[\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}} - \vec{B}_{ext}\cdot\delta\vec{\varphi}\right] \d V	-
\int\limits_{\Gamma^{\sigma}} \vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d A
+\\
&
+
\int\limits_{\mathfrak{C}_0}\left(\vec{\bar{\mu}} \cdot \delta\vec{\mtx{\varphi}}
+
\frac{1}{2}\,\left[\ten{\Sigma}\,\ten{P}_{12}\right]:\nabla\delta\mtx{\vec{\varphi}} \right) \abs{C}\d s
+
\sum_{s=0,L}\left[\bar{\vec{\mu}}^s\cdot\delta\mtx{\vec{\varphi}}
+
\frac{1}{2}\,\left[\ten{\Sigma}^s\,\ten{P}_{12}\right]: \nabla\delta\mtx{\vec{\varphi}}\right] \abs{A_s}
= 0,
\end{aligned}
\end{equation}
%Note that the component~$\ten{\Sigma}\vec{d}_3$ does not enter in the matrix equation. 
and the beam contributions  yield
\begin{align}
&-\int\limits_{\mathfrak{C}_0}\left(
{\mathfrak{n}}^{\prime} + \bar{\tilde{\vec{n}}}
+
\bar{\vec{\mu}}\abs{C}\right)\cdot\delta\fib{\vec{\varphi}}\d s = 0,  
\label{eq:sys:loads}
\\	
&-\int\limits_{\mathfrak{C}_0}\biggl({\mathfrak{m}}^{\prime} + \tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}}
+
\bar{\tilde{\vec{m}}}
+
\tilde{\vec{\mu}}_\tau\abs{C}\biggr)\cdot\delta\vec{\phi} \d s = 0,
\label{eq:sys:moments}
\end{align}
supplemented by the constitutive equations in weak form
\begin{align}
&\int\limits_{\mathfrak{C}_0}\delta{\mathfrak{g}}\cdot\left(\fib{\ten{R}}\,\frac{\partial\tilde{\Psi}(\vec{\Gamma},\vec{K})}{\partial\vec{\Gamma}}-{\mathfrak{n}} \right)\d s = 0,
\label{eq:constitutive_n}
\\
&\int\limits_{\mathfrak{C}_0}\delta{\mathfrak{k}}\cdot\left( \fib{\ten{R}}\,\frac{\partial\tilde{\Psi}(\vec{\Gamma},\vec{K})}{\partial\vec{K}}-{\mathfrak{m}} \right)\,\text{d}s = 0,
\label{eq:constitutive_m}
\end{align}
the coupling constraints
\begin{align}
&\int\limits_{\mathfrak{C}_0}\delta\vec{\bar{\mu}} \cdot\left(\vec{\mtx{\varphi}}-\fib{\vec{\varphi}}\right)\d s = 0,	
\label{eq:sys:pi1}
\\
&\int\limits_{\mathfrak{C}_0}
\big(\vec{F}_{c}-\fib{\vec{R}}\big)\,\ten{P}_{12}:\delta\ten{\Sigma}\d s = 0 \qquad (6\text{ equations})
\label{eq:sys:pi2}
\end{align}
and the beam endpoints conditions at $s=0,L$:
\begin{align}
&\mathfrak{n} = \abs{A_s}\,\bar{\vec{\mu}}^s,
\label{eq:sys:bc_n}
\\
&\mathfrak{m} = \abs{A_s}\,\tilde{\vec{\mu}}_\tau^s.
\label{eq:sys:bc_m}
\end{align}

%\begin{remark}
%	Note that in~\eqref{eq:new:sys:moments2}, the spherical part of~$\fib{\vec{R}}\tp\ten{\Sigma}$, $\mu_n\ten{\Id}$, yields zero term, since $\axl\left(\fib{\vec{R}}\ten{P}_{12}\fib{\vec{R}}\tp\right)=0$.
%	That is, pressure produces no moments.
%\end{remark}

\begin{remark}
	Note that the component~$\ten{\Sigma}\,\vec{D}_3$ does not enter in the system at all, and that $\delta\ten{\Sigma}\,\ten{P}_{12}$, has only $6$ degrees of freedom: three for bending and torsion of the cross-section, one for dilatation and two more for the shear (directions $\vec{D}_{\alpha}$).
	
	%	Moreover, for $\delta\ten{\Sigma} = \VPTen{\delta\vec{\mu}_\tau}$ and $\delta\ten{\Sigma} = \delta\mu_n\,\ten{\Id}$, \eqref{eq:new:sys:pi3} respectively reproduces~\eqref{eq:sys:pi2} and ~\eqref{eq:sys:pi3}:
	%	\begin{align}\label{key}
	%	\int\limits_{\mathfrak{C}_0}
	%	\skew{\vec{F}_{c}\ten{P}_{12}\fib{\vec{R}}\tp}:\VPTen{\delta\vec{\mu}_\tau}\d s &= 0,\\
	%	\int\limits_{\mathfrak{C}_0}
	%	\tr\left[\big(\vec{F}_{c}-\fib{\vec{R}}\big)\ten{P}_{12}\fib{\vec{R}}\tp\right]\delta\mu_n\d s &= 0,
	%	\end{align}
	%	and deviatoric part gives us two more equations:
	%	\begin{align}\label{key}
	%	\int\limits_{\mathfrak{C}_0}
	%	\left(\vec{d}_{1}\cdot\vec{F}_{c}\vec{D}_{1} - \vec{d}_{2}\cdot\vec{F}_{c}\vec{D}_{2}\right) \,\delta\mu_{dev}^1\d s &= 0,\\	
	%	\int\limits_{\mathfrak{C}_0}
	%	\left(\vec{d}_{1}\cdot\vec{F}_{c}\vec{D}_{2} + \vec{d}_{2}\cdot\vec{F}_{c}\vec{D}_{1}\right) \,\delta\mu_{dev}^2\d s &= 0.
	%	\end{align}
\end{remark}

\begin{remark}
	Note that \eqref{eq:sys:pi2} can simply be written with 6 equations:
	\begin{align}\label{key}
	\int\limits_{\mathfrak{C}_0}
	\big(\vec{F}_{c}\,\vec{D}_{1}-\vec{d}_{1}\big)\cdot\delta\tilde{\vec{\mu}}_1\d s &= 0,\\
	\int\limits_{\mathfrak{C}_0}
	\big(\vec{F}_{c}\,\vec{D}_{2}-\vec{d}_{2}\big)\cdot\delta\tilde{\vec{\mu}}_2\d s &= 0.
	\end{align}
Here, the components of the vectors $\delta\tilde{\vec{\mu}}_k$ are given by the $k$-th column of the matrix in (\ref{eq:new:LM_matrix})	to the basis $\vec{d}_i$.
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\paragraph{Reduced system.} 
%According to the trace theorem~\cite{?}, if $\delta\vec{\varphi}\in\W{1}{p}(\Omega)$, $p>2$, the trace of $\delta\vec{\varphi}$ on the beam~$\tilde{\vec{\varphi}}_0(\mathfrak{C}_0)$ is in~$\L{2}(\mathfrak{C}_0)$.
%%If $\delta\vec{\varphi}\big|_{\mathfrak{C}_0}$ is in $\HS_{\delta\fib{\vec{\varphi}}}(\mathfrak{C}_0)$, 
%Then, 
Considering $\delta\fib{\vec{\varphi}} = \delta\vec{\varphi}\big|_{\mathfrak{C}_0}$, we can condense \eqref{eq:sys:loads} and \eqref{eq:sys:bc_n} to the matrix equation~\eqref{eq:sys:matrix}, which leads after integration by parts to
\begin{equation}\label{eq:new:sys:matrix_condense}
\begin{aligned}
&\int\limits_{\mtx{\Omega}} \left(\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}}- \vec{B}_{ext}\cdot\delta\vec{\varphi}\right) \d V
-
\int\limits_{\Gamma^{\sigma}} \vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d A
+
\int\limits_{\mathfrak{C}_0}\left(\left[\mathfrak{n}\otimes\vec{D}_3\right] : \nabla\delta\mtx{\vec{\varphi}}
-
\bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}\right)\d s
\\&+
\frac{1}{2}\,\int\limits_{\mathfrak{C}_0}
\left(\ten{\Sigma}\,\ten{P}_{12}\right):\nabla\delta\mtx{\vec{\varphi}} \abs{C}\d s
+
\frac{1}{2} \sum_{s=0,L}
\left(\ten{\Sigma}^s\,\ten{P}_{12}\right): \nabla\delta\mtx{\vec{\varphi}}\,\abs{A_s}
= 0.
\end{aligned}
\end{equation}

\rev{Do we need here any remark about regularity of the traces ?}

Thus, we have eliminated the set of Lagrange multipliers $\bar{\vec{\mu}}$.
% using \eqref{eq:sys:load}.
To eliminate the other Lagrange multipliers~$\ten{\Sigma}$, let us define
\begin{equation}\label{key}
 \hat{\vec{\phi}} = \axl\left(\left(\ten{\Id}-\frac{1}{2}\fib{\vec{R}}\ten{P}_{12}\fib{\vec{R}}\tp\right)\nabla\delta\vec{\mtx{\varphi}}\,\ten{P}_{12}\fib{\vec{R}}\tp\right).
\end{equation}
%If $\delta\vec{\varphi}\in\W{2}{p}(\Omega)$, $p>2$, then $ \nabla\delta\vec{\mtx{\varphi}}\,\vec{D}_\alpha \in\W{1}{p}(\Omega)$ with the traces on the beam in~$\L{2}(\mathfrak{C}_0)$.
%$\hat{\vec{\phi}}(\delta\vec{\mtx{\varphi}})\in \HS_{\delta\vec{\phi}}$ for all~$\delta\vec{\varphi}\in \HS_{\delta\vec{\varphi}}$, 
Then integration with $\delta\vec{\phi}=\hat{\vec{\phi}}(\delta\vec{\varphi})\in\L{2}(\mathfrak{C}_0)$ in~\eqref{eq:sys:moments} along with~\eqref{eq:new:prop:decomposition} yields
\begin{multline}
\int\limits_{\mathfrak{C}_0}\ten{\mathcal{P}}_{\alpha}
\left({\mathfrak{m}}^{\prime} + \tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}}+\bar{\tilde{\vec{m}}}\right)
\otimes\vec{D}_{\alpha}
:
\nabla\delta\vec{\mtx{\varphi}}
\d s
+
\\
+
\int\limits_{\mathfrak{C}_0}
\biggl(\frac{1}{2}\ten{\Sigma}\ten{P}_{12}
-
\underbrace{\frac{1}{2}\fib{\vec{R}}\sym{\ten{P}_{12}\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}}}_{\ten{\mathcal{Q}}_{\alpha}\tilde{\vec{\mu}}_n^s\otimes\vec{D}_{\alpha}}\biggr)
:
\nabla\delta\vec{\mtx{\varphi}}
\abs{C}\d s = 0.
\end{multline}
%\begin{multline}
%\int\limits_{\mathfrak{C}_0}
%\fib{\ten{R}}\tp\left({\mathfrak{m}}^{\prime} + \tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}}+\bar{\tilde{\vec{m}}}\right)
%\cdot
%\axl\left(\left(\ten{\Id}-\frac{1}{2}\ten{P}_{12}\right)\fib{\vec{R}}\tp\nabla\delta\vec{\mtx{\varphi}}\,\ten{P}_{12}\right)
%\d s
%+
%\\
%+
%\int\limits_{\mathfrak{C}_0}
%\axl\left(\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}\right)\cdot\axl\left(\left(\ten{\Id}-\frac{1}{2}\ten{P}_{12}\right)\fib{\vec{R}}\tp\nabla\delta\vec{\mtx{\varphi}}\,\ten{P}_{12}\right)
%\abs{C}\d s = 0.
%\end{multline}
%%Hence, applying~\eqref{eq:new:prop:decomposition}, we obtain
%%\begin{multline}
%%\frac{1}{2}\int\limits_{\mathfrak{C}_0}
%%\left(\ten{\Id}-\frac{1}{2}\fib{\ten{R}}\ten{P}_{12}\fib{\ten{R}}\tp\right)\VPTen{{\mathfrak{m}}^{\prime} + \tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}}
%%+
%%\bar{\tilde{\vec{m}}}}
%%\fib{\ten{R}}\ten{P}_{12}
%%:
%%\nabla\delta\vec{\mtx{\varphi}}
%%\d s
%%+
%%\\
%%+
%%\frac{1}{2}\int\limits_{\mathfrak{C}_0}
%%\left(\frac{1}{2}\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}
%%-
%%\frac{1}{2}\sym{\ten{P}_{12}\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}}\right):\fib{\ten{R}}\tp\nabla\delta\vec{\mtx{\varphi}}
%%\abs{C}\d s = 0.
%%\end{multline}
Subtracting the above equation from~\eqref{eq:new:sys:matrix_condense} and integrating by parts, we obtain
\begin{equation}%\label{eq:sys:matrix_condense2}
\begin{aligned}
&\int\limits_{\mtx{\Omega}} \left(\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}}- \vec{B}_{ext}\cdot\delta\vec{\varphi}\right) \d V
-
\int\limits_{\partial\Omega_{N}} \!\!\vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d S
+
\int\limits_{\mathfrak{C}_0}\left(\mathfrak{n}\otimes\vec{D}_3 : \nabla\delta\mtx{\vec{\varphi}}
-
\bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}\right)\d s\\
&
+
\int\limits_{\mathfrak{C}_0}
\left[\ten{\mathcal{P}}_{\alpha}\mathfrak{m}\otimes\vec{D}_\alpha\otimes\vec{D}_3\right]\,\vdots\,\nabla^2\delta\mtx{\vec{\varphi}}
\d s
+ \int\limits_{\mathfrak{C}_0}
\biggl[\ten{\mathcal{P}}_{\alpha}^\prime\mathfrak{m}
-\ten{\mathcal{P}}_{\alpha}\left(\tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}} +\bar{\tilde{\vec{m}}}\right)
\biggl]\otimes\vec{D}_{\alpha}:\nabla\delta\mtx{\vec{\varphi}}\,\d s
\\
&
+ \int\limits_{\mathfrak{C}_0}
\ten{\mathcal{Q}}_{\alpha}\tilde{\vec{\mu}}_n\otimes\vec{D}_{\alpha}:\nabla\delta\vec{\mtx{\varphi}} \abs{C}\d s
+
\sum_{s=0,L}
\ten{\mathcal{Q}}_{\alpha}\tilde{\vec{\mu}}_n^s\otimes\vec{D}_{\alpha}: \nabla\delta\mtx{\vec{\varphi}}_s\,\abs{A}
= 0,
\end{aligned}
\end{equation}
%%Let us note that for all~$\vec{v}$ it holds
%%\begin{equation}\label{key}
%%\begin{aligned}
%%\left(\ten{\Id}-\frac{1}{2}\fib{\ten{R}}\ten{P}_{12}\fib{\ten{R}}\tp\right) & \VPTen{\vec{v}}\fib{\ten{R}}\ten{P}_{12} \\
%%&=
%%\left(\frac{1}{2}\fib{\ten{R}}\ten{P}_{12}\fib{\ten{R}}\tp + \vec{d}_3\otimes\vec{d}_3\right)\VPTen{\vec{d}_{\alpha}}\tp\vec{v}\otimes\vec{D}_{\alpha}
%%\\
%%&=
%%\underbrace{\left(\frac{1}{2}\vec{d}_2\otimes\vec{d}_3 - \vec{d}_3\otimes\vec{d}_2\right)}_{\ten{\mathcal{P}}_1}\vec{v}\otimes\vec{D}_1
%%+
%%\underbrace{\left(-\frac{1}{2}\vec{d}_1\otimes\vec{d}_3 + \vec{d}_3\otimes\vec{d}_1\right)}_{\ten{\mathcal{P}}_2}\vec{v}\otimes\vec{D}_2
%%\\
%%&=
%%(\vec{v}\cdot\vec{d}_1)\vec{d}_3\otimes\vec{D}_2  - (\vec{v}\cdot\vec{d}_2)\vec{d}_3\otimes\vec{D}_1 + (\vec{v}\cdot\vec{d}_3)\frac{\vec{d}_2\otimes\vec{D}_1-\vec{d}_1\otimes\vec{D}_2}{2}
%%\end{aligned}
%%\end{equation}
%%Besides, according to~\eqref{eq:new:LM_matrix}, we have
%%\begin{equation}\label{key}
%%\begin{aligned}
%%\fib{\ten{R}}\ten{P}_{12} & \sym{\fib{\vec{R}}\tp\ten{\Sigma}}\ten{P}_{12}
%%\\
%%&=
%%\tilde{\mu}_n\left(\vec{d}_1\otimes\vec{D}_1+\vec{d}_2\otimes\vec{D}_2\right)
%%+
%%\tilde{\mu}_{s,1}\left(\vec{d}_1\otimes\vec{D}_1-\vec{d}_2\otimes\vec{D}_2\right)
%%+
%%\tilde{\mu}_{s,2}\left(\vec{d}_2\otimes\vec{D}_1+\vec{d}_1\otimes\vec{D}_2\right)
%%\\
%%&=
%%\underbrace{\left(\vec{d}_1\otimes\vec{d}_1 + \vec{d}_1\otimes\vec{d}_2 + \vec{d}_2\otimes\vec{d}_3\right)}_{\ten{\mathcal{Q}}_1}\tilde{\vec{\mu}}^{sym}\otimes\vec{D}_1
%%\\
%%&+
%%\underbrace{\left(\vec{d}_2\otimes\vec{d}_1 - \vec{d}_2\otimes\vec{d}_2 + \vec{d}_1\otimes\vec{d}_3\right)}_{\ten{\mathcal{Q}}_2}\tilde{\vec{\mu}}^{sym}\otimes\vec{D}_2,
%%%&=
%%%(\tilde{\vec{\mu}}^{sym}\cdot\vec{d}_1)\vec{d}_1\otimes\vec{D}_1
%%%+
%%%(\tilde{\vec{\mu}}^{sym}\cdot\vec{d}_2\vec{d}_2\otimes\vec{D}_2
%%%+
%%%(\tilde{\vec{\mu}}^{sym}\cdot\vec{d}_3)\frac{\vec{d}_2\otimes\vec{D}_1+\vec{d}_1\otimes\vec{D}_2}{2}
%%%\\
%%%&=
%%%\underbrace{\left(\vec{d}_1\otimes\vec{d}_1 + \frac{1}{2}\vec{d}_2\otimes\vec{d}_3\right)}_{\ten{\mathcal{Q}}_1}\tilde{\vec{\mu}}^{sym}\otimes\vec{D}_1
%%%+
%%%\underbrace{\left(\vec{d}_2\otimes\vec{d}_2 + \frac{1}{2}\vec{d}_1\otimes\vec{d}_3\right)}_{\ten{\mathcal{Q}}_2}\tilde{\vec{\mu}}^{sym}\otimes\vec{D}_2,
%%\end{aligned}
%%\end{equation}
%%where $
%%\tilde{\vec{\mu}}^{sym} = \tilde{\mu}_n\vec{d}_1 + \tilde{\mu}_{s,1}\vec{d}_2 + \tilde{\mu}_{s,2}\vec{d}_3
%%$.
%%%and
%%%\begin{equation}\label{key}
%%%	\sym{\fib{\vec{R}}\tp\ten{\Sigma}} = \begin{bmatrix}
%%%	\tilde{\mu}^{sym}_1 & \tilde{\mu}^{sym}_3\\
%%%	\tilde{\mu}^{sym}_3 & \tilde{\mu}^{sym}_2
%%%	\end{bmatrix}.
%%%\end{equation}
%%Then, we obtain after integration by parts and some tedious, but straight forward manipulations
%%\begin{equation}\label{eq:new:sys:matrix_condense3}
%%\begin{aligned}
%%\int\limits_{\mtx{\Omega}} &\left(\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}}- \vec{B}_{ext}\cdot\delta\vec{\varphi}\right) \d V 
%%-
%%\int\limits_{\partial\Omega_{N}} \!\!\vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d S
%%+
%%\int\limits_{\mathfrak{C}_0}\left(\mathfrak{n}\otimes\vec{D}_3 : \nabla\delta\mtx{\vec{\varphi}}
%%-
%%\bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}\right)\d s  \\
%%&
%%+
%%\int\limits_{\mathfrak{C}_0}
%%\left[\ten{\mathcal{P}}_{\alpha}\mathfrak{m}\otimes\vec{D}_\alpha\otimes\vec{D}_3\right]\,\vdots\,\nabla^2\delta\mtx{\vec{\varphi}}
%%\d s
%%+ \int\limits_{\mathfrak{C}_0}
%%\biggl[\ten{\mathcal{P}}_{\alpha}^\prime\mathfrak{m}
%%-\ten{\mathcal{P}}_{\alpha}\left(\tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}} +\bar{\tilde{\vec{m}}}\right)
%%\biggl]\otimes\vec{D}_{\alpha}:\nabla\delta\mtx{\vec{\varphi}}\,\d s
%%\\
%%&
%%+ \frac{1}{2}\,\int\limits_{\mathfrak{C}_0}
%%\ten{\mathcal{Q}}_{\alpha}\tilde{\vec{\mu}}^{sym}\otimes\vec{D}_{\alpha}:\nabla\delta\vec{\mtx{\varphi}} \abs{C}\d s
%%+
%%\frac{1}{2} \sum_{s=0,L}
%%\ten{\mathcal{Q}}_{\alpha}\tilde{\vec{\mu}}^{sym}_s\otimes\vec{D}_{\alpha}: \nabla\delta\mtx{\vec{\varphi}}_s\,\abs{A}
%%= 0,
%%\end{aligned}.
%%\end{equation}
Let us now introduce $\vec{\eta}(s)$ satisfying
\begin{equation}\label{eq:DiffEq_eta}
\begin{aligned}
\vec{\eta}^\prime + \tilde{\vec{\mu}}_n \abs{C} &= 0, \\
\vec{\eta}(0) =\abs{A}\tilde{\vec{\mu}}_n^0, \quad & \vec{\eta}(L) = \abs{A}\tilde{\vec{\mu}}_n^L.
\end{aligned}
\end{equation}
\rev{Why is it possible ? Consistency equation ?}

Hence, after integration by parts, the final condensed system writes:
\begin{equation}\label{eq:new:sys:matrix_very_condense}
\begin{aligned}
\int\limits_{\mtx{\Omega}_0} &\biggl(\underbrace{\drv{\mtx{\Psi}}{\ten{\mtx{F}}}}_{\vec{P}}:\nabla\delta\vec{\mtx{\varphi}}- \vec{B}_{ext}\cdot\delta\vec{\varphi}\biggl) \d V 
-
\int\limits_{\partial\Omega_{N}} \!\!\vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d S
+
\int\limits_{\mathfrak{C}_0}\biggl(\underbrace{\mathfrak{n}\otimes\vec{D}_3}_{\vec{P}^{\mathfrak{n}}} : \nabla\delta\mtx{\vec{\varphi}}
-
\bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}\biggl)\d s  \\
&
+
\int\limits_{\mathfrak{C}_0}
\underbrace{\left[\left(\ten{\mathcal{P}}_{\alpha}\mathfrak{m}+\ten{\mathcal{Q}}_{\alpha}\vec{\eta}\right)\otimes\vec{D}_\alpha\otimes\vec{D}_3\right]}_{\mathfrak{P}}\,\vdots\,\nabla^2\delta\mtx{\vec{\varphi}}
\d s
\\
&+
\int\limits_{\mathfrak{C}_0}
\underbrace{\left[\ten{\mathcal{P}}_{\alpha}^\prime\mathfrak{m}
+ \ten{\mathcal{Q}}_{\alpha}^\prime\vec{\eta}
-\ten{\mathcal{P}}_{\alpha}\left(\tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}} +\bar{\tilde{\vec{m}}}\right)
\right]\otimes\vec{D}_{\alpha}}_{\vec{P}^{\mathfrak{m}}}:\nabla\delta\mtx{\vec{\varphi}}\,\d s
= 0,
\end{aligned}.
\end{equation}
such that we can write in a more compact fashion
\begin{equation}
\begin{aligned}
\int\limits_{\mtx{\Omega}_0}\biggl(\vec{P}:\nabla\delta\vec{\mtx{\varphi}} - &\vec{B}_{ext}\cdot\delta\vec{\varphi}\biggl) \d V -
\int\limits_{\partial\Omega_{N}} \!\!\vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d A +\\
&\int\limits_{\mathfrak{C}_0}\biggl(\mathfrak{P}\,\vdots\,\nabla^2\delta\mtx{\vec{\varphi}} + (\vec{P}^{\mathfrak{n}}+\vec{P}^{\mathfrak{m}} - \vec{P}):\nabla\delta\vec{\mtx{\varphi}} - 
(\bar{\tilde{\vec{n}}}-\vec{B}_{ext}) \cdot \delta\mtx{\vec{\varphi}}\biggl)\d S = 0.
\end{aligned}
\end{equation}
supplemented with constitutive equations~\eqref{eq:constitutive_n}-\eqref{eq:constitutive_m} and coupling constraints
\begin{align}\label{key}
\int\limits_{\mathfrak{C}_0}
\big(\vec{F}_{c}\vec{D}_{1}-\vec{d}_{1}\big)\cdot\delta\tilde{\vec{\mu}}_1\d s &= 0,\\
\int\limits_{\mathfrak{C}_0}
\big(\vec{F}_{c}\vec{D}_{2}-\vec{d}_{2}\big)\cdot\delta\tilde{\vec{\mu}}_2\d s &= 0.
\end{align}
Besides,
\begin{equation}\label{key}
	\ten{\mathcal{P}}_{\alpha}^\prime = \VPTen{\fib{\vec{R}}\vec{\kappa}}\ten{\mathcal{P}}_{\alpha} - \ten{\mathcal{P}}_{\alpha}\VPTen{\fib{\vec{R}}\vec{\kappa}},
	\qquad
	\ten{\mathcal{Q}}_{\alpha}^\prime = \VPTen{\fib{\vec{R}}\vec{\kappa}}\ten{\mathcal{Q}}_{\alpha} - \ten{\mathcal{Q}}_{\alpha}\VPTen{\fib{\vec{R}}\vec{\kappa}}.
\end{equation}
\rev{Please, double check whether it's correct.}

Here, we now obtain an explicit representation for the third order stress tensor introduced in \eqref{eq:secondGradient} as
\begin{equation}
\mathfrak{P} = \left(\ten{\mathcal{P}}_{\alpha}\mathfrak{m}+\ten{\mathcal{Q}}_{\alpha}\vec{\eta}\right)\otimes\vec{D}_\alpha\otimes\vec{D}_3 \; \delta_{\fib{\vec{\varphi}}_0(\mathfrak{C}_0)}(\X),
\end{equation}
which emanates from the condensation of the moment equation of the beams. Note that this term directly depends on the resultant torque~$\mathfrak{m}$, derived from, e.g. \eqref{eq:simpleMat}, which is written in terms of the second and the polar moment of area, respectively.
Above, $\delta_{\fib{\vec{\varphi}}_0(\mathfrak{C}_0)}(\X)$ stands for the line Dirac delta function on~$\fib{\vec{\varphi}}_0(\mathfrak{C}_0)$.

\rev{Why we have a special notation for $[0,L]$ and nothing for $\fib{\vec{\varphi}}_0([0,L])$ ? }



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Legacy
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{comment}
	
	Next, we assume that $\tilde{\vec{\mu}}$ is a combination of torque and pressure (i.e.\ we neglect the shear)
	\begin{equation}\label{eq:key4}
	\tilde{\vec{\mu}}(\theta^{\alpha},s) = \vec{\mu}_{\tau}(s)\times\fib{\vec{R}}(s)\,\vec{N}(\theta^{\alpha}) + \mu_{n}(s)\,\fib{\vec{R}}(s)\,\vec{N}(\theta^{\alpha}),
	\end{equation}
	where $\vec{N}=(\theta^{\alpha}\,\vec{D}_{\alpha})/\|\theta^{\alpha}\,\vec{D}_{\alpha}\|\big|_{\Circ(s)}$ is the unit outer normal to the interface in the reference configuration. This term can be rewritten using $\vec{N}=\vec{D}_1\,\cos\theta + \vec{D}_2\,\sin\theta$, where $\cos\theta = \theta^{1}\,\vec{D}_{1}\cdot\theta^{2}\,\vec{D}_{2}/(\|\theta^{1}\,\vec{D}_{1}\|\|\theta^{2}\,\vec{D}_{2}\|)$, such that
	\begin{equation}
	\delta\Pi_{C} = \delta \int\limits_{\mathfrak{C}_0} \int\limits_{C(s)}\left(\bar{\vec{\mu}} + \vec{\mu}_{\tau}\times\fib{\vec{R}}\,\vec{N} + \mu_{n}\,\fib{\vec{R}}\,\vec{N}\right)
	\cdot\big( (\vec{x}_{c} + \vec{F}_{c}\,\theta^{\alpha}\,\vec{D}_{\alpha}) -(\tilde{\vec{\varphi}} + \theta^{\alpha}\,\vec{d}_{\alpha})\big)\d C\d s.
	\end{equation}
	Regarding that
	\begin{equation}
	\int\limits_{C(s)}\theta^{\alpha}\,\vec{d}_{\alpha}(s)\d C = \vec{0},
	\end{equation}
	holds for an appropriate choice of the coordinate system, we obtain
	\begin{equation}\label{eq:const}
	\delta\Pi_{C} = \delta \int\limits_{\mathfrak{C}_0}\left[\bar{\vec{\mu}}\cdot(\vec{x}_{c} -\tilde{\vec{\varphi}})\int\limits_{C(s)}\d C + 
	\int\limits_{C(s)} \left(\vec{\mu}_{\tau}\times\fib{\vec{R}}\,\vec{N} + \mu_{n}\,\fib{\vec{R}}\,\vec{N}\right)\cdot\left(\big(\vec{F}_{c}-\fib{\vec{R}}\big)\,\theta^{\alpha}\,\vec{D}_{\alpha}\right) \d C\right]\d s.
	\end{equation}
	The first term on the right hand side enforces the position of the centerline of the beam along its counterpart in the continuum via the virtual work of
	\begin{equation}\label{eq:pi1}
	\delta\Pi_C^1 = \delta\int\limits_{\mathfrak{C}_0}\bar{\vec{\mu}}\cdot(\vec{x}_{c} -\tilde{\vec{\varphi}})|C(s)|\d s. 
	\end{equation}
	For the second term follows
	\begin{equation}\label{eq:tan1}
	\int\limits_{C(s)}\left(\vec{\mu}_{\tau}\times\fib{\vec{R}}\,\vec{N}\right)\cdot\left(\big(\vec{F}_{c}-\fib{\vec{R}}\big)\,\theta^{\alpha}\,\vec{D}_{\alpha}\right) \d C =
	\vec{\mu}_{\tau}\cdot\fib{\vec{R}}\int\limits_{C(s)}\left(\vec{N}\times\fib{\vec{R}}\tp\,\vec{F}_{c}\,\vec{N}\right)\|\theta^{\alpha}\,\vec{D}_{\alpha}\|\d C.
	\end{equation}
	Using again the circular parametrization $\vec{N}=\vec{D}_1\cos\theta + \vec{D}_2\sin\theta$ leads to
	\begin{equation}\label{eq:integral2condition}
	\int\limits_{0}^{2\,\pi} \vec{N}\times\bigl(\fib{\vec{R}}\tp\,\vec{F}_{c}\,\vec{N} \bigr)\,\d\theta = 
	2\,\pi\axl\left(\fib{\ten{R}}\tp\,\ten{F}_{c}\,\ten{P}_{12}\right),
	\end{equation}
	where $\ten{P}_{12} = \vec{D}_1\otimes\vec{D}_1 + \vec{D}_2\otimes\vec{D}_2$, see Appendix \ref{app:Axial} for details. Hence, we can conclude that 
	\begin{equation}\label{eq:moments_constrain}
	\begin{aligned}
	\delta\Pi_C^2
	&= \delta\int\limits_{\mathfrak{C}_0}\vec{\mu}_{\tau}\cdot\fib{\ten{R}}\,\axl\left(\fib{\ten{R}}\tp\,\ten{F}_c\,\ten{P}_{12}\right) |C(s)|\d s
	= \delta\int\limits_{\mathfrak{C}_0}\vec{\mu}_{\tau}\cdot\axl\left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right) |C(s)|\d s \\
	&= \int\limits_{\mathfrak{C}_0}\left(
	\delta\vec{\mu}_{\tau}\cdot\axl\left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right) +
	\vec{\mu}_{\tau}\cdot\axl\left(\delta\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp +
	\ten{F}_c\,\ten{P}_{12}\,\delta\fib{\ten{R}}\tp\right)
	\right)|C(s)|\d s.
	\end{aligned}
	\end{equation}
	Hence, the last term in~\eqref{eq:moments_constrain} gives rise to
	\begin{equation}\label{eq:moments_coupling_term2}
	\begin{aligned}
	\vec{\mu}_{\tau}\cdot\axl\left(
	\delta\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right)
	&=
	\frac{1}{2}\,\left[\vec{\mu}_{\tau}\right]_\times :\left( \delta\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right)
	=
	\frac{1}{2}\,\left(\left[\vec{\mu}_{\tau}\right]_\times\,\fib{\ten{R}}\,\ten{P}_{12}\right) : \nabla\delta\mtx{\vec{\varphi}} \\
	&=
	\frac{1}{2}\,\left((\vec{\mu}_{\tau}\times\vec{d}_1)\otimes\vec{D}_1 + (\vec{\mu}_{\tau}\times\vec{d}_2)\otimes\vec{D}_2\right) : \nabla\delta\mtx{\vec{\varphi}}\\
	&=
	\frac{1}{2}\,\left(\vec{\mu}_{\tau}\times\vec{d}_{\alpha}\right) \cdot \left(\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_{\alpha}\right)\,,\quad\alpha\in[1,\,2],
	\end{aligned} 
	\end{equation}
	and
	\begin{equation}\label{eq:moments_coupling_term1}
	\begin{aligned}
	\vec{\mu}_{\tau}\cdot\axl\left(
	\ten{F}_c\,\ten{P}_{12}\,\delta\fib{\ten{R}}\tp\right)
	&=
	\frac{1}{2}\,\left[\vec{\mu}_{\tau}\right]_\times : \left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\,\left[\delta\vec{\phi}\right]_\times\tp\right)
	=
	-\frac{1}{2}\,\left(\left[\vec{\mu}_{\tau}\right]_\times\,\ten{F}_c\,\ten{P}_{12}\fib{\ten{R}}\tp \right): \left[\delta\vec{\phi}\right]_\times\\
	&=
	-\axl\left(\left[\vec{\mu}_{\tau}\right]_\times\,\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right) \cdot \delta\vec{\phi}.
	%\\
	%&=
	%\frac{1}{2}\,\left(\ten{P}_{12}\,\vec{F}_c\tp\,\fib{\vec{R}} - \tr\left(\ten{P}_{12}\,\vec{F}_c\tp\,\fib{\vec{R}}\right)\,\ten{\Id}\right)\tp\,\fib{\ten{R}}\tp\,\vec{\mu}_{\tau} \cdot\delta\vec{\phi}\\
	%&=
	%\frac{1}{2}\,\left(\fib{\vec{R}}\tp\vec{F}_c\ten{P}_{12}\,\fib{\vec{R}}\tp - \left(\vec{d}_1\tp\vec{F}_c\vec{D}_1 + \vec{d}_2\tp\vec{F}_c\vec{D}_2\right)\,\fib{\vec{R}}\tp\right)\vec{\mu}_{\tau}
	%\cdot\delta\vec{\phi},
	\end{aligned} 
	\end{equation}
	
	\begin{remark}
	Note that $\vec{\mu}_{\tau}\times\vec{d}_{\alpha}$ is a bending force applied to the beam surface $\vec{D}_\alpha$ from the matrix. Moreover,
	\begin{equation}\label{key6}
	-\axl\left(\left[\vec{\mu}_{\tau}\right]_\times\,\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right) =
	\left[\vec{d}_1, \, \vec{d}_2,\,  \vec{d}_3\right]
	\begin{bmatrix}
	(\vec{\mu}_{\tau}\times\vec{d}_{3})\cdot\ten{F}_c\,\vec{D}_2 \\
	-(\vec{\mu}_{\tau}\times\vec{d}_{3})\cdot\ten{F}_c\,\vec{D}_1 \\
	(\vec{\mu}_{\tau}\times\vec{d}_{2})\cdot\ten{F}_c\,\vec{D}_1 - (\vec{\mu}_{\tau}\times\vec{d}_{1})\cdot\ten{F}_c\,\vec{D}_2
	\end{bmatrix}
	\end{equation}
	represents the residual moments, i.e.\ projections of the bending forces (e.g. with regard to the first two components of $\mathbb{K}_2$ used in eq. \eqref{eq:simpleMat}),  onto the deformed directors under matrix deformations. It is important to remark, that this potentially over-constrains the system in the case of Bernoulli-Euler beams, as the bending terms are already prescribed by the position constraints in \eqref{eq:pi1}.
	\end{remark}
	The last term in (\ref{eq:const}) reads
	\begin{equation}\label{eq:tan2}
	\int\limits_{C(s)} \mu_{n}\,\left(\fib{\vec{R}}\,\vec{N}\right)\cdot\left(\big(\vec{F}_{c}-\fib{\vec{R}}\big)\,\theta^{\alpha}\,\vec{D}_{\alpha}\right) \d C = 
	\mu_{n}\int\limits_{C(s)}\left(\vec{N}\cdot\left(\fib{\vec{R}}\tp\vec{F}_{c}\,\vec{N}\right)-\vec{N}\cdot\left(\vec{I}\,\vec{N}\right)\right)\|\theta^{\alpha}\vec{D}_{\alpha}\|\d C,
	\end{equation}
	and measures the compression.
	In case of circular cross-section, we obtain from \eqref{eq:tan2} (see Appendix~\ref{app:Axial}) the last constraint
	\begin{equation}\label{eq:pdvApi3}
	\begin{aligned}
	\delta\Pi_C^3 &= \delta\int\limits_{\mathfrak{C}_0}\mu_n \left(\frac{1}{2}\,\tr\left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right)  - 1\right)|C(s)|\d s,\\
	&= \phantom{\delta}\int\limits_{\mathfrak{C}_0}\left[\delta\mu_n \left(\frac{1}{2}\,\tr\left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right)  - 1\right) +\right.\\ 
	&\phantom{=\delta\int\limits_{\mathfrak{C}_0}[[}\left.\frac{\mu_n}{2}\left(\vec{d}_{\alpha}\cdot\left(\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_{\alpha} \right)
	+ 
	\tr\left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\left[\delta\vec{\phi}\right]_\times\tp\right) \right)\right]|C(s)|\d s.
	\end{aligned}
	\end{equation}
	This last equation constrains the volumetric changes of the beam volume. Since classical beam theories do not consider dilatations or contractions of the beam sections, the Poisson ratio used in the constitutive relation \eqref{eq:beamMR} is equal zero, see \cite{ortigosa2016} for further discussions. 
	
	Note that in~\eqref{eq:pdvApi3}, the last term
	\begin{equation}\label{key}
	\int\limits_{\mathfrak{C}_0}
	\frac{\mu_n}{2}\,\tr\left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\left[\delta\vec{\phi}\right]_\times\tp\right)
	\d s
	=
	\int\limits_{\mathfrak{C}_0}
	\mu_n \axl\left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right)\cdot\delta\vec{\phi}
	\d s
	\end{equation}
	corresponds to the first term of~\eqref{eq:moments_constrain} and then vanishes under coupling constraints, i.e. the hydrostatic pressure does not create moments.
	%\rev{This constrain can be useful, if one introduces beam radius~$r(s)$ as additional variable.}
	
	Likewise, we derive in the same way the endpoint constraints
	\begin{align}
	\delta\Pi_A^1 
	&=
	\delta\sum_{s=0,L}\bar{\vec{\mu}}^s\cdot(\vec{x}_{c} -\tilde{\vec{\varphi}})\,|A(s)|,\label{eq:ep:pi1}\\
	\delta\Pi_A^2
	&= \delta\sum_{s=0,L}\vec{\mu}_{\tau}^s\cdot\axl\left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right) |A(s)|,\label{eq:ep:pi2}\\
	\delta\Pi_A^3
	&=
	\delta\sum_{s=0,L}\mu_n^s \left(\frac{1}{2}\tr\left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\,\right) - 1\right)|A(s)|.\label{eq:ep:pi3}
	\end{align}
	
	
	\paragraph{Total system.}
	Finally, we obtain the principle of virtual work for the  coupled matrix/fiber system, hence
	\begin{equation}
	\delta\Pi^{int} + \delta\Pi^{ext} + \delta\fib{\Pi}^{int} + \delta\fib{\Pi}^{ext} + \delta\Pi_C^{(1,2,3)} + \delta\Pi_A^{(1,2,3)} = 0,
	\end{equation}
	with regard to \eqref{eq:pdvA}, \eqref{eq:pdvaBeam} and \eqref{eq:pdvaHW2} along with the virtual work of the coupling conditions in \eqref{eq:pi1}, \eqref{eq:moments_constrain}, \eqref{eq:pdvApi3} and \eqref{eq:ep:pi1}, \eqref{eq:ep:pi2}, \eqref{eq:ep:pi3}. With regard to the matrix material, i.e.\ the variation with respect to $\delta\vec{\varphi}$, we obtain
	\begin{equation}\label{eq:sys:matrix}
	\begin{aligned}
	&\int\limits_{\mtx{\Omega}_0} \drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}} - \vec{B}_{ext}\cdot\delta\vec{\varphi} \d V	-
	\int\limits_{\Gamma^{\sigma}} \vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d A
	+\\
	&\int\limits_{\mathfrak{C}_0}\left(\vec{\bar{\mu}} \cdot \delta\vec{\mtx{\varphi}}
	+
	\frac{1}{2}\,\left(\vec{\mu}_{\tau}\times\vec{d}_{\alpha}+\mu_n\vec{d}_{\alpha}\right)\cdot \left(\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_{\alpha}\right) \right) \abs{C}\d s
	+\\
	&\sum_{s=0,L}|A|\left[\bar{\vec{\mu}}^s\cdot\delta\mtx{\vec{\varphi}}_s\,|A|
	+
	\frac{1}{2}\,\left(\vec{\mu}_{\tau}^s\times\vec{d}_{\alpha}+\mu_n^s\,\vec{d}_{\alpha}\right)\cdot \left(\nabla\delta\mtx{\vec{\varphi}}_s\,\vec{D}_{\alpha}\right)\right] 
	= 0.
	\end{aligned}
	\end{equation}
	Note that $\vec{\mu}_{\tau}\times\vec{d}_3$ does not enter in the matrix equation. The beam contributions  yield
	%\begin{align}
	%	&\int\limits_{\mathfrak{C}_0}-\left({\mathfrak{n}}^{\prime} + \bar{\tilde{\vec{n}}}\right)\cdot\delta\tilde{\vec{\varphi}}
	%	-
	%	 \vec{\bar{\mu}} \cdot \delta\vec{\fib{\varphi}}\abs{C}\d s = 0,  
	%	 \label{eq:sys:load}\\	
	%	&\int\limits_{\mathfrak{C}_0}-\left({\mathfrak{m}}^{\prime} + \tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}}
	%	+
	%	\bar{\tilde{\vec{m}}}\right)\cdot\delta\vec{\phi}
	%	+
	%	\axl\left(-\left[\vec{\mu}_{\tau}\right]_\times\ten{F}_c\ten{P}_{12}\fib{\ten{R}}\tp
	%	+
	%	\mu_n\ten{F}_c\ten{P}_{12}\fib{\ten{R}}\tp\right) \cdot \delta\vec{\phi} \abs{C}\d s = 0,
	%	\label{eq:sys:moments}
	%\end{align}
	%With regard to \eqref{eq:sys:pi2}, the second last term in \eqref{eq:sys:moments} vanish, i.e.\ the hydrostatic pressure does not create moments. Moreover, if we take \eqref{eq:apx:axl2mat} and \eqref{eq:sys:pi3} into account, we obtain for the beam
	\begin{align}
	&\int\limits_{\mathfrak{C}_0}\left({\mathfrak{n}}^{\prime} + \bar{\tilde{\vec{n}}}\right)\cdot\delta\tilde{\vec{\varphi}}
	+
	\vec{\bar{\mu}} \cdot \delta\vec{\fib{\varphi}}\,\abs{C}\d s = 0,  
	\label{eq:sys:load2}\\	
	&\int\limits_{\mathfrak{C}_0}\left({\mathfrak{m}}^{\prime} + \tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}}
	+
	\bar{\tilde{\vec{m}}}\right)\cdot\delta\vec{\phi}
	+
	\left(\ten{\Id}-\frac{1}{2}\,\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp
	\right)\vec{\mu}_{\tau} \cdot \delta\vec{\phi}\, \abs{C}\d s = 0,
	\label{eq:sys:moments2}
	\end{align}
	where the last term in~\eqref{eq:sys:moments2} is written with regards to~\eqref{eq:apx:axl2mat} (see Appendix \ref{app:weird_term}) and~\eqref{eq:sys:pi3}.
	The system~\eqref{eq:sys:matrix}-\eqref{eq:sys:moments2} is supplemented by the constitutive equations
	\begin{align}
	&\int\limits_{\mathfrak{C}_0}\delta{\mathfrak{g}}\cdot\left(\fib{\ten{R}}\,\frac{\partial\tilde{\Psi}(\vec{\Gamma},\vec{K})}{\partial\vec{\Gamma}}-{\mathfrak{n}} \right)\d s = 0,
	\label{eq:constitutive_n}\\
	&\int\limits_{\mathfrak{C}_0}\delta{\mathfrak{k}}\cdot\left(\fib{\ten{R}}\,\frac{\partial\tilde{\Psi}(\vec{\Gamma},\vec{K})}{\partial\vec{K}}-{\mathfrak{m}}\right)\,\text{d}s = 0,
	\label{eq:constitutive_m}
	\end{align}
	the coupling constraints
	\begin{align}
	&\int\limits_{\mathfrak{C}_0}\delta\vec{\bar{\mu}} \cdot\left(\fib{\vec{\varphi}}-\vec{\mtx{\varphi}}\right)\d s = 0,	
	\label{eq:sys:pi1}\\
	&\int\limits_{\mathfrak{C}_0}\delta\vec{\mu}_{\tau}\cdot\axl\left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\,\right) \d s = 0,
	\label{eq:sys:pi2}\\
	&\int\limits_{\mathfrak{C}_0}\delta\mu_n \left(\frac{1}{2}\,\tr\left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\,\right) - 1\right)\d s = 0.
	%	&\int\limits_{\mathfrak{C}_0}\delta\mu_n \left(\frac{1}{2}\left(\vec{d}_{\alpha}\tp\vec{F}_{c}\,\vec{D}_{\alpha}\right) - 1\right)\d s = 0
	\label{eq:sys:pi3}
	\end{align}
	and the beam endpoint conditions at $s=0,L$:
	\begin{align}
	&\mathfrak{n} = \abs{A}\,\bar{\vec{\mu}}^s 
	\label{eq:sys:bc_n}\\
	&\mathfrak{m} = \abs{A}\,\left(\ten{\Id}-\frac{1}{2}\,\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp
	\right)\vec{\mu}_{\tau}^s
	\label{eq:sys:bc_m} \\
	&\fib{\vec{\varphi}} = \vec{\mtx{\varphi}},	
	\label{eq:bc1}\\
	&\axl\left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right) = 0,
	\label{eq:bc2}\\
	&\frac{1}{2}\tr\left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right) = 1.
	\label{eq:bc3}
	\end{align}
	
	\begin{remark}
	Note that
	\begin{align}
	\axl\left(\ten{F}_c\,\ten{P}_{12}\fib{\ten{R}}\tp\,\right)
	&=
	\frac{1}{2}\left[\vec{d}_1,  \vec{d}_2,  \vec{d}_3\right]\cdot\begin{bmatrix} 
	\vec{d}_3\cdot\ten{F}_c\vec{D}_2 \\ 
	-\vec{d}_3\cdot\ten{F}_c\vec{D}_1\\
	\vec{d}_2\cdot\ten{F}_c\vec{D}_1 - \vec{d}_1\cdot\ten{F}_c\vec{D}_2	
	\end{bmatrix},
	\label{eq:remark_constraints_axl}
	\\
	\tr\left(\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right) - 2
	&=
	\vec{d}_1\cdot\left(\ten{F}_c\vec{D}_1 - \vec{d}_1\right) + \vec{d}_2\cdot\left(\ten{F}_c\vec{D}_2 - \vec{d}_d\right),
	\label{eq:remark_constraints_tr}
	\end{align}
	Thus, the constraints~\eqref{eq:sys:pi2},~\eqref{eq:bc2} restrict $\ten{F}_c\vec{D}_{\alpha}$, $\alpha=1,2$ to be orthogonal to~$\vec{d}_3$, that is, the cross-section deformed under the matrix deformation is in the same plane that the deformed beam cross-section.
	The third component in~\eqref{eq:remark_constraints_axl} determines the deformation on that plane.	
	Besides, together with~\eqref{eq:sys:pi3},~\eqref{eq:bc3} it implies $\abs{\ten{F}_c\vec{D}_1 - \vec{d}_1} = \abs{\ten{F}_c\vec{D}_2 - \vec{d}_d}$.
	
	
	\end{remark}
	
	
	If $\delta\vec{\varphi}\big|_{\mathfrak{C}_0}$ is in $\HS_{\delta\fib{\vec{\varphi}}}(\mathfrak{C}_0)$ then using \eqref{eq:sys:pi1}, we can condense \eqref{eq:sys:load} and \eqref{eq:sys:bc_n} to~\eqref{eq:sys:matrix}. Hence, \eqref{eq:sys:load2} can be rewritten as
	\begin{equation}
	\int\limits_{\mathfrak{C}_0}\left({\mathfrak{n}}^{\prime} + \bar{\tilde{\vec{n}}}\right)\cdot\delta\vec{\varphi}
	+ \vec{\bar{\mu}} \cdot \delta\vec{\varphi}\abs{C}\d s = 0.
	\end{equation}
	Insertion in \eqref{eq:sys:matrix} and subsequent differentiation by parts, \eqref{eq:sys:bc_n} yields
	\paragraph{Reduced system.} If $\delta\vec{\varphi}\big|_{\mathfrak{C}_0}$ is in $\HS_{\delta\fib{\vec{\varphi}}}(\mathfrak{C}_0)$, then we can condense \eqref{eq:sys:load2} and \eqref{eq:sys:bc_n} to the matrix equation~\eqref{eq:sys:matrix}, which leads after integration by parts to
	\begin{equation}\label{eq:sys:matrix_condense}
	\begin{aligned}
	&\int\limits_{\mtx{\Omega}} \left(\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}}- \vec{B}_{ext}\cdot\delta\vec{\varphi}\right) \d V
	-
	\int\limits_{\partial\Omega_{N}} \!\!\vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d S
	+
	\int\limits_{\mathfrak{C}_0}\left(\mathfrak{n}\otimes\vec{D}_3 : \nabla\delta\mtx{\vec{\varphi}}
	-
	\bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}\right)\d s
	\\&+
	\int\limits_{\mathfrak{C}_0}
	\frac{1}{2}\,\left(\vec{\mu}_{\tau}\times\vec{d}_{\alpha}+\mu_n\vec{d}_{\alpha}\right)\cdot \nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_{\alpha} \abs{C}\d s
	+
	\sum_{s=0,L}
	\frac{1}{2}\,\left(\vec{\mu}_{\tau}^s\times\vec{d}_{\alpha}+\mu_n^s\vec{d}_{\alpha}\right)\cdot \nabla\delta\mtx{\vec{\varphi}}_s\,\vec{D}_{\alpha}\, |A|
	= 0.
	\end{aligned}
	\end{equation}
	Thus, we have eliminated the set of Lagrange multipliers $\bar{\vec{\mu}}$.
	% using \eqref{eq:sys:load}.
	To eliminate the second set of Lagrange multipliers $\vec{\mu}_{\tau}$, we have to
	%make use of \eqref{eq:sys:pi2} along with \eqref{eq:apx:axl2mat} and 
	assume that
	%\begin{equation}\label{eq:restrictionSpace}
	$\ten{A}\tp\axl\left(
	\delta\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right)
	%\qquad 
	\in \HS_{\delta\vec{\phi}}$
	for all~$\delta\vec{\varphi}\in \HS_{\delta\vec{\varphi}}$,
	%\end{equation}
	where we denote $\ten{A}=\left(\ten{\Id}-\frac{1}{2}\ten{F}_c\ten{P}_{12}\fib{\ten{R}}\tp\right)^{-1}$.
	%i.e.\ the variation of $\vec{\varphi}$ is in the space $\HS_{\delta\vec{\phi}}$ with respect to the momentum constraints in \eqref{eq:sys:pi2}. Insertion in \eqref{eq:sys:moments2} allows us to write
	In this case, substituting $\delta\vec{\phi}=\ten{A}\tp\axl\left(
	\delta\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right)$ in~\eqref{eq:sys:moments2}, we obtain
	\begin{equation}
	\int\limits_{\mathfrak{C}_0}
	\left[
	\ten{A}\,
	\left({\mathfrak{m}}^{\prime} + \tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}}
	+
	\bar{\tilde{\vec{m}}}\right)
	+
	\abs{C}\vec{\mu}_{\tau}
	\right]\cdot \axl\left(
	\delta\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right)
	\d s = 0.
	\end{equation}
	Thus, \eqref{eq:sys:matrix} yields
	\begin{equation}\label{eq:sys:matrix_condense2}
	\begin{aligned}
	&\int\limits_{\mtx{\Omega}} \left(\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}}- \vec{B}_{ext}\cdot\delta\vec{\varphi}\right) \d V
	-
	\int\limits_{\partial\Omega_{N}} \!\!\vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d S
	+
	\int\limits_{\mathfrak{C}_0}\left(\mathfrak{n}\otimes\vec{D}_3 : \nabla\delta\mtx{\vec{\varphi}}
	-
	\bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}\right)\d s\\
	&- \int\limits_{\mathfrak{C}_0}
	\left[\ten{A}\left({\mathfrak{m}}^{\prime} + \tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}} + \bar{\tilde{\vec{m}}}\right)\,\right]
	\cdot\axl\left(\delta\ten{F}_c\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right)\d s \\
	& + \int\limits_{\mathfrak{C}_0}
	\frac{1}{2}\,\mu_n\vec{d}_{\alpha}\cdot\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_{\alpha} \abs{C}\d s +
	\sum_{s=0,L} \frac{1}{2}\,\left(\vec{\mu}_{\tau}^s\times\vec{d}_{\alpha}+\mu_n^s\vec{d}_{\alpha}\right)\cdot \nabla\delta\mtx{\vec{\varphi}}_s\,\vec{D}_{\alpha}\, |A|
	= 0.
	\end{aligned}
	\end{equation}
	Finally, we obtain after integration by parts and some tedious, but straight forward manipulations
	\begin{equation}\label{eq:sys:matrix_condense3}
	\begin{aligned}
	\int\limits_{\mtx{\Omega}} &\left(\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}}- \vec{B}_{ext}\cdot\delta\vec{\varphi}\right) \d V 
	-
	\int\limits_{\partial\Omega_{N}} \!\!\vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d S
	+
	\int\limits_{\mathfrak{C}_0}\left(\mathfrak{n}\otimes\vec{D}_3 : \nabla\delta\mtx{\vec{\varphi}}
	-
	\bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}\right)\d s  \\
	+\frac{1}{2}\int\limits_{\mathfrak{C}_0}&
	\,\left[\left(\ten{A}\,\mathfrak{m}\times\tilde{\vec{R}}\vec{D}_{\alpha}\right)\otimes\vec{D}_\alpha\otimes\vec{D}_3\right]\,\vdots\,\nabla^2\delta\mtx{\vec{\varphi}}
	+ \biggl[\left(\ten{A}\,\mathfrak{m}\times\tilde{\vec{R}}\vec{D}_{\alpha}\right)\otimes\nabla\vec{D}_\alpha\,\vec{D}_3 \\
	& -\left(\nabla\left(\left[\vec{d}_\alpha\right]_\times\,\ten{A}\right):(\mathfrak{m}\otimes\vec{D}_3)\right)\otimes\vec{D}_\alpha
	-\left(\ten{A}\,\left(\tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}} +\bar{\tilde{\vec{m}}}\right)\times\vec{d}_\alpha\right)\otimes\vec{D}_\alpha
	\biggl]:\nabla\delta\mtx{\vec{\varphi}}\,\d s \\
	+\int\limits_{\mathfrak{C}_0}&
	\frac{1}{2}\,\mu_n\vec{d}_{\alpha}\cdot\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_{\alpha} \abs{C}\d s +
	\sum_{s=0,L} \frac{1}{2}\,\mu_n^s\vec{d}_{\alpha}\cdot \nabla\delta\mtx{\vec{\varphi}}_s\,\vec{D}_{\alpha}\, |A|
	= 0.
	\end{aligned}
	\end{equation}
	Here, we now obtain an explicit representation for the third order stress tensor introduced in \eqref{eq:secondGradient} as
	\begin{equation}
	\mathfrak{P} = \left(\ten{A}\,\mathfrak{m}\times\tilde{\vec{R}}\vec{D}_{\alpha}\right)\otimes\vec{D}_\alpha\otimes\vec{D}_3,
	\end{equation}
	which emanates from the condensation of the moment equation of the beams. Note that this term directly depends on the resultant contact torque, derived from, e.g. \eqref{eq:simpleMat}, which is written in terms of the second and the polar moment of area, respectively. 
	
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}

\begin{equation}
\begin{aligned}
\ten{A}\,\mathfrak{m}'\cdot\axl\left(\delta{\ten{F}_c}\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right)&=\frac{1}{2}\,\ten{A}\,\mathfrak{m}'\times\vec{d}_\alpha\,\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_\alpha\\
&=-\frac{1}{2}\,\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}'\,\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_\alpha\\
&=\frac{1}{2}\,\varepsilon_{ijk}\,\left[\ten{A}\right]_{jl}\,\left[\mathfrak{m}'\right]_{l}\,\left[\vec{d}_\alpha\right]_{k}\,\left[\nabla\delta\mtx{\vec{\varphi}}\right]_{iM}\,\left[\vec{D}_\alpha\right]_{M}\\
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
-\frac{1}{2}\,\nabla\left[\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}\,\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_\alpha\right]\,\vec{D}_3=\,&-\frac{1}{2}\,\nabla\left[\hat{\vec{d}}_\alpha\,\ten{A}\right]\,\vec{D}_3\,\mathfrak{m}\,\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_\alpha-\frac{1}{2}\,\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}'\,\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_\alpha\\
&-\frac{1}{2}\,\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}\,\nabla^2\delta\mtx{\vec{\varphi}}:\vec{D}_\alpha\otimes\vec{D}_3-\frac{1}{2}\,\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}\,\nabla\delta\mtx{\vec{\varphi}}\,\nabla\vec{D}_\alpha\,\vec{D}_3
\end{aligned}
\end{equation}
Boundary condition drops out:
\begin{equation}
\begin{aligned}
-\frac{1}{2}\,\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}'\,\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_\alpha=\,&\frac{1}{2}\,\nabla\left[\hat{\vec{d}}_\alpha\,\ten{A}\right]\,\vec{D}_3\,\mathfrak{m}\,\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_\alpha+\frac{1}{2}\,\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}\,\nabla^2\delta\mtx{\vec{\varphi}}:\vec{D}_\alpha\otimes\vec{D}_3\\
&+\frac{1}{2}\,\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}\,\nabla\delta\mtx{\vec{\varphi}}\,\nabla\vec{D}_\alpha\,\vec{D}_3\\
=&\,\frac{1}{2}\,\left[\nabla\left(\hat{\vec{d}}_\alpha\,\ten{A}\right):(\mathfrak{m}\otimes\vec{D}_3)\otimes\vec{D}_\alpha+\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}\otimes\nabla\vec{D}_\alpha\,\vec{D}_3\right]:\nabla\delta\mtx{\vec{\varphi}}\\
&+\frac{1}{2}\,\left[\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}\otimes\vec{D}_\alpha\otimes\vec{D}_3\right]:\cdot\nabla^2\delta\mtx{\vec{\varphi}}
\end{aligned}
\end{equation}







\begin{equation}\label{eq:sys:matrix_condense3}
\begin{aligned}
&\int\limits_{\mtx{\Omega}} \left(\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}}- \vec{B}_{ext}\cdot\delta\vec{\varphi}\right) \d V
-
\int\limits_{\partial\Omega_{N}} \!\!\vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d S
+
\int\limits_{\mathfrak{C}_0}\left(\mathfrak{n} \cdot \nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_3
-
\bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}\right)\d s\\
& + \int\limits_{\mathfrak{C}_0}
\ten{A}\,\mathfrak{m}\cdot\axl\left(\nabla^2\delta\mtx{\vec{\varphi}}\,\vec{D}_3\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right)\\
&-\ten{A}\,\left(-\frac{1}{2}\nabla\ten{F}_c\vec{D}_3\ten{P}_{12}\fib{\ten{R}}\tp\right)\ten{A}\,\mathfrak{m}\cdot\axl\left(\nabla\delta\mtx{\vec{\varphi}}\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right)\\
&-\ten{A}\,\left(\tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}} +\bar{\tilde{\vec{m}}}\right)\cdot
\axl\left(\nabla\delta\mtx{\vec{\varphi}}\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right)\d s \\
& + \int\limits_{\mathfrak{C}_0}
\frac{1}{2}\,\mu_n\vec{d}_{\alpha}\cdot\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_{\alpha} \abs{C}\d s +
\sum_{s=0,L} \frac{1}{2}\,\mu_n^s\vec{d}_{\alpha}\cdot \nabla\delta\mtx{\vec{\varphi}}_s\,\vec{D}_{\alpha}\, |A|
= 0.
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
\ten{A}\,\mathfrak{m}'\cdot\axl\left(\delta{\ten{F}_c}\,\ten{P}_{12}\,\fib{\ten{R}}\tp\right)&=\frac{1}{2}\,\ten{A}\,\mathfrak{m}'\times\vec{d}_\alpha\,\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_\alpha\\
&=-\frac{1}{2}\,\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}'\,\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_\alpha\\
&=\frac{1}{2}\,\varepsilon_{ijk}\,\left[\ten{A}\right]_{jl}\,\left[\mathfrak{m}'\right]_{l}\,\left[\vec{d}_\alpha\right]_{k}\,\left[\nabla\delta\mtx{\vec{\varphi}}\right]_{iM}\,\left[\vec{D}_\alpha\right]_{M}\\
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
-\frac{1}{2}\,\nabla\left[\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}\,\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_\alpha\right]\,\vec{D}_3=\,&-\frac{1}{2}\,\nabla\left[\hat{\vec{d}}_\alpha\,\ten{A}\right]\,\vec{D}_3\,\mathfrak{m}\,\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_\alpha-\frac{1}{2}\,\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}'\,\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_\alpha\\
&-\frac{1}{2}\,\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}\,\nabla^2\delta\mtx{\vec{\varphi}}:\vec{D}_\alpha\otimes\vec{D}_3-\frac{1}{2}\,\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}\,\nabla\delta\mtx{\vec{\varphi}}\,\nabla\vec{D}_\alpha\,\vec{D}_3
\end{aligned}
\end{equation}
Boundary condition drops out:
\begin{equation}
\begin{aligned}
-\frac{1}{2}\,\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}'\,\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_\alpha=\,&\frac{1}{2}\,\nabla\left[\hat{\vec{d}}_\alpha\,\ten{A}\right]\,\vec{D}_3\,\mathfrak{m}\,\nabla\delta\mtx{\vec{\varphi}}\,\vec{D}_\alpha+\frac{1}{2}\,\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}\,\nabla^2\delta\mtx{\vec{\varphi}}:\vec{D}_\alpha\otimes\vec{D}_3\\
&+\frac{1}{2}\,\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}\,\nabla\delta\mtx{\vec{\varphi}}\,\nabla\vec{D}_\alpha\,\vec{D}_3\\
=&\,\frac{1}{2}\,\left[\nabla\left(\hat{\vec{d}}_\alpha\,\ten{A}\right):(\mathfrak{m}\otimes\vec{D}_3)\otimes\vec{D}_\alpha+\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}\otimes\nabla\vec{D}_\alpha\,\vec{D}_3\right]:\nabla\delta\mtx{\vec{\varphi}}\\
&+\frac{1}{2}\,\left[\hat{\vec{d}}_\alpha\,\ten{A}\,\mathfrak{m}\otimes\vec{D}_\alpha\otimes\vec{D}_3\right]:\cdot\nabla^2\delta\mtx{\vec{\varphi}}
\end{aligned}
\end{equation}



\end{comment}





\begin{comment}

\textcolor{blue}{We have two questions:
\begin{itemize}
\item Is $\delta\vec{\varphi}\big|_{\mathfrak{C}_0}$ is in $\HS_{\delta\fib{\vec{\varphi}}}(\mathfrak{C}_0)$? Stefan and I are concerned about this, if we use a collocation type method.
\item For the condensation, we have to use the beam equations in their strong form (we show this below), i.e.\ as you mentioned a few week ago, this is a different requirement as provided until now.
\end{itemize}}

\rev{Thus, we've eliminated $\bar{\vec{\mu}}$ and the equation~\eqref{eq:sys:load} is not needed anymore.}

\rev{
Notations: 
we have to write it in more compact way.
Also we should shorten endpoints terms, maybe using Einstein summation.
Besides, directional derivatives~$\nabla\vec{v}\,\vec{D}_i$ could be written as $\frac{\partial}{\partial \vec{D}_i}\vec{v}$.
}

Moments equation~\eqref{eq:sys:moments} can also be condensed, see~\eqref{eq:condensed_moments} in Appendix~\ref{app:condensed_moments}.
Thus, for the unknowns $\vec{\mtx{\varphi}}$, $\vec{\phi}$, $\mu_{n}$ and $\mathfrak{n}$, $\mathfrak{m}$, we have \eqref{eq:condensed_moments}, \eqref{eq:sys:pi2}, \eqref{eq:sys:pi3} and \eqref{eq:constitutive_n}-\eqref{eq:constitutive_m}.

\end{comment}




==> sections/sec_Coupling4.tex <==


In this work, starting from a surface-to-volume coupling formulation for the matrix/beam system, we derive a reduced surrogate model, where the new coupling constraints defined on the beam centerline involve the deformation gradient and transfer both the linear forces and the moments of the beam to the matrix. 
The reduced model is based on the following assumptions:
\begin{itemize}
\item[A1. \textit{Overlapping domains}.] 
The matrix continuum is extended inside the beam domain.
This yields a modeling error due to additional stiffness, which depends on the fiber radius~$r$ and the ratio of the matrix stiffness to the fiber stiffness.
Such type of modeling error was studied for diffusion problem in~\cite{koppl2018mathematical}.

\item[A2. \textit{Form of the coupling force}.]
We make an assumption on the form of the coupling force (Lagrange multiplier), such that, applied to a beam cross-section, it presents the mean force, couple stresses, shear and dilatation forces.

\item[A3. \textit{Sufficient regularity}.] 	
We assume additional regularity of the solution, such that the traces of deformation and of its gradient are defined on the beam centerline. We will then truncate Taylor expansion of the deformation in the cross-section with respect to the radius~$r$. Considering all terms up to the linear part yields a modeling error of order~$\O\left(r^2\right)$.
\end{itemize}


\input{tikz/coupled_system/coupled_system}

Let us consider the matrix/beam system illustrated in Figure \ref{fig:matrix-fiber}.
The coupling conditions are defined via Lagrange multipliers on the beam mantle~$\Gamma_C$ and at the end faces $A_0$, $A_L$ (see Figure~\ref{fig:fiber3D_ref}).
The work associated to the coupling forces over the whole matrix/beam interface reads
\begin{equation}\label{eq:CouplingTerm}
\Pi_{\Gamma} = \int\limits_{\partial\tilde{\Omega}}\vec{\mu}\cdot(\vec{\varphi}-\fib{\vec{x}})\d A =\Pi_{C} + \Pi_{A},
\end{equation}
where
\begin{equation}\label{eq:coupling_term_init}
\Pi_{C} = \int\limits_{\mathfrak{C}_0} \int\limits_{C(s)}\vec{\mu}\cdot(\vec{\varphi}-\fib{\vec{x}})\d C\d s,
\qquad
\Pi_{A} = 
%\sum_{s=0,L} 
\EC{\int\limits_{A_s}\vec{\mu}\cdot(\vec{\varphi}-\fib{\vec{x}})\d A}.
\end{equation}
Above, $A_s$ and $C(s)$ are respectively the beam cross-section and its boundary corresponding to the arc length $s$.
The area and the circumference of the cross-section are respectively denoted as $\abs{A} := \pi\, r^2$ and $\abs{C} := 2\,\pi\, r$.
Here and further, for the sake of shortness, we use the following abuse of notations: for any function $f(\X)$ defined in~$\Omega$,
$f(\theta^\alpha, s):=f(\fib{\X}(\theta^\alpha, s))$ means the restriction of $f$ onto the beam domain~$\fib{\Omega}$ in convective coordinates; and $f(s):=f(\fib{\vec{\varphi}}_0(s))$, $s\in\mathfrak{C}_0$, is understood in the sense of the trace $f|_{\mathfrak{C}_0}$ of $f$ on the beam centerline.

\input{tikz/fiber3D/fiber3D}

\subsection{Coupling term model}
The Lagrange multiplier~$\vec{\mu}$, physically interpreted as the interface load, is defined on the beam mantle $\Gamma_C = \lbrace (r\,\cos\theta, r\,\sin\theta, s) \; | \, s\in[0,L], \theta\in[0, 2\,\pi]\rbrace$, where $r$ is the beam radius and $\theta=\arctan(\theta^2/\theta^1)$ denotes the angle along the beam cross-section circumference.
Thus, $\vec{\mu}=\vec{\mu}(\theta, s)$ can be decomposed in Fourier series as periodic function of the angle~$\theta\in[0, 2\,\pi]$.
Here, we base our reduced model on truncation of this series after the first two terms.
That is, we assume the interface load in the form:
\begin{equation}\label{eq:LM_mu}
\vec{\mu}(\theta, s) = \bar{\vec{\mu}}(s) + \tilde{\vec{\mu}}_1(s)\,\cos\theta + \tilde{\vec{\mu}}_2(s)\,\sin\theta,
\end{equation}
where $\bar{\vec{\mu}}(s) = \frac{1}{2\,\pi\, r}\int_{0}^{2\pi}\vec{\mu}(\theta, s)\d\theta$ is the mean cross-sectional load, and $\tilde{\vec{\mu}}_{\alpha}$, $\alpha=1,2$, are respectively the first cosine and sine Fourier coefficients of $\vec{\mu}$.
These two terms compose the load fluctuation
\begin{equation}\label{eq:new:mu_tilde}
	\tilde{\vec{\mu}}(\theta,s)
	:= \ten{\Sigma}(s)\,\vec{N}(\theta)
	= \tilde{\vec{\mu}}_1(s)\,\cos\theta + \tilde{\vec{\mu}}_2(s)\,\sin\theta,
\end{equation}
where $\ten{\Sigma}=\tilde{\vec{\mu}}_{\alpha}\otimes\vec{D}_{\alpha}$ denotes the interface stress tensor, and $\vec{N}=\vec{D}_1\,\cos\theta + \vec{D}_2\,\sin\theta$ is the unit outer normal to the interface in the reference configuration. Note that $\int_{0}^{2\pi}\tilde{\vec{\mu}}(\theta,s)\d\theta = 0$.

While $\bar{\vec{\mu}}$ corresponds to the resulting force in the cross-section and, therefore, couples position of the beam center-line to the matrix, $\tilde{\vec{\mu}}$ contains the coupled stresses, shears and hydrostatic pressure, and is thus responsible for transition of the beam bending and torsion to the matrix.
In the following proposition, we discuss in detail the structure of $\tilde{\vec{\mu}}$ and $\ten{\Sigma}$.


%We decompose the interface Lagrange multipliers $\vec{\mu}$, physically interpreted as interface load, into mean and fluctuation parts
%\begin{equation}\label{eq:LM_mu}
%\vec{\mu}\big|_{\Circ(s)} = \bar{\vec{\mu}}(s) + \tilde{\vec{\mu}}(\theta^{\alpha},s),\quad\text{where}\quad
%\bar{\vec{\mu}}(s) = \frac{1}{|C(s)|}\int\limits_{C(s)}\vec{\mu}\d C,\quad\int\limits_{C(s)}\tilde{\vec{\mu}}\d C = \vec{0},
%\end{equation}
%where the average term~$\bar{\vec{\mu}}$ corresponds to the resulting force applied to the cross-section, while the zero-mean term~$\tilde{\vec{\mu}}$ contains the hydrostatic pressure, shear and coupled stresses, produced by the matrix/beam coupling. 
%Therefore, we make an assumption that~$\tilde{\vec{\mu}}$ is in the following form:
%\begin{equation}\label{eq:new:mu_tilde}
%\tilde{\vec{\mu}}(\theta^{\alpha},s) = \ten{\Sigma}(s)\,\vec{N}(\theta^{\alpha}),
%\end{equation}
%where $\ten{\Sigma}$ denotes the interface stress tensor, and $\vec{N}=(\theta^{\alpha}\,\vec{D}_{\alpha})/\|\theta^{\alpha}\,\vec{D}_{\alpha}\|\big|_{\Circ(s)}$ is the unit outer normal to the interface in the reference configuration.
%This term can be rewritten using $\vec{N}=\vec{D}_1\,\cos\theta + \vec{D}_2\,\sin\theta$, where $\cos\theta = \theta^{1}\,\vec{D}_{1}\cdot\theta^{2}\,\vec{D}_{2}/(\|\theta^{1}\,\vec{D}_{1}\|\|\theta^{2}\,\vec{D}_{2}\|)$.
%Remark that in \eqref{eq:new:mu_tilde},  $\ten{\Sigma}\,\vec{D}_1$ and $\ten{\Sigma}\,\vec{D}_2$ are respectively the first coefficients in Fourier sine and cosine decompositions of~$\vec{\mu}$ as function of angle~$\theta$.
%Thus, assuming the Lagrange multiplier~$\vec{\mu}$ in the form~\eqref{eq:LM_mu}-\eqref{eq:new:mu_tilde}, we ignore the higher order frequencies in its Fourier series.
%%Note also that $\int_{C(s)}\ten{\Sigma}(s)\,\vec{N}(\theta^{\alpha})\d C = \ten{\Sigma}(s)\int_{C(s)}\,\vec{N}(\theta^{\alpha})\d C = 0$.

%Let us now consider the structure of $\tilde{\vec{\mu}}$ in details.

\begin{proposition}\label{th:Sigma_structure}
	Due to the definition~\eqref{eq:new:mu_tilde}, the stress tensor~$\ten{\Sigma}$ has only six degrees of freedom.
	In particular, denoting $\ten{\mathcal{D}}:=\vec{D}_j\otimes\vec{e}_j$, we write $\ten{\Sigma}$ in the following form, involving coupled stresses, shears and dilatation:
	\begin{equation}\label{eq:new:LM_matrix}
	\ten{\Sigma} =
	\fib{\vec{R}}\,\ten{\mathcal{D}}
	\begin{bmatrix}
	\tilde{\mu}_{n,1} & \tilde{\mu}_{n,3} - \tilde{\mu}_{\tau,3} & 0\\
	\tilde{\mu}_{n,3} + \tilde{\mu}_{\tau,3} & \tilde{\mu}_{n,2} & 0\\
	-2\,\tilde{\mu}_{\tau,2} &  2\,\tilde{\mu}_{\tau,1} & 0
	\end{bmatrix}
	\ten{\mathcal{D}}\tp,
	\end{equation}
where $\tilde{\mu}_{n,1}$, $\tilde{\mu}_{n,2}$ and $\tilde{\mu}_{n,3}$ are associated to the dilatation and the shear of the cross-section, $\tilde{\mu}_{\tau,1}$ and $\tilde{\mu}_{\tau,2}$ to the bending, and $\tilde{\mu}_{\tau,3}$ to the torsion.	
Let $\tilde{\vec{\mu}}_n = \tilde{\mu}_{n,j}\,\vec{d}_j$
and $\tilde{\vec{\mu}}_\tau = \tilde{\mu}_{\tau,j}\,\vec{d}_j = \axl\left(\ten{\Sigma}\,\fib{\vec{R}}\tp\right)$.	
Then, we have
\begin{equation}\label{eq:PQ_decomp}
\ten{\Sigma} = 
\left(
	\ten{\mathcal{P}}_{\alpha}\,\tilde{\vec{\mu}}_\tau 
+ 	\ten{\mathcal{Q}}_{\alpha}\,\tilde{\vec{\mu}}_n
\right)\otimes\vec{D}_\alpha,
\end{equation}
where
\begin{equation}\label{eq:shortcuts}
\begin{aligned}
\ten{\mathcal{P}}_1 &= \phantom{+}\vec{d}_2\otimes\vec{d}_3 - 2\,\vec{d}_3\otimes\vec{d}_2, 
&\qquad
\ten{\mathcal{Q}}_1 &= \vec{d}_1\otimes\vec{d}_1 + \vec{d}_2\otimes\vec{d}_3, \\ 
\ten{\mathcal{P}}_2 &= -\vec{d}_1\otimes\vec{d}_3 + 2\,\vec{d}_3\otimes\vec{d}_1,
&\qquad
\ten{\mathcal{Q}}_2 &= \vec{d}_2\otimes\vec{d}_2 + \vec{d}_1\otimes\vec{d}_3.
\end{aligned}
\end{equation}
Moreover, the tensor 
\begin{equation}\label{nu_sym}
	[\tilde{\vec{\mu}}_n]_s := \fib{\vec{R}}\tp\,\ten{\mathcal{Q}}_{\alpha}\,\tilde{\vec{\mu}}_n\otimes\vec{D}_\alpha = \tilde{\mu}_{n,1}\,\vec{D}_1\otimes\vec{D}_1 + \tilde{\mu}_{n,2}\,\vec{D}_2\otimes\vec{D}_2 + \tilde{\mu}_{n,3}\,\left(\vec{D}_1\otimes\vec{D}_2 + \vec{D}_2\otimes\vec{D}_1\right)
\end{equation}
is symmetric. 
%\CH{\sout{for any vector~$\tilde{\vec{\mu}}_n =  \tilde{\mu}_{n,j}\,\vec{d}_j$.}}
%\CH{Additionally we note that the decomposition 
%\begin{equation}\label{eq:new:prop:decomposition}
%\begin{aligned}
%\ten{\Sigma}
%&=
%\left(2\,\ten{I}-\fib{\vec{R}}\,\left(\vec{D}_{\alpha}\otimes\vec{D}_{\alpha}\right)\,\fib{\vec{R}}\tp\right)\underbrace{\skew{\ten{\Sigma}\,\fib{\vec{R}}\tp}}_{\VPTen{\tilde{\vec{\mu}}_\tau}}\fib{\vec{R}}\,\left(\vec{D}_{\alpha}\otimes\vec{D}_{\alpha}\right)\\
%&\phantom{=\,}+
%\underbrace{\fib{\vec{R}}\,\left(\vec{D}_{\alpha}\otimes\vec{D}_{\alpha}\right)\,\fib{\vec{R}}\tp\,\sym{\ten{\Sigma}\,\fib{\vec{R}}\tp}\,\fib{\vec{R}}\,\left(\vec{D}_{\alpha}\otimes\vec{D}_{\alpha}\right)}_{\ten{\mathcal{Q}}_{\alpha}\,\tilde{\vec{\mu}}_n\otimes\vec{D}_\alpha}\,,		
%\end{aligned}
%\end{equation}
%holds.}
\end{proposition}


%\begin{proof} \rev{Should we keep the proof ?}
%\begin{equation}
%	\begin{aligned}
%	\left(\ten{I}-\frac{1}{2}\,\fib{\vec{R}}\,\ten{P}_{12}\,\fib{\vec{R}}\tp\right)\,\skew{\ten{\Sigma}\,\ten{P}_{12}\,\fib{\vec{R}}\tp}\,\fib{\vec{R}}\,\ten{P}_{12}
%	&=
%	\frac{1}{2}\,\ten{\Sigma}\,\ten{P}_{12}-\frac{1}{4}\,\fib{\vec{R}}\,\ten{P}_{12}\,\left(\ten{\Sigma}\tp\,\fib{\vec{R}}+\fib{\vec{R}}\tp\,\ten{\Sigma}\right)\,\,\ten{P}_{12}\\
%	&=
%	\frac{1}{2}\,\ten{\Sigma}\,\ten{P}_{12}
%	-\frac{1}{2}\,\fib{\vec{R}}\,\sym{\ten{P}_{12}\,\fib{\vec{R}}\tp\,\ten{\Sigma}\,\ten{P}_{12}}.
%	\end{aligned}	
%	\end{equation}	
%\end{proof}

The following lemma gives the representation of the energy contribution due to the coupling on the beam mantle~$\Gamma_C$.
\begin{lemma}\label{th:CouplingTerm}
	If $\vec{\mu}$ is in form~\eqref{eq:LM_mu}, the coupling energy term~\eqref{eq:coupling_term_init}$_1$ writes
\begin{equation}\label{eq:coupling_term_lemma}
	\begin{aligned}
	\Pi_{C}
	&=
	\int\limits_{\mathfrak{C}_0} \vec{\mu}\cdot\left(\vec{\varphi}-\tilde{\vec{x}}\right) \abs{C}\d s
	\\
	&=
	\int\limits_{\mathfrak{C}_0} \bar{\vec{\mu}}\cdot\left(\bar{\vec{\varphi}}-\tilde{\vec{\varphi}}\right) \abs{C}\d s
	+
	\frac{1}{2}\int\limits_{\mathfrak{C}_0} \ten{\Sigma}:\left(\ten{\Phi}-\fib{\vec{R}}\right) \abs{C}\d s
	\\
	&=	
	\int\limits_{\mathfrak{C}_0} \bar{\vec{\mu}}\cdot\left(\bar{\vec{\varphi}}-\tilde{\vec{\varphi}}\right) \abs{C}\d s
	+
	\frac{1}{2}\int\limits_{\mathfrak{C}_0} \tilde{\vec{\mu}}_{\alpha}\cdot\left(\hat{\vec{\varphi}}_{\alpha}-\vec{d}_{\alpha}\right) \abs{C}\d s
	,
	\end{aligned}
	\end{equation}
	with
	\begin{align}
	\bar{\vec{\varphi}} &= \frac{1}{\abs{C}}\int\limits_{C(s)}\vec{\varphi}\d C,
	&\ten{\Phi} &= \frac{2}{\abs{C}}\int\limits_{C(s)} \vec{\varphi} \otimes \vec{N}\d C,
	\end{align}
	and Fourier cosine and sine coefficients respectively
	\begin{align}
	\hat{\vec{\varphi}}_1 &= \frac{2}{\abs{C}}\int\limits_{C(s)}\vec{\varphi}\,\cos\theta\d C,
	&\hat{\vec{\varphi}}_2 &= \frac{2}{\abs{C}}\int\limits_{C(s)}\vec{\varphi}\,\sin\theta\d C.
	\end{align}
\end{lemma}

\begin{proof}
	Substitution of \eqref{eq:LM_mu} and \eqref{eq:new:mu_tilde} to \eqref{eq:coupling_term_init}$_1$ yields
	\begin{equation}\label{eq:coupling_term_proof}
	\Pi_{C}
	=
	\int\limits_{\mathfrak{C}_0}\int\limits_{C(s)}\underbrace{\left(\bar{\vec{\mu}} +  \ten{\Sigma}\,\vec{N}\right)}_{\vec{\mu}}
	\cdot\biggl(\vec{\varphi}-\underbrace{\left(\tilde{\vec{\varphi}}+\fib{\vec{R}}\,\vec{N}\,r\right)}_{\tilde{\vec{x}}}\biggr) \d C\d s
	.
	\end{equation}
	Given $\vec{N} = \vec{D}_{1}\cos\theta + \vec{D}_{2}\sin\theta$, we have $\int_{C(s)}\vec{N}\d C = \vec{0}$ and $\int_{C(s)}\vec{N}\otimes\vec{N}\d C = \pi\,\vec{D}_{\alpha}\otimes\vec{D}_{\alpha}$.
	In particular,
	\begin{equation}
	\begin{split}
	\int\limits_{0}^{2\pi} \vec{N}\otimes\vec{N}\,\d\theta
	=&\vec{D}_1\otimes\vec{D}_1\,\underbrace{\int\limits_{0}^{2\pi}\cos^2\theta \,\d\theta}_{=\pi}
	+
	\vec{D}_2\otimes\vec{D}_2\,\underbrace{\int\limits_{0}^{2\pi}\sin^2\theta\d\theta}_{=\pi} \\
	&+ \left[\vec{D}_1\otimes\vec{D}_2+\vec{D}_2\otimes\vec{D}_1\right]\,\underbrace{\int\limits_{0}^{2\pi}\sin\theta\,\cos\theta\,\d\theta}_{=0}
	= \pi\,\vec{D}_\alpha\otimes\vec{D}_\alpha.
	\end{split}
	\end{equation}
%	\begin{equation}\label{eq:int_N}
%		\int\limits_{C(s)}\vec{N}\d C = \vec{0}
%		\qquad\text{and}\qquad
%		\int\limits_{C(s)}\vec{N}\otimes\vec{N}\d C = \pi\,\ten{P}_{12}.
%	\end{equation}
	Thus, taking into account that $\ten{\Sigma}\,\vec{D}_{\alpha}\otimes\vec{D}_{\alpha} = \ten{\Sigma}$, \eqref{eq:coupling_term_proof} writes
	\begin{equation}
	\begin{aligned}
	\Pi_{C}
	&=
	\int\limits_{\mathfrak{C}_0}\bar{\vec{\mu}}\cdot\int\limits_{C(s)}\left(\vec{\varphi}-\tilde{\vec{\varphi}}\right)\d C\d s
	+ 
	\int\limits_{\mathfrak{C}_0}\ten{\Sigma}:\int\limits_{C(s)}\left(\vec{\varphi}-\fib{\vec{R}}\,\vec{N}\,r\right)\otimes\vec{N} \d C\d s
	\\
	&=
	\int\limits_{\mathfrak{C}_0} \bar{\vec{\mu}}\cdot\left[\int\limits_{C(s)}\vec{\varphi}\d C-\tilde{\vec{\varphi}}\abs{C}\right] \d s
	+
	\int\limits_{\mathfrak{C}_0} \ten{\Sigma}:\left[\int\limits_{C(s)}\vec{\varphi}\otimes\vec{N}\d C - \pi \,r\,\fib{\vec{R}}\right]\d s
	.
	\end{aligned}	
	\end{equation}
	Hence if follows~\eqref{eq:coupling_term_lemma}$_2$.
	Finally, \eqref{eq:coupling_term_lemma}$_3$ is obtained by substitution of $\ten{\Sigma} = \tilde{\vec{\mu}}_{\alpha}\otimes\vec{D}_{\alpha}$ into  \eqref{eq:coupling_term_lemma}$_2$.
\end{proof}

\begin{remark}\label{rmk:wellposedness}
	Let us note that if $\vec{\varphi}\in\H{1}(\Omega)^3$, then according to the trace theorem, $\bar{\vec{\varphi}}\in\H{\frac{1}{2}}(\mathfrak{C}_0)^3$ and thus is in~$\L{2}(\mathfrak{C}_0)^3$.
	Likewise, $ \ten{\Phi} \in \L{2}(\mathfrak{C}_0)^{3\times 3} $.
	Thus, for $ \tilde{\vec{\varphi}}\in\H{1}(\mathfrak{C}_0)^3 $, $ \fib{\vec{R}}\in\H{1}(\mathfrak{C}_0)^{3\times 3}$,  $ \bar{\vec{\mu}}\in\L{2}(\mathfrak{C}_0)^3 $ 
	and $ \ten{\Sigma}\in\L{2}(\mathfrak{C}_0)^{3\times 3}$, the integral in~\eqref{eq:coupling_term_lemma}$_2$ is defined.
\end{remark}

Thus, we obtained the energy term~\eqref{eq:coupling_term_lemma}$_2$ coupling the 1D Cosserat beam to the 3D material matrix to the circular integrals of the matrix deformation~$\vec{\varphi}$ on the lateral area $\Gamma_C$ of the beam.
Such approach is common for 1D-3D coupling models (see, e.g., \cite{d2008coupling,koppl2018mathematical}), since the trace of~$\vec{\varphi}\in\H{1}(\Omega)^3$ on the beam centerline~$\mathfrak{C}_0$ is not well-defined.
However,  in practice, computation of the circular integrals can be subtle.
Moreover, Galerkin approximation using smooth basis functions allows us to deal with the traces of the matrix on the beam centerline. In this paper, we are not addressing mathematical aspects of the variational problem,  but rather focus on the computational model.
So, considering Galerkin projection, we assume necessary regularity and make use of the following lemma.

\begin{lemma}\label{th:expansion_in_r}
Let $\vec{\varphi}$ be regular enough, such that the traces $\vec{\varphi}_c(s):=\vec{\varphi}(\tilde{\vec{\varphi}}_0(s))$ and $\vec{F}_c(s):=\vec{F}(\tilde{\vec{\varphi}}_0(s))$ are square integrable. 	Then, if $\vec{\mu}$ is in form~\eqref{eq:LM_mu}, the coupling energy term~\eqref{eq:coupling_term_init}$_1$ writes
	\begin{equation}\label{eq:centerline_projection}
	\Pi_C
	=
	\int\limits_{\mathfrak{C}_0}\left[\bar{\vec{\mu}}\cdot(\vec{\varphi}_{c} -\tilde{\vec{\varphi}})
	+
	\frac{1}{2}\,\ten{\Sigma}:
	\big(\ten{F}_c-\fib{\vec{R}}\big)
	\right]\abs{C}\d s
	+ \O(r^2).
	\end{equation}
\end{lemma}

\begin{proof}
	Using Fourier representation of the trace of $\vec{\varphi}$ onto the plane containing $C(s)$ and the formal power series of the exponential, we can write
\begin{equation}\label{eq:FormalTaylor}
	\begin{aligned}
		\vec{\varphi}\bigr|_{C(s)} 
		&= 
		\int\limits_{\R^2}\hat{\vec{\varphi}}(\vec{\omega},s)\, \exp{\i\,\vec{\omega}\cdot\vec{N}(\theta)\,r} \d\vec{\omega}
		=
		\sum_{k=0}^{\infty}\,\int\limits_{\R^2}\hat{\vec{\varphi}}(\vec{\omega},s)\, \frac{\left(\i\,\vec{\omega}\cdot\vec{N}(\theta)\,r\right)^k}{k!} \d\vec{\omega}
		\\
		&=
		\vec{\varphi}_c(s) + \vec{F}_{c}(s)\cdot\vec{N}(\theta)\,r + \O(r^2).
	\end{aligned}
\end{equation}	
	Then, substitution of~\eqref{eq:FormalTaylor}$_2$ to the equation~\eqref{eq:coupling_term_lemma}$_2$ of Lemma~\ref{th:CouplingTerm} yields the statement.
\end{proof}

Under the assumption that the fiber is thin, we neglect in~\eqref{eq:centerline_projection} the terms with powers of~$r$ greater than one, keeping only the linear term.

Eventually, one can consider the end faces $A_s = \lbrace (\rho\,\cos\theta, r\,\sin\theta, s) \; | \, \rho\in[0,r], \theta\in[0, 2\,\pi] \rbrace$, $s\in\{0,L\}$.
Similar to~\eqref{eq:LM_mu}-\eqref{eq:new:mu_tilde} with replacing a circular mean by a cross-sectional one, we treat the Lagrange multipliers~$\vec{\mu}$ on the end faces $A_0$ and $A_L$:
\begin{equation}\label{eq:LM_mu_A}
\vec{\mu}(\rho,\theta,s) = \bar{\vec{\mu}}(\rho,s) + \ten{\Sigma}(\rho,s)\,\vec{N}(\theta),
\end{equation}
where $\bar{\vec{\mu}}(\rho, s) = \frac{1}{2\,\pi\,\rho}\int_{0}^{2\pi}\vec{\mu}(\rho, \theta, s)\d\theta$, and $\ten{\Sigma}$ has the same form as in~\eqref{eq:new:LM_matrix}.
Then, using the same arguments as in Lemma~\ref{th:CouplingTerm} and Lemma~\ref{th:expansion_in_r}, the coupling energy term at the end faces writes
\begin{equation}\label{eq:PiA_init}
\Pi_{A}
=
%\sum_{s=0,L}
\EC{\int_{0}^{r} \left[\bar{\vec{\mu}}\cdot\left(\vec{\varphi}_c-\tilde{\vec{\varphi}}\right)
+
\frac{1}{2}\,\ten{\Sigma}:\left(\ten{F}_c-\fib{\vec{R}}\right)\right]\, \abs{C(\rho)}\d\rho}
+ \O(r^3).
\end{equation}
However, since this term scales as $r^2$, we also neglect it.

\begin{remark}
Remark that further consideration of higher order terms in the expansion~\eqref{eq:FormalTaylor} will lead to higher gradients models, reducing the modeling error.
\end{remark}

Thus, the virtual work associated to the kinematic constraints is obtained as variation of~\eqref{eq:centerline_projection} in the following form:
\begin{equation}\label{eq:VirtWork_coupling}
\begin{aligned}
\delta\Pi_\Gamma
\approx
\delta\Pi_C
\approx&\,
\int\limits_{\mathfrak{C}_0}\bigl[\delta\bar{\vec{\mu}}\cdot(\vec{\varphi}_{c} -\tilde{\vec{\varphi}})
+
\bar{\vec{\mu}}\cdot(\delta\vec{\varphi} -\delta\tilde{\vec{\varphi}})\bigr]\abs{C}\d s 
\\
&+\,
\int\limits_{\mathfrak{C}_0}\left[
\frac{1}{2}\,\ten{\Sigma}:\big(\nabla\delta\vec{\varphi}-\left[\delta\vec{\phi}\right]_\times\fib{\vec{R}}\big)
+
\frac{1}{2}\,\delta\ten{\Sigma}:\big(\vec{F}_{c}-\fib{\vec{R}}\big)
\right]\abs{C}\d s,
\end{aligned}
\end{equation}
where we note that $\frac{1}{2}\,\ten{\Sigma}:\left(\VPTen{\delta\vec{\phi}}\,\fib{\ten{R}}\right) = \tilde{\vec{\mu}}_\tau\cdot\delta\vec{\phi}$.

\subsection{Total coupled system}
Finally, we obtain the principle of virtual work for the  coupled matrix/beam system
\begin{equation}
%\delta\Pi^{int} + \delta\Pi^{ext} + \delta\fib{\Pi}^{int} + \delta\fib{\Pi}^{ext} + \delta\Pi_C + \delta\Pi_A = 0,
\delta\Pi^{int} + \delta\Pi^{ext} + \delta\fib{\Pi}^{int} + \delta\fib{\Pi}^{ext} + \delta\Pi_\Gamma = 0,
\end{equation}
in terms of \eqref{eq:pdvA} and \eqref{eq:pdvaHW2} along with the virtual work of the coupling forces in \eqref{eq:VirtWork_coupling}. Regarding the matrix material, i.e., the variation with respect to $\vec{\varphi}$, we obtain
\begin{equation}\label{eq:sys:matrix}
\begin{aligned}
\int\limits_{\mtx{\Omega}_0} \left[\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}} - \vec{B}_{ext}\cdot\delta\vec{\varphi}\right] \d V	-
\int\limits_{\Gamma^{\sigma}} \vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d A
+
\int\limits_{\mathfrak{C}_0}\left(\vec{\bar{\mu}} \cdot \delta\vec{\mtx{\varphi}}
+
\frac{1}{2}\,\ten{\Sigma}:\nabla\delta\mtx{\vec{\varphi}} \right) \abs{C}\d s
%+
%\EC{\bar{\vec{\mu}}^{e}\cdot\delta\mtx{\vec{\varphi}}
%	+
%	\frac{1}{2}\,\ten{\Sigma}^{e}: \nabla\delta\mtx{\vec{\varphi}}} \abs{A}
= 0,
\end{aligned}
\end{equation}
and the beam contributions  yield
\begin{align}
&-\int\limits_{\mathfrak{C}_0}\left(
{\mathfrak{n}}^{\prime} + \bar{\tilde{\vec{n}}}
+
\bar{\vec{\mu}}\abs{C}\right)\cdot\delta\fib{\vec{\varphi}}\d s = 0,  
\label{eq:sys:loads}
\\	
&-\int\limits_{\mathfrak{C}_0}\left({\mathfrak{m}}^{\prime} + \tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}}
+
\bar{\tilde{\vec{m}}}
+
\tilde{\vec{\mu}}_\tau\abs{C}\right)\cdot\delta\vec{\phi} \d s = 0,
\label{eq:sys:moments}
\end{align}
with boundary conditions $\EC{\delta\tilde{\vec{\varphi}}\cdot\left(\mathfrak{n}-\vec{n}_{ext}^{e}\right)} = 0$ and $\EC{\delta\vct{\phi}\cdot\left(\mathfrak{m}-\vec{m}_{ext}^{e}\right)} = 0$, and supplemented by the weak constitutive equations
\begin{align}
&\int\limits_{\mathfrak{C}_0}\delta{\mathfrak{g}}\cdot\left(\fib{\ten{R}}\,\frac{\partial\tilde{\Psi}(\vec{\Gamma},\vec{K})}{\partial\vec{\Gamma}}-{\mathfrak{n}} \right)\d s = 0,
\label{eq:constitutive_n}
\\
&\int\limits_{\mathfrak{C}_0}\delta{\mathfrak{k}}\cdot\left( \fib{\ten{R}}\,\frac{\partial\tilde{\Psi}(\vec{\Gamma},\vec{K})}{\partial\vec{K}}-{\mathfrak{m}} \right)\,\text{d}s = 0,
\label{eq:constitutive_m}
\end{align}
as well as the coupling constraints
\begin{align}
\int\limits_{\mathfrak{C}_0}\delta\vec{\bar{\mu}} \cdot\left(\vec{\mtx{\varphi}}_c-\fib{\vec{\varphi}}\right)\abs{C}\d s &= 0,
%&\EC{\delta\bar{\vec{\mu}}^{e}\cdot(\vec{\varphi}_{c} -\tilde{\vec{\varphi}})}\abs{A} &= 0
\label{eq:sys:pi1}
\\
\frac{1}{2}\,\int\limits_{\mathfrak{C}_0}\delta\ten{\Sigma}:\big(\vec{F}_{c}-\fib{\vec{R}}\big)\abs{C}\d s &= 0.
%&\,\,\frac{1}{2}\,\EC{\delta\ten{\Sigma}^{e}:(\vec{F}_{c}-\fib{\vec{R}})}\abs{A} &= 0.
\label{eq:sys:pi2}
\end{align}

\begin{remark}\label{re:shear}
Note that the variation of $\ten{\Sigma} = \vec{\mu}_{\alpha}\otimes\vec{D}_{\alpha}$ has the form $\delta\ten{\Sigma} = \delta\vec{\mu}_{\alpha}\otimes\vec{D}_{\alpha}$.
Thus, the constraints~\eqref{eq:sys:pi2} can be rewritten as follows:
\begin{equation}\label{key6}
\frac{1}{2}\,	\int\limits_{\mathfrak{C}_0}
\big(\vec{F}_{c}\,\vec{D}_{1}-\vec{d}_{1}\big)\cdot\delta\tilde{\vec{\mu}}_1\abs{C}\d s = 0,
\qquad
\frac{1}{2}\,	\int\limits_{\mathfrak{C}_0}
\big(\vec{F}_{c}\,\vec{D}_{2}-\vec{d}_{2}\big)\cdot\delta\tilde{\vec{\mu}}_2\abs{C}\d s = 0.
\end{equation}
Alternatively, in line with the representation~\eqref{eq:PQ_decomp}, let $\delta\ten{\Sigma} = \left(\ten{\mathcal{P}}_{\alpha}\,\delta\tilde{\vec{\mu}}_\tau + \ten{\mathcal{Q}}_{\alpha}\,\delta\tilde{\vec{\mu}}_n\right)\otimes\vec{D}_\alpha$.
Then, the constraints~\eqref{eq:sys:pi2} rewrite as 
\begin{align}
\frac{1}{2}\,\int\limits_{\mathfrak{C}_0}\left(
\ten{\mathcal{P}}_{\alpha}\tp\,\left[\vec{F}_{c}\,\vec{D}_{\alpha}-\vec{d}_{\alpha} \right]\right)
\cdot\delta\tilde{\vec{\mu}}_{\tau}\abs{C}\d s& = 0,
\label{eq:coup_cond1}
\\
\label{eq:coup_cond2}
\frac{1}{2}\,\int\limits_{\mathfrak{C}_0} \left(
\ten{\mathcal{Q}}_{\alpha}\tp\,\left[\vec{F}_{c}\,\vec{D}_{\alpha}-\vec{d}_{\alpha} \right]\right)
\cdot\delta\tilde{\vec{\mu}}_{n}\abs{C}\d s &= 0,
\end{align}
such that the hydrostatic pressure and shear are separated from the bending and torsional parts.
In fact, the last condition does not involve the beam at all, restraining only the stretches and the shears of the matrix, which is shown in the following lemma.

\end{remark}

\begin{lemma}\label{th:area_cond_F}
	Condition \eqref{eq:coup_cond2} can be rewritten as
	\begin{equation}\label{eq:area_cond_F}
%	\int\limits_{\mathfrak{C}_0} \left(\vec{F}_{c}\tp\,\vec{F}_{c}-\ten{I}\right):\fib{\ten{R}}\tp\ten{\mathcal{Q}}_{\alpha}\delta\tilde{\vec{\mu}}_{n}\otimes\vec{D}_\alpha
%	\abs{C}\d s = 0.
	\frac{1}{2}\,\int\limits_{\mathfrak{C}_0} \left(\vec{F}_{c}\tp\,\vec{F}_{c}-\ten{I}\right):[\delta\tilde{\vec{\mu}}_{n}]_s\, \abs{C}\,\d s = 0,
	\end{equation}
	with
	$
	[\delta\tilde{\vec{\mu}}_{n}]_s =\delta\tilde{\mu}_{n,1}\,\vec{D}_1\otimes\vec{D}_1 + \delta\tilde{\mu}_{n,2}\,\vec{D}_2\otimes\vec{D}_2
	 + \delta\tilde{\mu}_{n,3}\,(\vec{D}_1\otimes\vec{D}_2 + \vec{D}_2\otimes\vec{D}_1)
	$.
\end{lemma}


\begin{proof}
	Integrating in~\eqref{eq:sys:pi2} with $\delta\ten{\Sigma} = \fib{\ten{R}}\,[\delta\tilde{\vec{\mu}}_{n}]_s$ and $\delta\ten{\Sigma} = \ten{F}_{c}\,[\delta\tilde{\vec{\mu}}_{n}]_s$, and using symmetry of $[\delta\tilde{\vec{\mu}}_{n}]_s$, we obtain 
	\begin{equation}\label{eq:area_cond_F_proof}
	\frac{1}{2}\,\int\limits_{\mathfrak{C}_0} \ten{R}\tp\,(\ten{F}_{c}-\fib{\ten{R}}):[\delta\tilde{\vec{\mu}}_{n}]_s\,
	\abs{C}\,\d s = 0,
	\qquad
	\frac{1}{2}\,\int\limits_{\mathfrak{C}_0} (\ten{F}_{c}-\fib{\ten{R}})\tp\,\ten{F}_{c}:[\delta\tilde{\vec{\mu}}_{n}]_s\,
	\abs{C}\,\d s = 0,
	\end{equation}
	respectively. Given $	\ten{F}_{c}\tp\,\ten{F}_{c}-\ten{I} = \fib{\ten{R}}\tp\,(\ten{F}_{c}-\fib{\ten{R}}) + (\ten{F}_{c}-\fib{\ten{R}})\tp\,\ten{F}_{c}$, summing up the integrals in~\eqref{eq:area_cond_F_proof} yields the statement.
\end{proof}

\begin{lemma}\label{th:R2F}
	The following equality holds:
	\begin{equation}\label{eq:R2F}
	\int\limits_{\mathfrak{C}_0}\ten{\mathcal{Q}}_{\alpha}\,\tilde{\vec{\mu}}_n
	\otimes\vec{D}_{\alpha}:\nabla\delta\mtx{\vec{\varphi}}\, \abs{C}\,\d s 
	=
	\int\limits_{\mathfrak{C}_0}\ten{F}_{c}\,[\tilde{\vec{\mu}}_{n}]_s:\nabla\delta\mtx{\vec{\varphi}} \,\abs{C}\,\d s 
	\end{equation}
\end{lemma}

\begin{proof}
	Integrating in~\eqref{eq:sys:pi2} with $\delta\ten{\Sigma} = \nabla\delta\mtx{\vec{\varphi}}\,[\tilde{\vec{\mu}}_{n}]_s$ yields the statement.
\end{proof}

In the following proposition, the above system is reduced by condensing equations~\eqref{eq:sys:loads}-\eqref{eq:sys:moments} and eliminating the Lagrange multipliers.  
\begin{proposition}[\textbf{Condensed system}]\label{th:condensed_sys}
Let $V=\{v\in\H{1}(\Omega_0),\text{s.t. } \vec{D}_\alpha\cdot \nabla v|_{\mathfrak{C}_0}\in\L{2}(\mathfrak{C}_0) \}$.
The system~\eqref{eq:sys:matrix}-\eqref{eq:sys:pi2} can be reduced to the following system of the unknowns $\vec{\varphi}\in V^3$, $\fib{\vec{\varphi}},\vec{\phi}\in\left(\H{1}(\mathfrak{C}_0)\right)^3$, $\mathfrak{n},\mathfrak{m},\tilde{\vec{\mu}}_n\in\left(\L{2}(\mathfrak{C}_0)\right)^3$:
%The system~\eqref{eq:sys:matrix}-\eqref{eq:sys:pi2} can be reduced to the following system of the unknowns $\vec{\varphi}:\Omega_0\to\R^3$, $\fib{\vec{\varphi}}:\mathfrak{C}_0\to\R^3$, $\vec{\phi}:\mathfrak{C}_0\to\R^3$, $\mathfrak{n}:\mathfrak{C}_0\to\R^3$, $\mathfrak{m}:\mathfrak{C}_0\to\R^3$ and $\CH{\tilde{\vec{\mu}}_n}:\mathfrak{C}_0\to\R^3$:
\begin{equation}\label{eq:condensedCompact}
\begin{aligned}
\int\limits_{\mtx{\Omega}_0}\bigl(\vec{P}:\nabla\delta\vec{\mtx{\varphi}}\, -\, \vec{B}_{ext}\cdot\delta\vec{\varphi}\bigl) \d V 
-\int\limits_{\Gamma^{\sigma}} \vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d A &\\
+\,\int\limits_{\mathfrak{C}_0}\biggl(\mathfrak{P}\,\vdots\,\nabla^2\delta\mtx{\vec{\varphi}} + \bigl(\vec{P}^{\mathfrak{n}}+\vec{P}^{\mathfrak{m}} + \vec{P}^{g} + \frac{1}{2}\,\ten{F}_{c}\,[\tilde{\vec{\mu}}_n]_s\,\abs{C}
\bigr):\nabla\delta\vec{\mtx{\varphi}} 
- \bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}
\biggl)\d s&\\
-\EC{\vec{n}_{ext}^{e}\cdot\delta\mtx{\vec{\varphi}}	+	\frac{1}{2}\left(\ten{\mathcal{P}}_{\alpha}\,\vec{m}_{ext}^{e} \otimes\,\vec{D}_{\alpha}\right):\nabla\delta\mtx{\vec{\varphi}}}&= 0 ,
\\[4mm]
\int\limits_{\mathfrak{C}_0}\delta{\mathfrak{g}}\cdot\left(\fib{\ten{R}}\,\frac{\partial\tilde{\Psi}(\vec{\Gamma},\vec{K})}{\partial\vec{\Gamma}}-{\mathfrak{n}} \right)\d s+\int\limits_{\mathfrak{C}_0}\delta{\mathfrak{k}}\cdot\left( \fib{\ten{R}}\,\frac{\partial\tilde{\Psi}(\vec{\Gamma},\vec{K})}{\partial\vec{K}}-{\mathfrak{m}} \right)\,\d s &=0\,,
\\[4mm]
\int\limits_{\mathfrak{C}_0}\delta\vec{\bar{\mu}} \cdot\left(\vec{\mtx{\varphi}}_c-\fib{\vec{\varphi}}\right)\,\abs{C}\,\d s
+ \frac{1}{2}\,
\int\limits_{\mathfrak{C}_0}
\ten{\mathcal{P}}_{\alpha}\tp\left(\vec{F}_{c}\,\vec{D}_{\alpha}-\vec{d}_{\alpha} \right)\cdot\delta\tilde{\vec{\mu}}_\tau\,\abs{C}\, \d s&\\
%	+
%	\delta\vec{b}\cdot\int\limits_{\mathfrak{C}_0}
%	\ten{\mathcal{Q}}_{\alpha}\tp\left(\vec{F}_{c}\,\vec{D}_{\alpha}-\vec{d}_{\alpha} \right)\d s
%		+
%	\int\limits_{\mathfrak{C}_0}
%	\ten{\mathcal{Q}}_{\alpha}\tp\left(\vec{F}_{c}\,\vec{D}_{\alpha}-\vec{d}_{\alpha} \right)
%	\cdot\delta\tilde{\mu}_n\d s
+\frac{1}{2}\,\int\limits_{\mathfrak{C}_0} \left(\vec{F}_{c}\tp\vec{F}_{c}-\ten{I}\right):[\delta\tilde{\vec{\mu}}_n]_s\,\abs{C}\, \d s
&= 0\,,
\end{aligned}
\end{equation}
for all $\delta\vec{\varphi}\in \{v\in\H{1}(\Omega_0),\text{s.t. } \vec{D}_\alpha\cdot\nabla v|_{\mathfrak{C}_0}\in\H{1}(\mathfrak{C}_0) \}^3$, $\delta{\mathfrak{g}},\delta{\mathfrak{k}},\delta\vec{\bar{\mu}},\delta\tilde{\vec{\mu}}_\tau,\delta\tilde{\vec{\mu}}_n\in\left(\L{2}(\mathfrak{C}_0)\right)^3$,
where the corresponding stresses are defined as follows:
\begin{align}
\vec{P} &:= \drv{\mtx{\Psi}}{\ten{\mtx{F}}}, \\
\vec{P}^{\mathfrak{n}} &:= \mathfrak{n}\otimes\vec{D}_3, \\
\vec{P}^{\mathfrak{m}} &:= \frac{1}{2}\,\left[\ten{\mathcal{P}}_{\alpha}^\prime\,\mathfrak{m}		
-\ten{\mathcal{P}}_{\alpha}\left(\tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}} +\bar{\tilde{\vec{m}}}\right)
%		+ \ten{\mathcal{Q}}_{\alpha}\,\tilde{\vec{\mu}}_n
\right]\otimes\vec{D}_{\alpha}, \\
\vec{P}^{g} &:= \frac{1}{2}\,\ten{\mathcal{P}}_{\alpha}\,\mathfrak{m}\otimes\vec{D}_\alpha^\prime,
\\
\mathfrak{P} &:= \frac{1}{2}\,\ten{\mathcal{P}}_{\alpha}\,\mathfrak{m}\otimes\vec{D}_\alpha\otimes\vec{D}_3.\label{eq:thirdOrderDef}
\end{align}
Recall that the tensors~$\ten{\mathcal{P}}_{\alpha}$ and $[\delta\tilde{\vec{\mu}}_n]_s$ are defined in Proposition~\ref{th:Sigma_structure}.
\end{proposition}

\begin{remark}
	Note that the term $\vec{P}^{g}$ is due to the initial curvature of the beam.	
	In the case of a straight initial configuration, i.e.,\ when $\vec{D}_{\alpha}^\prime\equiv 0$, this term vanishes.	
	Moreover, according to Appendix \ref{app:derivativeP}, we have in this case
	$\ten{\mathcal{P}}_{\alpha}^\prime = \VPTen{\vec{\kappa}}\ten{\mathcal{P}}_{\alpha} - \ten{\mathcal{P}}_{\alpha}\VPTen{\vec{\kappa}}$.
\end{remark}

\begin{remark}
We now obtain in~\eqref{eq:condensedCompact} an explicit representation for the third order stress tensor introduced in~\eqref{eq:secondGradient}, which emanates from the condensation of the moment equation of the beams. Note that this term directly depends on the resultant torque~$\mathfrak{m}$, derived from, e.g.,\ \eqref{eq:simpleMat}, which is written in terms of the second and the polar areal moment,  respectively. This third order stress tensor is restricted to the line $\mathfrak{C}_0$ at the scale of the fiber, which is, in general,  in terms of [\textmu m] for short fiber reinforced polymers. For a more general strain gradient framework at a macroscopic scale, suitable homogenization procedures have to be applied.
\end{remark}

\begin{proof}[Proof of Proposition~\ref{th:condensed_sys}]
Using~\eqref{eq:sys:loads} with test functions~$\delta\fib{\vec{\varphi}} = \delta\vec{\varphi}|_{\mathfrak{C}_0}$,  we obtain~\eqref{eq:sys:matrix}.  Hence, after integration by parts and noting that $\partial_s \equiv \vec{D}_3\cdot\nabla$ and the endpoint conditions $\mathfrak{n} = \vec{n}_{ext}^{e}$ at $s=0,L$, we obtain
	\begin{equation}\label{eq:new:sys:matrix_condense}
	\begin{aligned}
	&\int\limits_{\mtx{\Omega}_0} \left(\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}}- \vec{B}_{ext}\cdot\delta\vec{\varphi}\right) \d V
	-
	\int\limits_{\Gamma^{\sigma}} \vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d A
	\\
	&
	+\int\limits_{\mathfrak{C}_0}\left(\left[\mathfrak{n}\otimes\vec{D}_3\right] : \nabla\delta\mtx{\vec{\varphi}}
	-
	\bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}\right)\d s
	-
	\EC{\vec{n}_{ext}^{e}\cdot\delta\mtx{\vec{\varphi}}} 
	\\&+
	\int\limits_{\mathfrak{C}_0}
	\frac{1}{2}\,\ten{\Sigma}:\nabla\delta\mtx{\vec{\varphi}} \abs{C}\d s
%	+
%	\EC{\frac{1}{2}\,\ten{\Sigma}^{e}: \nabla\delta\mtx{\vec{\varphi}}} \abs{A}
	= 0.
	\end{aligned}
	\end{equation}
Thus, we have eliminated the set of Lagrange multipliers $\bar{\vec{\mu}}$. For the second set of Lagrange multipliers~$\ten{\Sigma}$, we integrate in~\eqref{eq:sys:moments} with the test functions~$\delta\vec{\phi}= \ten{\mathcal{P}}_{\alpha}\tp\,\nabla\delta\vec{\mtx{\varphi}} \,\vec{D}_{\alpha} \in\L{2}(\mathfrak{C}_0)$. Taking the decomposition~\eqref{eq:PQ_decomp} and Lemma~\eqref{th:R2F} into account,  yields
	\begin{equation}\label{eq:expl_stress}
	-\int\limits_{\mathfrak{C}_0}\left[\ten{\mathcal{P}}_{\alpha}
	\left({\mathfrak{m}}^{\prime} + \tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}}+\bar{\tilde{\vec{m}}}\right)
	\otimes\vec{D}_{\alpha}
	+
	\left(\ten{\Sigma}
	-
	\ten{F}_{c}\,[\tilde{\vec{\mu}}_n]_s
%	\ten{\mathcal{Q}}_{\alpha}\,\tilde{\vec{\mu}}_n\otimes\vec{D}_{\alpha}
	\right)	\abs{C}	
	\right]
	:
	\nabla\delta\vec{\mtx{\varphi}}
	\d s
	= 0.
	\end{equation}
Then, multiplying the above equation by $\frac{1}{2}$, adding it to~\eqref{eq:new:sys:matrix_condense} and integrating it by parts with the endpoint conditions $\mathfrak{m} = \vec{m}_{ext}^{e}$  at $s=0,L$, we obtain
	\begin{equation}\label{eq:new:sys:matrix_very_condense}
	\begin{aligned}
	&\,\int\limits_{\mtx{\Omega}_0} \biggl(\underbrace{\drv{\mtx{\Psi}}{\ten{\mtx{F}}}}_{\vec{P}}:\nabla\delta\vec{\mtx{\varphi}} - \vec{B}_{ext}\cdot\delta\vec{\varphi}\biggl) \d V 
	-
	\int\limits_{\Gamma^{\sigma}} \vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d A
	\\
	&
	+
	\int\limits_{\mathfrak{C}_0}\biggl(\underbrace{\mathfrak{n}\otimes\vec{D}_3}_{\vec{P}^{\mathfrak{n}}} : \nabla\delta\mtx{\vec{\varphi}}
	-
	\bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}\biggl)\d s  
	-
	\EC{\vec{n}_{ext}^{e}\cdot\delta\mtx{\vec{\varphi}}
		+
		\frac{1}{2}\left(\ten{\mathcal{P}}_{\alpha}\,\vec{m}_{ext}^{e} \otimes\,\vec{D}_{\alpha}\right):\nabla\delta\mtx{\vec{\varphi}}}
	\\
	&
	+\,
	\int\limits_{\mathfrak{C}_0}
	\underbrace{\frac{1}{2}\left[\ten{\mathcal{P}}_{\alpha}\,\mathfrak{m}\otimes\vec{D}_\alpha\otimes\vec{D}_3\right]}_{\mathfrak{P}}\,\vdots\,\nabla^2\delta\mtx{\vec{\varphi}}
	\d s
	+
	\int\limits_{\mathfrak{C}_0}
	\underbrace{\frac{1}{2}\left[\ten{\mathcal{P}}_{\alpha}\,\mathfrak{m}\otimes\vec{D}_\alpha^\prime\right]}_{\vec{P}^{g}}:\nabla\delta\mtx{\vec{\varphi}}
	\d s
	\\
	&+\,
	\int\limits_{\mathfrak{C}_0}
	\biggl(\underbrace{\frac{1}{2}\left[\ten{\mathcal{P}}_{\alpha}^\prime\,\mathfrak{m}
%		+ \ten{\mathcal{Q}}_{\alpha}\,\tilde{\vec{\mu}}_n
		-\ten{\mathcal{P}}_{\alpha}\left(\tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}} +\bar{\tilde{\vec{m}}}\right)
		\right]\otimes\vec{D}_{\alpha}}_{\vec{P}^{\mathfrak{m}}}
		+
		\frac{1}{2}\,\ten{F}_{c}\,[\tilde{\vec{\mu}}_n]_s\,\abs{C}\biggr):\nabla\delta\mtx{\vec{\varphi}}\,\d s
	= 0,
	\end{aligned}
	\end{equation}
	supplemented with constitutive equations~\eqref{eq:constitutive_n}-\eqref{eq:constitutive_m} and coupling constraints \eqref{eq:sys:pi1}, \eqref{eq:coup_cond1} and \eqref{eq:area_cond_F}.
\end{proof}

\begin{remark}
For the physical interpretation of the third order stress tensor $\mathfrak{P}$ given in \eqref{eq:thirdOrderDef}, let us consider equation~\eqref{eq:expl_stress}, such that the stress contributions of the condensed beam equations along the line integral are written as
\begin{equation}
\ten{\Sigma} =  \bigl(\vec{\mathcal{P}}_{\alpha}\underbrace{\left[-(\mathfrak{m}^{\prime} +\tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}} +\bar{\tilde{\vec{m}}})\abs{C}\inv\right]}_{ \tilde{\vec{\mu}}_\tau} + \ten{\mathcal{Q}}_{\alpha}\,\tilde{\vec{\mu}}_n\bigr)\otimes\vec{D}_{\alpha}.
\end{equation}
Using the component $\tilde{\mu}_{\tau,j}$ and $\tilde{\mu}_{n,j}$ with regard to the basis $\vec{d}_j$ in the actual configuration and \eqref{def_grad_beam_2} we find
\begin{equation}
\begin{aligned}
 \ten{\Sigma}\,\fib{\ten{F}}\tp = 
\tilde{\vec{R}}\,\vec{\mathcal{D}}
\underbrace{\begin{bmatrix}
\tilde{\mu}_{n,1}   &  \tilde{\mu}_{n,3}-\tilde{\mu}_{\tau,3} & 0  \\
\tilde{\mu}_{n,3} +\tilde{\mu}_{\tau,3} & \tilde{\mu}_{n,2} & 0 \\
-2\,\tilde{\mu}_{\tau,2}   & 2\,\tilde{\mu}_{\tau,1}  &  0
\end{bmatrix}}_{\vec{\sigma}^{b}}\vec{\mathcal{D}}\tp\,\tilde{\vec{R}}\tp.
\end{aligned}
\end{equation}
The decomposition of $\vec{\sigma}^{b}$ in symmetric and skew symmetric parts reads
\begin{equation}
\begin{aligned}
\vec{\sigma}^{b}_{sym}=
\begin{bmatrix}
\tilde{\mu}_{n,1}   & \tilde{\mu}_{n,3} & -\tilde{\mu}_{\tau,2}  \\
\tilde{\mu}_{n,3}& \tilde{\mu}_{n,2} & \tilde{\mu}_{\tau,1}\\
-\tilde{\mu}_{\tau,2} & \tilde{\mu}_{\tau,1}  &  0
\end{bmatrix},\quad
\vec{\sigma}^{b}_{skw}=
\begin{bmatrix}
0   & -\tilde{\mu}_{\tau,3} &  \tilde{\mu}_{\tau,2}\\
\tilde{\mu}_{\tau,3} & 0 & -\tilde{\mu}_{\tau,1} \\
-\tilde{\mu}_{\tau,2}   & \tilde{\mu}_{\tau,1}  &  0
\end{bmatrix}.
\end{aligned}
\end{equation}
Note, that $\mathfrak{n}\otimes\vec{D}_3$ induces additional contributions to both parts if $\mathfrak{n}$ is not aligned with $\vec{d}_3$. Summarized, we obtain skew symmetric stress contributions, which can be considered as the result of the line divergence of the coupled forces.
\end{remark}



==> sections/sec_DirectorsParametrization.tex <==
% !TeX root = ../MAIN.tex

\subsection{Alternative parametrization of $\fib{\ten{R}}$.}
\rev{I believe, this is a more natural and more convenient parametrization, than quaternions or Euler angles.}
This parametrization corresponds to Rodrigues rotation formula. 

\begin{gather}\label{key}
\fib{\ten{R}}(s) = \Exp{\sum\limits_{j=1}^{3}\theta_j(s)\,\ten{L}_j} = \Exp{[\vec\theta]_{\times}},\\
\ten{L}_1 = 
\left[\begin{array}{ccc}
	0&0&0\\ 0&0&-1 \\0&1 &0
\end{array}\right], 
\qquad
\ten{L}_2 = 
\left[\begin{array}{ccc}
	0&0& 1\\ 0&0&0\\ -1 &0&0
\end{array}\right], 
\qquad
\ten{L}_3 =
\left[\begin{array}{ccc} 
	0& -1 &0\\ 1 &0&0\\0&0&0
\end{array}\right].
\end{gather}
Hence, its derivative is
\begin{equation}\label{key}
\drv{\fib{\ten{R}}}{s} = \fib{\ten{R}}\sum\limits_{j=1}^{3}\ten{L}_j\,\drv{\theta_j}{s}.
\end{equation}
Then the curvature vector can be written as
%\begin{align}\label{key}
%\vec{\kappa} 
%&= 
%-\mat{
%	\vec{d}_3\tp\,\partial_{s}{\vec{d}_2} \\
%	\vec{d}_1\tp\,\partial_{s}{\vec{d}_3} \\
%	\vec{d}_2\tp\,\partial_{s}{\vec{d}_1}
%}
%=
%\frac{1}{2}\,\mat{
%	\vec{d}_2\tp\,\partial_{s}{\vec{d}_3-\vec{d}_3\tp\,\partial_{s}{\vec{d}_2}} \\
%	\vec{d}_3\tp\,\partial_{s}{\vec{d}_1-\vec{d}_1\tp\,\partial_{s}{\vec{d}_3}} \\
%	\vec{d}_1\tp\,\partial_{s}{\vec{d}_2-\vec{d}_2\tp\,\partial_{s}{\vec{d}_1}}
%}\\
%&=
%\frac{1}{2}\,\axl\left(\fib{\ten{R}}\tp\,\drv{\fib{\ten{R}}}{s}\right)
%=
%\frac{1}{2}\,\axl\left(\fib{\ten{R}}\tp\,\fib{\ten{R}}\sum\limits_{j=1}^{3}\ten{L}_j\,\drv{\theta_j}{s}\right)
%=
%\frac{1}{2}\,\sum\limits_{j=1}^{3}\axl\ten{L}_j\,\drv{\theta_j}{s}\\
%&= -\drv{\vec{\theta}}{s}.
%\end{align}

Given vector~$\vec{\theta}$, the associated rotation matrix can be computed as follows.
\begin{equation}\label{key}
\ten{R} = \exp{\ten{A}}, \qquad \ten{A}\tp = -\ten{A}.
\end{equation}

\begin{equation}\label{key}
	\ten{A} = \sum\limits_{j=1}^{3}\theta_j\,\ten{L}_j
	=
	\left[\begin{array}{ccc}
		0 & -\theta_3 & \theta_2\\
		\theta_3 & 0 & -\theta_1 \\
		-\theta_3& \theta_1 &0
	\end{array}\right]
\end{equation}

\begin{equation}\label{key}
	\ten{R} = \exp{\ten{A}} = \ten{\Phi}\,\exp{\i\ten{\Lambda}}\,\ten{\Phi}\tpc, \qquad \ten{A} = \ten{\Phi}\,\ten{\Lambda}\,\ten{\Phi}\tpc.
\end{equation}
Eigenvalues of $\ten{A}$ are
\begin{equation}\label{key}
	\diag\ten{\Lambda} = 
	\left[\begin{array}{ccc}
		0 \\ +\i\abs{\vec{\theta}} \\ -\i\abs{\vec{\theta}}	
	\end{array}\right],
	\qquad
	\abs{\vec{\theta}}^2 = \theta_1^2 + \theta_2^2+ \theta_3^2.
\end{equation}
And the eigenvectors are
\begin{equation}\label{key}
	\ten{\Phi} = 
	\left[\begin{array}{ccc}
		\vec{\varphi}_1 & \vec{\varphi}_2 & \vec{\varphi}_3
	\end{array}\right],
\end{equation}
where
\begin{align}\label{key}
	\vec{\varphi}_1 &= \frac{\vec{\theta}}{\abs{\vec{\theta}}} \\
	\vec{\varphi}_2 &= \frac{\vec{w}_1}{\sqrt{2}} + \i\,\frac{\vec{w}_2}{\sqrt{2}} \\
	\vec{\varphi}_3 &= \frac{\vec{w}_2}{\sqrt{2}} + \i\,\frac{\vec{w}_1}{\sqrt{2}}
\end{align}
with vectors $\vec{w}_1$ and $\vec{w}_2$ being any orthonormal basis of the orthogonal complement of $\vec{\theta}$.
Thus, the directors can be computed via
\begin{equation}\label{key}
	\vec{d}_j = \sum_{i=1}^{3}\Phi_{ji}\,\exp{\Lambda_{ii}}\vec{\varphi}_i, \qquad j=1..3.
\end{equation}



==> sections/sec_Homogenization.tex <==
For short fiber reinforced polymers, we can now embed the fibers within the matrix material. However, the size of the fibers is still to small for large components. Therefore,w e aim at a framework of the FE$^2$ method to solve the boundary value problems on two scale, the macroscopic as well as the microscopic scale.

\paragraph{Macroscopic scale.}
We assume again a Lipschitz bounded domain $\bar{\Omega}_0\subset\mathbb{R}^3$ with boundary $\partial\bar{\Omega}_0$, parametrised in the reference coordinates $\bar{\vec{X}}$ with corresponding actual position $\bar{\vec{x}} = \vec{\varphi}(\bar{\vec{X}})$. Analogues to the microscale defined on $\Omega_0$, we introduce the deformation gradient tensor field as
\begin{equation}
\bar{\vec{F}} = \nabla_{\bar{\vec{X}}}\bar{\vec{\varphi}}(\bar{\vec{X}}).
\end{equation}
The principle of virtual work reads
\begin{equation}
\int\limits_{\bar{\Omega}_0}\nabla_{\bar{\vec{X}}}(\delta\bar{\vec{\varphi}}):\bar{\vec{P}}\,\text{d}V = \int\limits_{\bar{\Omega}_0}\delta\bar{\vec{\varphi}}\cdot\bar{\vec{B}}\,\text{d}V +
\int\limits_{\bar{\Gamma}^{\sigma}}\delta\bar{\vec{\varphi}}\cdot\bar{\vec{T}}\,\text{d}A.
\end{equation}
As before, we prescribe Dirichlet and Neumann boundary conditions with the standard relationship $\partial\bar{\Omega}_0 = \bar{\Gamma}^{\varphi}\cup\bar{\Gamma}^{\sigma}$ and $\bar{\Gamma}^{\varphi}\cap\bar{\Gamma}^{\sigma} = \emptyset$. In contrast to the microscale, we do not consider a strain energy function, i.e. we do not know the analytic relation between $\bar{\vec{P}}$ and $\bar{\vec{F}} $. Instead, we assume at each point of the domain $\bar{\Omega}_0$, that
\begin{equation}\label{eq:homoP}
\bar{\vec{P}} = \frac{1}{V}\int\limits_{\Omega_0} \vec{P}\,\text{d}V,
\end{equation}
is valid. Therefore, it is necessary to assume that the domain $\Omega_0$ can be considered as representative with respect to the mechanical behavior, and we call the domain representative volume element (RVE).

\paragraph{Hill-Mandel criteria.}
Next, we postulate a generalized macro-homogeneity condition given by
\begin{equation}
\bar{\vec{P}} :\dot{\bar{\vec{F}}} - \frac{1}{V}\int\limits_{\Omega_0} \vec{P}:\dot{\vec{F}}\,\text{d}V = 0,
\end{equation}
also known as the classical Hill–Mandel macro-homogeneity condition. This condition can be used to derive suitable boundary conditions on $\partial\Omega$ in the RVE. There, we first reformulate the last equation as
\begin{equation}\label{eq:Hill}
\frac{1}{V}\int\limits_{\Omega_0}[\vec{P}-\bar{\vec{P}}]:[\dot{\vec{F}}-\dot{\bar{\vec{F}}}]\,\text{d}V,
\end{equation}
where we have assumed that
\begin{equation}
\bar{\vec{F}} = \frac{1}{V}\int\limits_{\Omega_0} \vec{F}\,\text{d}V.
\end{equation}
It can be shown that the latter statement is true, if the Hill-Mandel condition holds, see [???keip2012]. With this, we can derive general boundary conditions using a divergence theorem (c.f. [???steinmann2016AppB], such that
\begin{equation}
\int\limits_{\partial\Omega_0}[\vec{T}-\bar{\vec{P}}\vec{N}]\cdot[\dot{\vec{x}}-\dot{\bar{\vec{F}}}\vec{X}]\,\text{d}A = 0,
\end{equation}
is equivalent to the former condition. This can be achieved by applying either suitable periodic Neumann boundary condition, or by using periodic Dirichlet conditions on opposite faces of the RVE.

\textcolor{red}{I can write some more details here, if necessary.}

\paragraph{Consistent linearisation of the macroscopic field equation.}
To obtain optimal convergence of the Newton-Raphson iteration, we need a consistent linearisation of the macroscopic weak form. This is particular challenging, as we do not have an analytical expression for the macroscopic stress field, i.e. we need
\begin{equation}
\Delta\bar{\vec{P}} = \frac{\partial\bar{\vec{P}}}{\partial\bar{\vec{F}}} =: \bar{\mathbb{C}}.
\end{equation}
With \eqref{eq:homoP}, we obtain immediately
\begin{equation}
\bar{\mathbb{C}} = \frac{1}{V}\int\limits_{\Omega_0} \frac{\partial\vec{P}}{\partial\bar{\vec{F}}} ,\text{d}V.
\end{equation}
Note that $\vec{P}$ depends on the microscale deformation. Hence, the next step follows analoguesly to the linearisation procedure of the internal constraints in plasticity: We split the microscopic deformation gradient into the constant macroscopic contributions $\bar{\vec{F}}$ and microscopic fluctuations $\vec{\omega}(\vec{X})$ as follows
\begin{equation}
\vec{F} = \bar{\vec{F}} + \vec{F}_{\omega},\;\text{where}\; \vec{F}_{\omega} = \nabla_{\vec{X}}\vec{\omega}.
\end{equation}
This allows us to write
\begin{equation}\label{eq:C}
\bar{\mathbb{C}} = \frac{1}{V}\int\limits_{\Omega_0} \mathbb{C}:[\mathbb{I}+\frac{\partial\vec{F}_{\omega}}{\partial\bar{\vec{F}}}],\text{d}V,
\end{equation}
where we have assumed that $\vec{P}:=\vec{P}(\vec{\omega})$. We require now suitable constraints $\vec{\Phi}^{hom} := \vec{\Phi}^{hom}(\bar{\vec{F}},\vec{F}_{\omega})$, which allows a consistent linearisation via
\begin{equation}
\Delta\vec{\Phi}^{hom} = \frac{\partial\vec{\Phi}^{hom}}{\partial\bar{\vec{F}}}:\Delta\bar{\vec{F}} + \frac{\partial\vec{\Phi}^{hom}}{\partial\vec{F}_{\omega}}:\Delta\vec{F}_{\omega}.
\end{equation}
It is obvious that the converged local balance equations can be used for this purpose, i.e.
\begin{equation}
\vec{\Phi}^{hom} = \int\limits_{\Omega_0}\delta\vec{F}_{\omega}:\vec{P}\,\text{d}V - \int\limits_{\Gamma^{\sigma}}\delta\vec{\omega}\cdot\vec{T}\,\text{d}A,
\end{equation} 
where we assume the absence of body forces. For pure Dirichlet boundary conditions, we obtain
\begin{equation}
\int\limits_{\Omega_0}\nabla_{\vec{X}}(\delta\vec{\omega}):\mathbb{C}:[\Delta\bar{\vec{F}} + \Delta\vec{F}_{\omega}]\,\text{d}V = 0 \quad\forall\;\delta\vec{\omega},
\end{equation}
which can be resolved in the discrete setting to obtain the missing second term on the right hand side in \eqref{eq:C}. 




==> sections/sec_Preconditioner.tex <==
% !TeX root = ../MAIN.tex

\newcommand{\MatrixBlock}{{\ten{K}_{M}}}
\newcommand{\FiberBlock}{{\ten{K}_{F}}}
\newcommand{\MFBlock}{{\ten{K}_{N}}}
\newcommand{\FMBlock}{{\ten{K}_{Q}}}

Solution of the non-linear problem~\eqref{eq:sys1D/3D:matrix}-\eqref{eq:sys1D/3D:moments} with Newton-Raphson method leads to the linear system
\begin{equation}\label{eq:prec:linsys}
\ten{K}\,\vec{y} = \vec{b}
\end{equation}
where $\vec{y}$ stands for the increment of the extended vector of dofs (matrix displacements~$\vec{u}$, fiber directors~$\vec{R}_{F}$, moments~$\vec{M}$ and forces~$\vec{N}$), $\vec{b}$ is the residual and $\ten{K}$ is the tangent matrix:
\begin{equation}\label{key}
	\ten{K} = 
	\mat{
		\MatrixBlock 	& \MFBlock_1 		& \cdots 	& \MFBlock_n 	\\
		\FMBlock_1 		& \FiberBlock_1 	& 0 		& 0 			\\
		\vdots 			& 0 				& \ddots 	& 0 			\\
		\FMBlock_n 		& 0 				& 0 		& \FiberBlock_n 
	},
\end{equation}
with the blocks $\MatrixBlock$ and $\FiberBlock_i$ corresponding to the tangent matrices of material matrix and fiber~$i$ respectively, and $\MFBlock_i$ and $\FMBlock_i$ being associated to the corresponding matrix/fiber interaction force contributions.
The global tangent matrix~$\ten{K}$ can be decomposed as
\begin{equation}\label{key}
	\ten{K} = 
	\underbrace{\mat{
		\MatrixBlock 	& 0 				& 0	 		& 0 		 	\\
		\FMBlock_1 		& \FiberBlock_1 	& 0 		& 0 			\\
		\vdots 			& 0 				& \ddots 	& 0 			\\
		\FMBlock_n 		& 0 				& 0 		& \FiberBlock_n 
	}}_{\ten{L}}
	+
	\underbrace{\mat{
		0 	& \MFBlock_1 		& \cdots 	& \MFBlock_n 	\\
		0 		& 0 	& 0 		& 0 			\\
		0 			& 0 				& 0 	& 0 			\\
		0 		& 0 				& 0 		& 0 
	}}_{\ten{U}}.
\end{equation}
Thus, the linear system~\eqref{eq:prec:linsys} can be solved using Gauss-Seidel iterative process:
\begin{equation}\label{key}
	\ten{L}\vec{y}_{k+1} = \vec{b} - \ten{U}\vec{y}_{k},
\end{equation}
where at each iteration the linear system can be solved by Gauss elimination.
So the iterative process can be formulated within the following sketch:
\begin{enumerate}
	\item Given the fiber forces $\vec{N}_{k}$, solve the material matrix system only to obtain the dofs corresponding to the matrix displacements.
	\item Given the matrix displacements dofs, for each fiber, solve the fiber system only to obtain the dofs corresponding to the fiber directors~$\vec{R}_{F}$, moments~$\vec{M}$ and forces~$\vec{N}$.
	\item Update fiber forces~$\vec{N}_{k+1}$ and proceed to the next iteration.
\end{enumerate}

==> sections/sec_TorsionBlocking.tex <==
% !TeX root = ../MAIN.tex

\subsection{Torsion blocking.}
%\paragraph{Torsion blocking.}
Note that the system~\eqref{eq:sys:PG} (respectively~\eqref{eq:sys:IGAcollocation}) can not have a unique solution.

\begin{lemma}	
	Let $(\vec{u}_{M}, \vec{r}, \ten{R}_{F})$ be solution to~\eqref{eq:sys:PG}, and let
	\begin{equation}\label{key}
		\ten{\hat{R}} = \mat{
			1 & & \\
			 & \cos\alpha & -\sin\alpha \\
			 & \sin\alpha & \cos\alpha \\
		},
	\end{equation}
	with arbitrary $\alpha\in\R$.
	If for stiffness tensor~\eqref{eq:stifnessTensors}  $\stiffnessC_{22}=\stiffnessC_{33}$ and $\stiffnessD_{22}=\stiffnessD_{33}$, then $(\vec{u}_{M}, \vec{r}, \ten{R}_{F}\ten{\hat{R}})$ is also solution to~\eqref{eq:sys:PG}.
\end{lemma}

\begin{proof}
	If $\stiffnessC_{22}=\stiffnessC_{33}$, then  $\ten{R}_{F}\ten{\hat{R}}\,\stiffnessC\,\ten{\hat{R}}\tp\ten{R}_{F}\tp = \ten{R}_{F}\,\stiffnessC\,\ten{R}_{F}\tp$.
	And thus, $\vec{N}(\vec{r}, \ten{R}_{F}) = \vec{N}(\vec{r}, \ten{R}_{F}\ten{\hat{R}})$.
	
	If $\stiffnessD_{22}=\stiffnessD_{33}$, then $\ten{R}_{F}\ten{\hat{R}}\,\stiffnessD = \ten{R}_{F}\,\stiffnessD\ten{\hat{R}}$.	
%	\begin{equation}\label{key}
%	\ten{\hat{R}}\vec{\kappa} 
%	= 
%	-\ten{\hat{R}}\mat{
%		\vec{d}_3\tp\,\partial_{s}{\vec{d}_2} \\
%		\vec{d}_1\tp\,\partial_{s}{\vec{d}_3} \\
%		-\vec{d}_1\tp\,\partial_{s}{\vec{d}_2}
%	}
%	=
%	-\mat{
%		\vec{d}_3\tp\,\partial_{s}{\vec{d}_2} \\
%		\vec{d}_1\tp\,\partial_{s}{\left(\cos\alpha\vec{d}_3 + \sin\alpha\vec{d}_2 \right)} \\
%		-\vec{d}_1\tp\,\partial_{s}{\left(\cos\alpha\vec{d}_2 - \sin\alpha\right)}
%	}
%	\end{equation}
	Hence, using the fact that \rev{(to check !!)}
	\begin{align}\label{key}
	\vec{\kappa}(\ten{R}_{F}\ten{\hat{R}})
	&=
	\frac{1}{2}\,\axl\left(\ten{\hat{R}}\tp\ten{R}_{F}\tp\,\drv{\ten{R}_{F}}{s}\ten{\hat{R}}\right)
	=
	\ten{\hat{R}}\tp\frac{1}{2}\,\axl\left(\ten{R}_{F}\tp\,\drv{\ten{R}_{F}}{s}\right) = \ten{\hat{R}}\tp\vec{\kappa}(\ten{R}_{F}),
	\end{align}
	we obtain  $\vec{M}(\ten{R}_{F}) = \vec{M}(\ten{R}_{F}\ten{\hat{R}})$.	
	Hence follows the statement.

	
\end{proof}

In order to fix the rotation, we impose additional moment in one of the fiber ends (here at $s=0$):
\begin{equation}\label{key}
	\vec{M}(0) = \mat{\vec{d}_2\cdot\vec{d}_3 \\ 0\\ 0}.
\end{equation}




==> sections/sec_discretization.tex <==
Concerning the spatial approximation, suitable isogeometric discretisation schemes are applied for the different fields. In particular, a standard IGA approach is applied to the matrix material, whereas a collocation type method is used to discretise the weighted residual. 

%For the coupling condition, the Lagrange multipliers are defined on the beam, which allows for a local condensation procedure of the position constraints.

\paragraph{Matrix material.}
A standard displacement-based finite element approach employs approximations of the deformation field $\vec{\varphi}$ and its variation of the form
\begin{equation}\label{eq:approxGeo}
\vec{\varphi}^{\mathrm{h}}=\sum\limits_{A\in\mathcal{I}}R^{A}\vec{q}_{A} \quad\text{and}\quad\delta\vec{\varphi}^{\mathrm{h}} =\sum\limits_{A\in\mathcal{I}}R^{A}\delta\vec{q}_{A},  
\end{equation}
respectively, where $\vec{q}_{A}\in\mathbb{R}^3$ and $\delta\vec{q}_{A}\in\mathbb{R}^3$. Here, \(R^A:\mathcal{B}_0^{\mathrm{h}}\rightarrow\mathbb{R}\) are NURBS based shape functions associated with control points \(A\in\mathcal{I}=\{1,\,\hdots,\,\mathfrak{M}\}\), where \(\mathfrak{M}\) denote the overall number of control points.
%
%\begin{equation}\label{eq:nurbs}
%R^{A} := R^{\vec{i}}(\vec{\xi}) = \frac{\prod\limits_{\alpha=1}^{3}B^{i_{\alpha}}(\xi^{\alpha})w_{\vec{i}}}{\sum\limits_{\vec{j}}\prod\limits_{\alpha=1}^{3}B^{j_{\alpha}}(\xi^{\alpha})w_{\vec{j}}},
%\end{equation}
%where \(B^{i_{\alpha}}\) are univariate non-rational B-splines defined on a parametric domain which is subdivided by the knot vector \([\xi_{1}^{\alpha},\xi_{2}^{\alpha},\hdots,\xi_{\mathfrak{N}_{\alpha}+p_{\alpha}+1}^{\alpha}]\). The recursive definition of a single univariate B-spline is given as follows
%\begin{equation}
%B^{i_{\alpha}}_{p_{\alpha}}(\xi^{\alpha})=\frac{\xi^{\alpha}-\xi^{\alpha}_{i_{\alpha}}}{\xi^{\alpha}_{i_{\alpha}+p_{\alpha}}-\xi^{\alpha}_{i_{\alpha}}}B^{i_{\alpha}}_{p_{\alpha}-1}(\xi^{\alpha})+\frac{\xi^{\alpha}_{i_{\alpha}+p_{\alpha}+1}-\xi^{\alpha}}{\xi^{\alpha}_{i_{\alpha}+p_{\alpha}+1}-\xi^{\alpha}_{i_{\alpha}+1}}B^{i_{\alpha}+1}_{p_{\alpha}-1}(\xi^{\alpha}),
%\end{equation}
%beginning with
%\begin{equation}
%B_{0}^{i_{\alpha}}(\xi^{\alpha})=\left\{\begin{array}{l}1\quad\text{if}\;\xi_{i_{\alpha}}\leq\xi^{\alpha}<\xi^{\alpha}_{i_{\alpha}+1} \\ 0\quad\text{otherwise}\end{array}\right. . 
%\end{equation}
%Here, \(w_{\vec{j}}\) are corresponding NURBS weights. 
%
The discrete form of \eqref{eq:pdvA} reads now
\begin{equation}\label{eq:pdvADis}
\delta\vec{q}_A\cdot\int\limits_{\Omega_0}\vec{P}\nabla_{\vec{X}}(R^A)\,\text{d}V - \delta\vec{q}_A\cdot\int\limits_{\Omega_0}R^A\vec{B}^{\mathrm{h}}_{ext}\,\text{d}V -
\delta\vec{q}_A\cdot\int\limits_{\Gamma^{\sigma}}R^a\vec{T}^{\mathrm{h}}_{ext}\,\text{d}A = 0,\quad\forall\delta\vec{q}_A,
\end{equation}
where $\vec{T}^{\mathrm{h}}_{ext}$ and $\vec{B}^{\mathrm{h}}_{ext}$ are appropriately approximated external contributions.

\paragraph{Beams.}
For the beam, we require in a first step the approximations of the centerline and the rotations. As all three parameter formulations involve the risk singularities, we use quaternions $\mathfrak{q}$, c.f. Appendix \ref{app:quarternions}. The approximation along the centerline is given by
\begin{equation}
\tilde{\vec{\varphi}}^{\mathrm{h}}=\sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\tilde{\vec{q}}_{A} \quad\text{and}\quad\mathfrak{q}^{\mathrm{h}}=\sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\mathfrak{q}_{A}.
\end{equation}
Here, $\tilde{R}^{A}:\mathfrak{C}_0^{\mathrm{h}}\rightarrow\mathbb{R}$ are one-dimensional, NURBS based shape functions with associated control points $A\in\mathcal{J} = \{1,\hdots,\mathfrak{O}\}$. For the mixed formulation as introduced before, additional approximations are required for the resultants
\begin{equation}
\mathfrak{n}^{\mathrm{h}}=\sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\mathfrak{n}_{A}\quad\text{and}\quad\mathfrak{m}^{\mathrm{h}}=\sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\mathfrak{m}_{A}.
\end{equation}
The test functions $\delta\tilde{\vec{\varphi}}^{\mathrm{h}}$ and $\delta\tilde{\vec{\phi}}^{\mathrm{h}}$ and in the context of the applied mixed method, $\delta\mathfrak{g}^{\mathrm{h}}$ and $\delta\mathfrak{k}^{\mathrm{h}}$ are discretised via a set of Dirac $\delta_{\mathfrak{C}_0^{\mathrm{h}}}$ functions, given as
\begin{equation}
\delta\tilde{\vec{\varphi}}^{\mathrm{h}} = \sum\limits_{i\in\mathcal{J}} \delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tilde{\vec{x}}-\tilde{\vec{x}}_i)\delta\tilde{\vec{q}}_i,\;
%\delta\mathfrak{q}^{\mathrm{h}}=\sum\limits_{i\in\mathcal{J}} \delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tilde{\vec{x}}-\tilde{\vec{x}}_i)\delta\mathfrak{q}_{A},\;
\delta\tilde{\vec{\phi}}^{\mathrm{h}} = \sum\limits_{i\in\mathcal{J}} \delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tilde{\vec{x}}-\tilde{\vec{x}}_i)\delta\tilde{\vec{\phi}}_i,
\end{equation}
and
\begin{equation}
\delta\mathfrak{g}^{\mathrm{h}} = \sum\limits_{i\in\mathcal{J}} \delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tilde{\vec{x}}-\tilde{\vec{x}}_i)\delta\mathfrak{g}_i,\quad
\delta\mathfrak{k}^{\mathrm{h}} = \sum\limits_{i\in\mathcal{J}} \delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tilde{\vec{x}}-\tilde{\vec{x}}_i)\delta\mathfrak{k}_i,
\end{equation}
where the \textit{collocation} points $\tilde{\vec{x}}_i$ are aligned at the beam center line. We refer to \cite{Weeger2018} for a proper choice of the collocation points $\tilde{\vec{x}}_i$ in terms of the Greville abscissae of the spline knot vector. 
%
%Taking the so-called sifting property (see \cite{hughes2013}, Section 2.2.2 for details) 
%\begin{equation}
%\int\limits_{\mathfrak{C}_0^{\mathrm{h}}}g(\tilde{\vec{x}})\delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tilde{\vec{x}}-\tilde{\vec{x}}_i)\d s = g(\tilde{\vec{x}_i}),
%\end{equation}
%into account, 
%
The discrete principle of virtual work for the beam contributions as given in \eqref{eq:pdvaHW2} reads
\begin{equation}
\begin{aligned}
&-\delta\tilde{\vec{q}}_i\cdot\left(\mathfrak{n}^{\mathrm{h}}(\tilde{\vec{x}}_i)^{\prime} + \bar{\tilde{\vec{n}}}^{\mathrm{h}}(\tilde{\vec{x}}_i)\right)
-\delta\tilde{\vec{\phi}}_i\cdot\left(\mathfrak{m}^{\mathrm{h}}(\tilde{\vec{x}}_i)^{\prime} + \tilde{\vec{\varphi}}^{\mathrm{h}}(\tilde{\vec{x}}_i)^{\prime}\times\mathfrak{n}^{\mathrm{h}}(\tilde{\vec{x}}_i) + \bar{\tilde{\vec{m}}}^{\mathrm{h}}(\tilde{\vec{x}}_i)\right) +\\
&\delta\mathfrak{g}_i\cdot\left(\mathfrak{n}^{\mathrm{h}}(\tilde{\vec{x}}_i) - \tilde{\vec{R}}(\tilde{\vec{x}}_i)\frac{\partial\tilde{\Psi}}{\partial\vec{\Gamma}}(\vec{\Gamma}^{\mathrm{h}}(\tilde{\vec{x}}_i),\vec{K}^{\mathrm{h}}(\tilde{\vec{x}}_i))\right)+\\
&\delta\mathfrak{k}_i\cdot\left(\mathfrak{m}^{\mathrm{h}}(\tilde{\vec{x}}_i) - \tilde{\vec{R}}(\tilde{\vec{x}}_i)\frac{\partial\tilde{\Psi}}{\partial\vec{K}}(\vec{\Gamma}^{\mathrm{h}}(\tilde{\vec{x}}_i),\vec{K}^{\mathrm{h}}(\tilde{\vec{x}}_i))\right) = 0\quad\forall \delta\tilde{\vec{q}}_i,\delta\tilde{\vec{\phi}}_i,\delta\mathfrak{g}_i,\delta\mathfrak{k}_i.
\end{aligned}
\end{equation}
If quaternions are used, the additional constraint $\mathfrak{q}^{\mathrm{h}}(\tilde{\vec{x}}_i)\cdot\mathfrak{q}^{\mathrm{h}}(\tilde{\vec{x}}_i) - 1 = 0$ is enforced at every collocation points to ensure that the rotation matrix $\tilde{\vec{R}}(\tilde{\vec{x}}_i)$ is orthonormal.


\paragraph{Coupling conditions.}
Next, we introduce suitable approximation for the Lagrange multipliers related to the first coupling conditions presented in \eqref{eq:pi1} as
\begin{equation}
\bar{\vec{\mu}}^{\mathrm{h}} = \sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\bar{\vec{\mu}}_{A},\quad  \delta\bar{\vec{\mu}}^{\mathrm{h}} = \sum\limits_{i\in\mathcal{J}} \delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tilde{\vec{x}}-\tilde{\vec{x}}_i)\delta\bar{\vec{\mu}}_i,
\end{equation}
following the discretisation of the beam, along which we define the Lagrange multipliers. With regard to \eqref{eq:pi1}, we obtain
\begin{equation}
\delta\Pi_C^1 = \delta\bar{\vec{\mu}}_i\cdot(\vec{x}^{\mathrm{h}}_{i} - \tilde{\vec{\varphi}}^{\mathrm{h}}(\tilde{\vec{x}}_i))|C(s)|  - 
\delta\tilde{\vec{q}}_i\cdot\bar{\vec{\mu}}^{\mathrm{h}}(\tilde{\vec{x}}_i)|C(s)| +
\delta\vec{q}_A\cdot\int\limits_{\mathfrak{C}_0} R^A\bar{\vec{\mu}}^{\mathrm{h}}|C(s)|\d s
\end{equation}
where $\tilde{\vec{\varphi}}^{\mathrm{h}}(\tilde{\vec{x}}_i)$ is the position of the centerline evaluated at the collocation point $\tilde{\vec{x}}_i$. Moreover, $\vec{x}^{\mathrm{h}}_{i} = \sum\limits_{A\in\mathcal{I}}R^{A}(\vec{\xi}_{i})\vec{q}_{A}$ is the corresponding positions in the matrix material. For the virtual work expression presented in \eqref{eq:moments_constrain} with regard to the reformulation in \eqref{eq:sys:moments2}, we introduce the discrete Lagrange multipliers
\begin{equation}
\vec{\mu}_{\tau}^{\mathrm{h}} = \sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\vec{\mu}^{\tau}_{A},\quad  \delta\vec{\mu}_{\tau}^{\mathrm{h}} = \sum\limits_{i\in\mathcal{J}} \delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tilde{\vec{x}}-\tilde{\vec{x}}_i)\delta\vec{\mu}^{\tau}_{i},
\end{equation}
and the abbreviation $\mathfrak{G}_i = \nabla_{\vec{X}}(R^A(\vec{\xi}_i))\vec{q}_A\,\ten{P}_{12}(\tilde{\vec{x}}_i)\fib{\ten{R}}\tp(\tilde{\vec{x}}_i)$, we obtain
\begin{equation}
\begin{aligned}
\delta\Pi_C^2 = &\delta\vec{\mu}^{\tau}_{i}\cdot\axl\left(\mathfrak{G}_i\right)\abs{C} +
\delta\tilde{\vec{\phi}}_i\cdot\left(\ten{\Id}-\mathfrak{G}_i\right)\vec{\mu}_{\tau}^{\mathrm{h}}(\tilde{\vec{x}}_i) \abs{C}+\\
&\delta\vec{q}_A\cdot\int\limits_{\mathfrak{C}_0}\frac{1}{2}\,\left(\vec{\mu}_{\tau}\times\vec{d}_{\alpha}\otimes\vec{D}_{\alpha}\right) \nabla_{\vec{X}}(R^A)\abs{C}\d s.
\end{aligned}
\end{equation}
Finally, we introduce the last set of discrete Lagrange multipliers
\begin{equation}
\mu_n^{\mathrm{h}} = \sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\mu^n_A,\quad  \delta\mu_n^{\mathrm{h}} = \sum\limits_{i\in\mathcal{J}} \delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tilde{\vec{x}}-\tilde{\vec{x}}_i)\delta\mu^n_i,
\end{equation}
and obtain
\begin{equation}
\delta\Pi_C^3 = \delta\mu_1^n\left(\frac{1}{2}\tr\left( \mathfrak{G}_i\right)-1\right)\abs{C}  + 
\delta\vec{q}_A\cdot\int\limits_{\mathfrak{C}_0}\frac{1}{2}\,\left(\mu_n\vec{d}_{\alpha}\otimes\vec{D}_{\alpha}\right) \nabla_{\vec{X}}(R^A)\abs{C}\d s.
\end{equation}



\rev{Reminder: Endpoints.}


\paragraph{Total system.}
For the matrix material, we have to solve
\begin{equation}\label{eq:pdvADis2}
\begin{aligned}
&\int\limits_{\Omega_0}\vec{P}\nabla_{\vec{X}}(R^A)\,\text{d}V - \int\limits_{\Omega_0}R^A\vec{B}^{\mathrm{h}}_{ext}\,\text{d}V -
\int\limits_{\Gamma^{\sigma}}R^A\vec{T}^{\mathrm{h}}_{ext}\,\text{d}A +\\
&\int\limits_{\mathfrak{C}_0}\left[R^A\bar{\vec{\mu}}^{\mathrm{h}} + 
\frac{1}{2}\,\left(\vec{\mu}_{\tau}\times\vec{d}_{\alpha}\otimes\vec{D}_{\alpha}+\mu_n\vec{d}_{\alpha}\otimes\vec{D}_{\alpha}\right) \nabla_{\vec{X}}(R^A)\right]\abs{C}\d s = \vec{0},
\end{aligned}
\end{equation}
for every node $A$. Additionally, at every collocation point $\tilde{\vec{x}}_i$ we solve the balance and constitutive equations
\begin{equation}\label{eq:beamDis}
\begin{aligned}
\vec{0} &= \mathfrak{n}^{\mathrm{h}}(\tilde{\vec{x}}_i)^{\prime} + \bar{\tilde{\vec{n}}}^{\mathrm{h}}(\tilde{\vec{x}}_i) + \bar{\vec{\mu}}^{\mathrm{h}}(\tilde{\vec{x}}_i)
|C(\tilde{\vec{x}}_i)| \\
\vec{0} &= \mathfrak{m}^{\mathrm{h}}(\tilde{\vec{x}}_i)^{\prime} + \tilde{\vec{\varphi}}^{\mathrm{h}}(\tilde{\vec{x}}_i)^{\prime}\times\mathfrak{n}^{\mathrm{h}}(\tilde{\vec{x}}_i) + 
\bar{\tilde{\vec{m}}}^{\mathrm{h}}(\tilde{\vec{x}}_i) -\left(\ten{\Id}-\frac{1}{2}\mathfrak{G}_i\right)\vec{\mu}_{\tau}^{\mathrm{h}}(\tilde{\vec{x}}_i) \abs{C(\tilde{\vec{x}}_i)},\\
\vec{0} &= \mathfrak{n}^{\mathrm{h}}(\tilde{\vec{x}}_i) - \tilde{\vec{R}}^{\mathrm{h}}(\tilde{\vec{x}}_i)\frac{\partial\tilde{\Psi}}{\partial\vec{\Gamma}}(\vec{\Gamma}^{\mathrm{h}}(\tilde{\vec{x}}_i),\vec{K}^{\mathrm{h}}(\tilde{\vec{x}}_i)),\\
\vec{0} &= \mathfrak{m}^{\mathrm{h}}(\tilde{\vec{x}}_i) - \tilde{\vec{R}}^{\mathrm{h}}(\tilde{\vec{x}}_i)\frac{\partial\tilde{\Psi}}{\partial\vec{K}}(\vec{\Gamma}^{\mathrm{h}}(\tilde{\vec{x}}_i),\vec{K}^{\mathrm{h}}(\tilde{\vec{x}}_i)),\\
0 &= \mathfrak{q}^{\mathrm{h}}(\tilde{\vec{x}}_i)\cdot\mathfrak{q}^{\mathrm{h}}(\tilde{\vec{x}}_i) - 1\\
\end{aligned}
\end{equation}
along with
\begin{equation}\label{eq:disc:constraints}
\begin{aligned}
\vec{0} &=(\vec{x}^{\mathrm{h}}_{i} - \tilde{\vec{\varphi}}^{\mathrm{h}}(\tilde{\vec{x}}_i))|C(\tilde{\vec{x}}_i)|,\\
\vec{0} &= \axl\left(\mathfrak{G}_i\right)\abs{C(\tilde{\vec{x}}_i)},\\
0 &= \frac{1}{2}\left(\tr\left( \mathfrak{G}_i\right)-1\right)\abs{C(\tilde{\vec{x}}_i)}.
\end{aligned}
\end{equation}
\rev{Factor $\abs{C}$ can be omitted by scaling both sides. }

Note that the rotation is written in terms of quaternions, i.e. $\tilde{\vec{R}}^{\mathrm{h}}(\tilde{\vec{x}}_i) := \tilde{\vec{R}}^{\mathrm{h}}(\mathfrak{q}(\tilde{\vec{x}}_i))$, evaluated at the Greville point.

\paragraph{Reduced system.}
The condensed system as presented in \eqref{eq:sys:matrix_condense3} reads 
\begin{equation}\label{eq:red2}
\begin{aligned}
&\int\limits_{\Omega_0}\vec{P}\nabla_{\vec{X}}(R^A)\,\text{d}V - \int\limits_{\Omega_0}R^A\vec{B}^{\mathrm{h}}_{ext}\,\text{d}V -
\int\limits_{\Gamma^{\sigma}}R^A\vec{T}^{\mathrm{h}}_{ext}\,\text{d}A +
\int\limits_{\mathfrak{C}_0}\left(\mathfrak{n}^{\mathrm{h}}\otimes\vec{D}_3\nabla_{\vec{X}}(R^A)-R^A\bar{\tilde{\vec{n}}}^{\mathrm{h}}\right)\d s \\
 &+\frac{1}{2}\int\limits_{\mathfrak{C}_0}\left[\left(\ten{A}^{\mathrm{h}}\,\mathfrak{m}^{\mathrm{h}}\times\tilde{\vec{R}}^{\mathrm{h}}\vec{D}_{\alpha}\right)\otimes\vec{D}_\alpha\otimes\vec{D}_3\right]\,:\,\nabla^2_{\vec{X}}(\delta R^A)
+ \biggl[ 
\left(\ten{A}^{\mathrm{h}}\,\mathfrak{m}^{\mathrm{h}}\times\tilde{\vec{R}}^{\mathrm{h}}\vec{D}_{\alpha}\right)\otimes\nabla\vec{D}_\alpha\,\vec{D}_3\\
&-\left(\nabla\left(\left[\vec{d}_\alpha\right]_\times\,\ten{A}^{\mathrm{h}}\right):(\mathfrak{m}^{\mathrm{h}}\otimes\vec{D}_3)\right)\otimes\vec{D}_\alpha
-\left(\ten{A}^{\mathrm{h}}\,\left(\tilde{\vec{\varphi}}^{\mathrm{h},\prime}\times{\mathfrak{n}}^{\mathrm{h}} +\bar{\tilde{\vec{m}}}^{\mathrm{h}}\right)\times\vec{d}_\alpha\right)\otimes\vec{D}_\alpha
\biggl]\nabla_{\vec{X}}(R^A)\d s \\
& \int\limits_{\mathfrak{C}_0}\frac{1}{2}\,\mu_n^{\mathrm{h}}\vec{d}_{\alpha}\nabla_{\vec{X}}(R^A)\,\vec{D}_{\alpha} \abs{C}\d s +
\sum_{s=0,L} \frac{1}{2}\,\mu_n^s\vec{d}_{\alpha}\nabla_{\vec{X}}(R^A_s)\,\vec{D}_{\alpha}\, |A|= \vec{0},
\end{aligned}
\end{equation}
evaluated at every node $A$. Note that beam values like e.g. $\mathfrak{n}^{\mathrm{h}} = \tilde{R}^A\mathfrak{n}_A$ are written in terms of the 1D shape functions of the beam. Moreover, $\ten{A}^{\mathrm{h}} = \left(\ten{\Id}-\frac{1}{2}\mathfrak{G}\right)^{-1}$. Additionally, we enforce at every Greville point
\begin{equation}\label{eq:beamDis2}
\begin{aligned}
\vec{0} &= \mathfrak{n}^{\mathrm{h}}(\tilde{\vec{x}}_i) - \tilde{\vec{R}}^{\mathrm{h}}(\tilde{\vec{x}}_i)\frac{\partial\tilde{\Psi}}{\partial\vec{\Gamma}}(\vec{\Gamma}^{\mathrm{h}}(\tilde{\vec{x}}_i),\vec{K}^{\mathrm{h}}(\tilde{\vec{x}}_i)),\\
\vec{0} &= \mathfrak{m}^{\mathrm{h}}(\tilde{\vec{x}}_i) - \tilde{\vec{R}}^{\mathrm{h}}(\tilde{\vec{x}}_i)\frac{\partial\tilde{\Psi}}{\partial\vec{K}}(\vec{\Gamma}^{\mathrm{h}}(\tilde{\vec{x}}_i),\vec{K}^{\mathrm{h}}(\tilde{\vec{x}}_i)),\\
0 &= \mathfrak{q}^{\mathrm{h}}(\tilde{\vec{x}}_i)\cdot\mathfrak{q}^{\mathrm{h}}(\tilde{\vec{x}}_i) - 1\\
\end{aligned}
\end{equation}
along with
\begin{equation}\label{eq:constraints2}
\begin{aligned}
\vec{0} &=(\vec{x}^{\mathrm{h}}_{i} - \tilde{\vec{\varphi}}^{\mathrm{h}}(\tilde{\vec{x}}_i))|C(\tilde{\vec{x}}_i)|,\\
\vec{0} &= \axl\left(\mathfrak{G}_i\right)\abs{C(\tilde{\vec{x}}_i)},\\
0 &= \frac{1}{2}\left(\tr\left( \mathfrak{G}_i\right)-1\right)\abs{C(\tilde{\vec{x}}_i)}.
\end{aligned}
\end{equation}
\rev{ Duplicating \eqref{eq:disc:constraints} several lines above. }

\paragraph{Discrete reduction scheme.}
Within the Newton-Raphson iteration, we have to solve at every step
\begin{equation}\label{eq:newton}
\begin{bmatrix}
\vec{K}_{\vec{\varphi}\vec{\varphi}} & \vec{K}_{\vec{\varphi}\tilde{\vec{\varphi}}} & 
\vec{K}_{\vec{\varphi}\mathfrak{n}} & \vec{K}_{\vec{\varphi}\mathfrak{m}} & 
\vec{K}_{\vec{\varphi}\mathfrak{q}} & \vec{K}_{\vec{\varphi}\mu_n} \\
\vec{K}_{\tilde{\vec{\varphi}}\vec{\varphi}} & \vec{K}_{\tilde{\vec{\varphi}}\tilde{\vec{\varphi}}} & \vec{0} & \vec{0} & \vec{0} & \vec{0} \\
\vec{0} & \vec{K}_{\mathfrak{n}\tilde{\vec{\varphi}}} &
\ten{\Id}_{\mathfrak{n}\mathfrak{n}} & \vec{0} & \vec{K}_{\mathfrak{n}\mathfrak{q}} & \vec{0} \\
\vec{0} & \vec{0} & \vec{0} & \ten{\Id}_{\mathfrak{m}\mathfrak{m}} & \vec{K}_{\mathfrak{m}\mathfrak{q}} & \vec{0} \\
\vec{K}_{\mathfrak{q}\vec{\varphi}} & \vec{0} & \vec{0} & \vec{0} & \vec{K}_{\mathfrak{q}\mathfrak{q}} & \vec{0} \\
\vec{K}_{\mu_n\vec{\varphi}} & \vec{0} & \vec{0} & \vec{0} & \vec{K}_{\mu_n\mathfrak{q}} & \vec{0}
\end{bmatrix}
\begin{bmatrix}
\Delta\vec{\varphi}\\
\Delta\tilde{\vec{\varphi}}\\
\Delta\mathfrak{n}\\
\Delta\mathfrak{m}\\
\Delta\mathfrak{q}\\
\Delta\vec{\mu}_n
\end{bmatrix} =
\begin{bmatrix}
\vec{R}_{\vec{\varphi}}\\
\vec{R}_{\tilde{\vec{\varphi}}}\\
\vec{R}_{\mathfrak{n}}\\
\vec{R}_{\mathfrak{m}}\\
\vec{R}_{\mathfrak{q}}\\
\vec{R}_{\mu_n}
\end{bmatrix},
\end{equation}
where we have made use of \eqref{eq:simpleMat}. Here, $\vec{R}_{\vec{\varphi}}$ correlates to \eqref{eq:red2}, $\vec{R}_{\tilde{\vec{\varphi}}}$ to \eqref{eq:constraints2}$_1$, $\vec{R}_{\mathfrak{n}}$ to \eqref{eq:beamDis2}$_1$, $\vec{R}_{\mathfrak{m}}$ to \eqref{eq:beamDis2}$_2$, $\vec{R}_{\mathfrak{q}}$ to \eqref{eq:beamDis2}$_3$ and \eqref{eq:constraints2}$_2$ and eventually $\vec{R}_{\mu_n}$ to \eqref{eq:constraints2}$_3$. Note, that the condensed system is not symmetric any more. Next, we solve the third and fourth line in \eqref{eq:newton}
\begin{equation}\label{eq:reduction1}
\Delta\mathfrak{n} = 
\vec{R}_{\mathfrak{n}}-\vec{K}_{\mathfrak{n}\tilde{\vec{\varphi}}}\Delta\tilde{\vec{\varphi}}-\vec{K}_{\mathfrak{n}\mathfrak{q}}\Delta\mathfrak{q},\quad
\Delta\mathfrak{m} = \vec{R}_{\mathfrak{m}}-\vec{K}_{\mathfrak{m}\mathfrak{q}}\Delta\mathfrak{q}.
\end{equation}
and obtain
\begin{equation}\label{eq:newton3}
\begin{bmatrix}
\vec{K}_{\vec{\varphi}\vec{\varphi}} & \bar{\vec{K}}_{\vec{\varphi}\tilde{\vec{\varphi}}} & 
\bar{\vec{K}}_{\vec{\varphi}\mathfrak{q}} & \vec{K}_{\vec{\varphi}\mu_n} \\
\vec{K}_{\tilde{\vec{\varphi}}\vec{\varphi}} & \vec{K}_{\tilde{\vec{\varphi}}\tilde{\vec{\varphi}}} & \vec{0} & \vec{0} \\
\vec{K}_{\mathfrak{q}\vec{\varphi}} & \vec{0} & \vec{K}_{\mathfrak{q}\mathfrak{q}} & \vec{0} \\
\vec{K}_{\mu_n\vec{\varphi}} & \vec{0} & \vec{K}_{\mu_n\mathfrak{q}} & \vec{0}
\end{bmatrix}
\begin{bmatrix}
\Delta\vec{\varphi}\\
\Delta\tilde{\vec{\varphi}}\\
\Delta\mathfrak{q}\\
\Delta\vec{\mu}_n
\end{bmatrix} =
\begin{bmatrix}
\bar{\vec{R}}_{\vec{\varphi}}\\
\vec{R}_{\tilde{\vec{\varphi}}}\\
\vec{R}_{\mathfrak{q}}\\
\vec{R}_{\mu_n}
\end{bmatrix},
\end{equation}
where $\bar{\vec{K}}_{\vec{\varphi}\tilde{\vec{\varphi}}} = \vec{K}_{\vec{\varphi}\tilde{\vec{\varphi}}}-\vec{K}_{\vec{\varphi}\mathfrak{n}}\vec{K}_{\mathfrak{n}\tilde{\vec{\varphi}}} $, $\bar{\vec{K}}_{\vec{\varphi}\mathfrak{q}} = \vec{K}_{\vec{\varphi}\mathfrak{q}}-\vec{K}_{\vec{\varphi}\mathfrak{m}}\vec{K}_{\mathfrak{m}\mathfrak{q}} -\vec{K}_{\vec{\varphi}\mathfrak{n}}\vec{K}_{\mathfrak{n}\mathfrak{q}}$ and $\bar{\vec{R}}_{\vec{\varphi}} = \vec{R}_{\vec{\varphi}}-\vec{K}_{\vec{\varphi}\mathfrak{m}}\vec{R}_{\mathfrak{m}}-\vec{K}_{\vec{\varphi}\mathfrak{n}}\vec{R}_{\mathfrak{n}}$. For the second last reduction step, we remove the second line using
\begin{equation}\label{eq:reduction3}
\Delta\tilde{\vec{\varphi}} = \vec{K}_{\tilde{\vec{\varphi}}\tilde{\vec{\varphi}}}^{-1}(\vec{R}_{\tilde{\vec{\varphi}}}-\vec{K}_{\tilde{\vec{\varphi}}\vec{\varphi}}\Delta\vec{\varphi}).
\end{equation}
and obtain
\begin{equation}\label{eq:newton4}
\begin{bmatrix}
\vec{K}_{\vec{\varphi}\vec{\varphi}}-\bar{\vec{K}}_{\vec{\varphi}\tilde{\vec{\varphi}}}\vec{K}_{\tilde{\vec{\varphi}}\tilde{\vec{\varphi}}}^{-1}\vec{K}_{\tilde{\vec{\varphi}}\vec{\varphi}}  & \bar{\vec{K}}_{\vec{\varphi}\mathfrak{q}} & \vec{K}_{\vec{\varphi}\mu_n} \\
\vec{K}_{\mathfrak{q}\vec{\varphi}} & \vec{K}_{\mathfrak{q}\mathfrak{q}} & \vec{0} \\
\vec{K}_{\mu_n\vec{\varphi}} & \vec{K}_{\mu_n\mathfrak{q}} & \vec{0}
\end{bmatrix}
\begin{bmatrix}
\Delta\vec{\varphi}\\
\Delta\mathfrak{q}\\
\Delta\vec{\mu}_n
\end{bmatrix} =
\begin{bmatrix}
\bar{\vec{R}}_{\vec{\varphi}}-\bar{\vec{K}}_{\vec{\varphi}\tilde{\vec{\varphi}}}\vec{K}_{\tilde{\vec{\varphi}}\tilde{\vec{\varphi}}}^{-1}\vec{R}_{\tilde{\vec{\varphi}}}\\
\vec{R}_{\mathfrak{q}}\\
\vec{R}_{\mu_n}
\end{bmatrix}.
\end{equation}
Again, we used the block diagonality of $\vec{K}_{\tilde{\vec{\varphi}}\tilde{\vec{\varphi}}}$ and will use $\vec{K}_{\mathfrak{q}\mathfrak{q}}$ to calculate
\begin{equation}\label{eq:reduction4}
\Delta\mathfrak{q} = \vec{K}_{\mathfrak{q}\mathfrak{q}}^{-1}(\vec{R}_{\mathfrak{q}}-\vec{K}_{\mathfrak{q}\vec{\varphi}}\Delta\vec{\varphi}),
\end{equation}
such that
\begin{equation}\label{eq:newton5}
\begin{bmatrix}
\widetilde{\vec{K}}_{\vec{\varphi}\vec{\varphi}} & \vec{K}_{\vec{\varphi}\mu_n} \\
\vec{K}_{\mu_n\vec{\varphi}} - \vec{K}_{\mu_n\mathfrak{q}}\vec{K}_{\mathfrak{q}\mathfrak{q}}^{-1}\vec{K}_{\mathfrak{q}\vec{\varphi}} & \vec{0}
\end{bmatrix}
\begin{bmatrix}
\Delta\vec{\varphi}\\
\Delta\vec{\mu}_n
\end{bmatrix} =
\begin{bmatrix}
\bar{\vec{R}}_{\vec{\varphi}}-\bar{\vec{K}}_{\vec{\varphi}\tilde{\vec{\varphi}}}\vec{K}_{\tilde{\vec{\varphi}}\tilde{\vec{\varphi}}}^{-1}\vec{R}_{\tilde{\vec{\varphi}}}
-\bar{\vec{K}}_{\vec{\varphi}\mathfrak{q}}\vec{K}_{\mathfrak{q}\mathfrak{q}}^{-1}\vec{R}_{\mathfrak{q}}\\
\vec{R}_{\mu_n}-\vec{K}_{\mu_n\mathfrak{q}}\vec{K}_{\mathfrak{q}\mathfrak{q}}^{-1}\vec{R}_{\mathfrak{q}}
\end{bmatrix},
\end{equation}
where $\widetilde{\vec{K}}_{\vec{\varphi}\vec{\varphi}} = \vec{K}_{\vec{\varphi}\vec{\varphi}}
-\bar{\vec{K}}_{\vec{\varphi}\tilde{\vec{\varphi}}}\vec{K}_{\tilde{\vec{\varphi}}\tilde{\vec{\varphi}}}^{-1}\vec{K}_{\tilde{\vec{\varphi}}\vec{\varphi}}
-\bar{\vec{K}}_{\vec{\varphi}\mathfrak{q}}\vec{K}_{\mathfrak{q}\mathfrak{q}}^{-1}\vec{K}_{\mathfrak{q}\vec{\varphi}}$. 

The system is now fully condensed and only the matrix degree of freedom remain along with the constraints in the second line of \eqref{eq:newton5}, which cannot be further condensed. However, a penalty or an augmented Lagrangian technique can be applied if necessary. Note that the manipulations in this Section are pure algebraic and do not alter the solution, but enhance the efficiency, as we can now gradually solve the system. To be specific, after solving \eqref{eq:newton5}, the equations \eqref{eq:reduction4}, \eqref{eq:reduction3}, \eqref{eq:reduction2} and \eqref{eq:reduction1} can be solved.

\rev{We can note that $\mu_n$ is kind of pressure, so maybe some analogies with Stokes are possible.}

\begin{remark}
The manipulations in this Section can be reconsidered as a multi-step discrete null-space reduction scheme. We refer to \cite{hesch2014b}, Section 5.1 for details on the reformulation of the reduction in terms of discrete null-space matrices.
\end{remark}

\rev{ Multi-step discrete null-space reduction scheme ? Is it the same that just the Schur complement ?}



\begin{comment}

\paragraph{Discrete reduction scheme}
From $\eqref{eq:beamDis}_1$, we obtain a system of equations in the form 
\begin{equation}
\bar{\vec{\mu}}_A \tilde{R}^A(\tilde{\vec{x}}_i) = -\frac{1}{|C(\tilde{\vec{x}}_i)|}\left( \mathfrak{n}_A \tilde{R}^A_{,s}(\tilde{\vec{x}}_i)+
    \bar{\tilde{\vec{n}}}(\tilde{\vec{x}}_i)\right), \quad i=1,\dots, \mathfrak{O},
\end{equation}
which can be expressed more compact as $\vec{M}_{\bar{\mu}} \vec{S} = -(\vec{M}_\mathfrak{n}\vec{S}'+\vec{M}_{\bar{\tilde{n}}})\vec{D}_C$, 
where
\begin{equation}
\begin{aligned}
\vec{M}_{\bar{\mu}} &= [\bar{\vec{\mu}}_1,\dots,\bar{\vec{\mu}}_\mathfrak{O}]\in \mathbb{R}^{3\times \mathfrak{O}},                                      && 
    \vec{S} = \left[\tilde{R}^A(\tilde{\vec{x}}_i) \right]_{1\leq A,i\leq\mathfrak{O}} 
    \in\mathbb{R}^{\mathfrak{O}\times\mathfrak{O}},                                                                                              \\
\vec{M}_\mathfrak{n} &= [\vec{\mathfrak{n}}_1,\dots,\vec{\mathfrak{n}}_\mathfrak{O}]\in \mathbb{R}^{3\times \mathfrak{O}},                       &&
    \vec{S}' = \left[\tilde{R}_{,s}^A(\tilde{\vec{x}}_i) \right]_{1\leq A,i\leq \mathfrak{O}} 
    \in\mathbb{R}^{\mathfrak{O}\times\mathfrak{O}},                                                                                              \\
    \vec{M}_{\bar{\tilde{n}}} &= \left[\bar{\tilde{\vec{n}}}(\tilde{\vec{x}}_1),\dots,\bar{\tilde{\vec{n}}}(\tilde{\vec{x}}_\mathfrak{O})\right] 
    \in \mathbb{R}^{3\times \mathfrak{O}},                                                                                                       &&
    \vec{D}_C = \op{Diag}\left[|C(\tilde{\vec{x}}_i)|^{-1}\right]_{i=1,\dots,\mathfrak{O}}\in\mathbb{R}^{\mathfrak{O}\times\mathfrak{O}}.
\end{aligned}
\end{equation}
Assuming that the matrix $\vec{S}$ is invertible (\textcolor{red}{how should the collocation-points be selected to ensure that?!}), we can 
now express the nodes of the discrete Lagrange multiplier $\bar{\vec{\mu}}^\mathrm{h}$ in terms of $\vec{\mathfrak{n}}_A$ via 
$\vec{M}_{\bar{\mu}} = -(\vec{M}_\mathfrak{n}\vec{S}'+\vec{M}_{\bar{\tilde{n}}})\vec{D}_C\vec{S}^{-1}$. Moreover, introducing 
additionally the matrices
\begin{equation}
...
\end{equation} 
the system of equations obtained by $\eqref{eq:beamDis}_2$ can analogously rewritten as $...$ such that the nodes of $\vec{\mu}_\tau^\mathrm{h}$ 
are given by $...$. Thus, $\bar{\vec{\mu}}_A$, $\vec{\mu}_A^{\tau}$ can be eliminated in \eqref{eq:pdvADis2} and we obtain
\begin{equation}
\begin{aligned}
&\int\limits_{\Omega_0}\vec{P}\nabla_{\vec{X}}(R^A)\,\text{d}V - \int\limits_{\Omega_0}R^A\vec{B}_{ext}\,\text{d}V -
\int\limits_{\Gamma^{\sigma}}R^A\vec{T}_{ext}\,\text{d}A +\\
&\int\limits_{\mathfrak{C}_0}\left[-R^A (\vec{M}_\mathfrak{n}\vec{S}'+\vec{M}_{\bar{\tilde{n}}})\vec{D}_C\vec{S}^{-1}\tilde{\vec{\mathcal{R}}}+ 
\frac{1}{2}\,\left(\vec{\mu}_{\tau}\times\vec{d}_{\alpha}\otimes\vec{D}_{\alpha}+\mu_n\vec{d}_{\alpha}\otimes\vec{D}_{\alpha}\right) \nabla_{\vec{X}}(R^A)\right]
\hspace{-0.5mm}\abs{C}\d s = \vec{0},
\end{aligned}
\end{equation}
where $\tilde{\vec{\mathcal{R}}}:=[\tilde{R}^1,\dots,\tilde{R}^\mathfrak{O}]^\mathrm{T}\colon \mathfrak{C}_0\to \mathbb{R}^{\mathfrak{O}}$ and
we have to take the endpoint conditions at $s = 0,\,L$ into account as well. 


However, it is more convenient to condense first and 
discretise the reduced form \eqref{eq:sys:matrix_condense}, such that
\begin{equation}\label{eq:pdvADis4}
\begin{aligned}
&\int\limits_{\Omega_0}\vec{P}\nabla_{\vec{X}}(R^A)\,\text{d}V - \int\limits_{\Omega_0}R^A\vec{B}_{ext}\,\text{d}V -
\int\limits_{\Gamma^{\sigma}}R^A\vec{T}_{ext}\,\text{d}A +\\
&\int\limits_{\mathfrak{C}_0}\left[\left(\tilde{R}^A\mathfrak{n}_A\otimes\vec{D}_3\right)\nabla(R^A) - R^A\bar{\tilde{\vec{n}}} + 
\frac{1}{2}\,\left(\vec{\mu}_{\tau}\times\vec{d}_{\alpha}\otimes\vec{D}_{\alpha}+\mu_n\vec{d}_{\alpha}\otimes\vec{D}_{\alpha}\right) \nabla_{\vec{X}}(R^A)\right]\abs{C}\d s = \vec{0}.
\end{aligned}
\end{equation}

\end{comment}

==> sections/sec_discretization2.tex <==
Concerning the spatial approximation, suitable isogeometric discretization schemes are employed for the different fields. In particular, a standard IGA approach is applied to the matrix material, whereas a collocation type method is used to discretize the weighted residual. 

%For the coupling condition, the Lagrange multipliers are defined on the beam, which allows for a local condensation procedure of the position constraints.

\paragraph{Matrix material.}
A standard displacement-based finite element approach employs approximations of the deformation field $\vec{\varphi}$ and its variation of the form
\begin{equation}\label{eq:approxGeo}
\vec{\varphi}^{\mathrm{h}}=\sum\limits_{A\in\mathcal{I}}R^{A}\,\vec{q}_{A} \quad\text{and}\quad\delta\vec{\varphi}^{\mathrm{h}} =\sum\limits_{A\in\mathcal{I}}R^{A}\,\delta\vec{q}_{A},  
\end{equation}
respectively, where $\vec{q}_{A}\in\mathbb{R}^3$ and $\delta\vec{q}_{A}\in\mathbb{R}^3$. Here, \(R^A:\mathcal{B}_0^{\mathrm{h}}\rightarrow\mathbb{R}\) are NURBS based shape functions associated with control points \(A\in\mathcal{I}=\{1,\,\hdots,\,\mathfrak{M}\}\), where \(\mathfrak{M}\) denote the overall number of control points. The discrete form of \eqref{eq:pdvA} reads now
\begin{equation}\label{eq:pdvADis}
\delta\vec{q}_A\cdot\left(\,\int\limits_{\Omega_0}\vec{P}^{\mathrm{h}}\,\nabla R^A\d V - \int\limits_{\Omega_0}R^A\,\vec{B}^{\mathrm{h}}_{ext}\d V -
\int\limits_{\Gamma^{\sigma}}R^A\,\vec{T}^{\mathrm{h}}_{ext}\,\text{d}A \right)= 0,\quad\forall\,\delta\vec{q}_A,
\end{equation}
where $\vec{P}^{\mathrm{h}}$, $\vec{B}^{\mathrm{h}}_{ext}$ and $\vec{T}^{\mathrm{h}}_{ext}$ are the appropriately approximated Piola-Kirchhoff stress and the external contributions.

\paragraph{Beams.}
For the beam, we require in a first step the approximations of the centerline and the rotations. As all three parameter formulations involve the risk of singularities, we use quaternions $\mathfrak{q}$, c.f. Appendix \ref{app:quarternions}. The approximation along the centerline is given by
\begin{equation}
\tilde{\vec{\varphi}}^{\mathrm{h}}=\sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\,\tilde{\vec{q}}_{A} \quad\text{and}\quad\mathfrak{q}^{\mathrm{h}}=\sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\,\mathfrak{q}_{A}.
\end{equation}
Here, $\tilde{R}^{A}:\mathfrak{C}_0^{\mathrm{h}}\rightarrow\mathbb{R}$ are one-dimensional, NURBS based shape functions with associated control points $A\in\mathcal{J} = \{1,\hdots,\mathfrak{O}\}$. For the mixed formulation as introduced before, additional approximations are required for the resultants
\begin{equation}
\mathfrak{n}^{\mathrm{h}}=\sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\,\mathfrak{n}_{A}\quad\text{and}\quad\mathfrak{m}^{\mathrm{h}}=\sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\,\mathfrak{m}_{A}.
\end{equation}
The test functions $\delta\tilde{\vec{\varphi}}^{\mathrm{h}}$ and $\delta\vec{\phi}^{\mathrm{h}}$ and in the context of the applied mixed method, $\delta\mathfrak{g}^{\mathrm{h}}$ and $\delta\mathfrak{k}^{\mathrm{h}}$ are discretized via a set of Dirac functions $\delta_{\mathfrak{C}_0^{\mathrm{h}}}$. Therefore, we introduce the set of  collocation points $\{\tau_i\},\,i=1,\hdots,n$ in terms of the Greville abscissae of the parametrisation $\tau$ of the spline knot vector of the one-dimensional shape functions $\tilde{R}^{A}$, see e.g. \cite{Weeger2017} . Thus, we obtain
\begin{equation}
\delta\tilde{\vec{\varphi}}^{\mathrm{h}} = \sum\limits_{i\in\mathcal{J}} \delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tau-\tau_i)\,\delta\tilde{\vec{q}}_i\quad,\quad
\delta\vec{\phi}^{\mathrm{h}} = \sum\limits_{i\in\mathcal{J}} \delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tau-\tau_i)\,\delta\vec{\phi}_i,
\end{equation}
and
\begin{equation}
\delta\mathfrak{g}^{\mathrm{h}} = \sum\limits_{i\in\mathcal{J}} \delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tau-\tau_i)\,\delta\mathfrak{g}_i\quad,\quad
\delta\mathfrak{k}^{\mathrm{h}} = \sum\limits_{i\in\mathcal{J}} \delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tau-\tau_i)\,\delta\mathfrak{k}_i.
\end{equation}
The discrete principle of virtual work for the beam contributions as given in \eqref{eq:pdvaHW2} reads
\begin{equation}
\begin{aligned}
-&\delta\tilde{\vec{q}}_i\cdot\left(\left[\mathfrak{n}^{\mathrm{h}}(\tau_i)\right]^{\prime} + \bar{\tilde{\vec{n}}}(\tau_i)\right)
-\delta{\vec{\phi}}_i\cdot\left(\left[\mathfrak{m}^{\mathrm{h}}(\tau_i)\right]^{\prime} + \left[\tilde{\vec{\varphi}}^{\mathrm{h}}(\tau_i)\right]^{\prime}\times\mathfrak{n}^{\mathrm{h}}(\tau_i) + \bar{\tilde{\vec{m}}}(\tau_i)\right) +\\
&\delta\mathfrak{g}_i\cdot\left( \tilde{\vec{R}}(\tau_i)\,\frac{\partial\tilde{\Psi}}{\partial\vec{\Gamma}}\left(\vec{\Gamma}(\tau_i),\vec{K}(\tau_i)\right)-\mathfrak{n}^{\mathrm{h}}(\tau_i) \right)+\\
&\delta\mathfrak{k}_i\cdot\left( \tilde{\vec{R}}(\tau_i)\,\frac{\partial\tilde{\Psi}}{\partial\vec{K}}\left(\vec{\Gamma}(\tau_i),\vec{K}(\tau_i)\right)-\mathfrak{m}^{\mathrm{h}}(\tau_i) \right) = 0\quad\forall\, \delta\tilde{\vec{q}}_i,\delta{\vec{\phi}}_i,\delta\mathfrak{g}_i,\delta\mathfrak{k}_i.
\end{aligned}
\end{equation}
If quaternions are used, the additional constraint $\mathfrak{q}^{\mathrm{h}}(\tau_i)\cdot\mathfrak{q}^{\mathrm{h}}(\tau_i) - 1 = 0$ is enforced at every collocation point to ensure that the rotation matrix $\tilde{\vec{R}}(\tau_i)$ is orthonormal. Here and in the following, we make use of $(\bullet)(\tau_i)$ for the corresponding value evaluated at the collocation point $\tau_i$ e.g.\ we can write $\tilde{\vec{R}}(\tau_i) := \tilde{\vec{R}}(\mathfrak{q}(\tau_i))$ if quaternions are used.

\paragraph{Coupling conditions.}
Next, we introduce suitable approximations for the Lagrange multipliers related to the coupling conditions presented in the first term of \eqref{eq:VirtWork_coupling} as
\begin{equation}
\bar{\vec{\mu}}^{\mathrm{h}} = \sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\,\bar{\vec{\mu}}_{A},\quad  \delta\bar{\vec{\mu}}^{\mathrm{h}} = \sum\limits_{i\in\mathcal{J}} \delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tau-\tau_i)\,\delta\bar{\vec{\mu}}_i,
\end{equation}
along with the 6 Lagrange multipliers in the second term
\begin{equation}
\vec{\Sigma}^{\mathrm{h}} = \sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\,\vec{\Sigma}_{A},\quad \delta\vec{\Sigma}^{\mathrm{h}} = \sum\limits_{i\in\mathcal{J}} \delta_{\mathfrak{C}_0^{\mathrm{h}}}(\tau-\tau_i)\,\delta\vec{\Sigma}_i,
\end{equation}
following the discretization of the beam, along which we define the Lagrange multipliers. With regard to \eqref{eq:VirtWork_coupling}, we obtain
\begin{equation}\label{eq:VirtWork_coupling_discrete}
\begin{aligned}
\delta\Pi_C
=\,& \delta\bar{\vec{\mu}}_i\cdot(\vec{\varphi}^{\mathrm{h}}_{i} -\tilde{\vec{\varphi}}^{\mathrm{h}}(\tau_i))\abs{C_i} - 
\delta\tilde{\vec{q}}_i\cdot\bar{\vec{\mu}}^{\mathrm{h}}(\tau_i)\abs{C_i} +
\delta\vec{q}_A\cdot\int\limits_{\mathfrak{C}_0}\hspace{-1mm}\left[R^A\,\bar{\vec{\mu}}^{\mathrm{h}} + \frac{1}{2}\,\ten{\Sigma}^{\mathrm{h}}\,\ten{P}_{12}\,\nabla R^A\right] \abs{C}\d s \\
&-\frac{1}{2}\left(\left[\delta\vec{\phi}_i\right]_\times\fib{\vec{R}}(\tau_i)\,\ten{P}_{12}(\tau_i)\right):\ten{\Sigma}^{\mathrm{h}}(\tau_i)\abs{C_i} +
\frac{1}{2}\left[\big(\vec{F}_{c}(\tau_i)-\fib{\vec{R}}(\tau_i)\big)\,\ten{P}_{12}(\tau_i)\right]:\delta\ten{\Sigma}_i\abs{C_i}\,.
\end{aligned}
\end{equation}
Moreover, $\vec{\varphi}^{\mathrm{h}}_{i} = \sum\limits_{A\in\mathcal{I}}R^{A}(\vec{\xi}_{i})\,\vec{q}_{A}$ are the corresponding positions in the matrix material and the circumference $\abs{C_i}=\abs{C(\tau_i)}$. Eventually, we have to assemble the endpoint contributions emanating from \eqref{eq:VirtWork_endpoints}. In particular, we evaluate \eqref{eq:VirtWork_endpoints} at the first and last Greville point and assemble the corresponding contributions into the total system, as will be shown next.

\paragraph{Discrete system.}
The discretised condensed system as proposed in \eqref{eq:condensedCompact} reads
\begin{equation}\label{eq:red2}
\begin{aligned}
\int\limits_{\Omega_0}\vec{P}^{\mathrm{h}}\,\nabla R^A\,\text{d}V - &\int\limits_{\Omega_0}R^A\,\vec{B}^{\mathrm{h}}_{ext}\,\text{d}V -
\int\limits_{\Gamma^{\sigma}}R^A\,\vec{T}^{\mathrm{h}}_{ext}\,\text{d}A +\\
&\int\limits_{\mathfrak{C}_0}\mathfrak{P}^{\mathrm{h}}\,:\,\nabla^2R^A + (\vec{P}^{\mathfrak{n},{\mathrm{h}}}+\vec{P}^{\mathfrak{m},{\mathrm{h}}})\,\nabla R^A - 
R^A\,\bar{\tilde{\vec{n}}}^{\mathrm{h}} \d s = \vec{0},
\end{aligned}
\end{equation}
evaluated at every node $A$. Additionally, at every collocation point $\tau_i$ we solve
\begin{equation}\label{eq:beamDis2}
\begin{aligned}
\vec{0} &= \tilde{\vec{R}}(\tau_i)\,\frac{\partial\tilde{\Psi}}{\partial\vec{\Gamma}}\left(\vec{\Gamma}(\tau_i),\vec{K}(\tau_i)\right)-\mathfrak{n}^{\mathrm{h}}(\tau_i),\\
\vec{0} &=  \tilde{\vec{R}}(\tau_i)\,\frac{\partial\tilde{\Psi}}{\partial\vec{K}}\left(\vec{\Gamma}(\tau_i),\vec{K}(\tau_i)\right)-\mathfrak{m}^{\mathrm{h}}(\tau_i) ,\\
0 &= \mathfrak{q}^{\mathrm{h}}(\tau_i)\cdot\mathfrak{q}^{\mathrm{h}}(\tau_i) - 1\\
\end{aligned}
\end{equation}
along with the discrete constraints
\begin{equation}\label{eq:disc:constraints}
\begin{aligned}
\vec{0} &= \left(\vec{\varphi}^{\mathrm{h}}_{i} - \tilde{\vec{\varphi}}^{\mathrm{h}}(\tau_i)\right)\abs{C_i},\\
\vec{0} &= \frac{1}{2}\,\big(\vec{F}_{c}(\tau_i)\,\vec{D}_1-\vec{d}_1(\tau_i)\big)\abs{C_i},\\
\vec{0} &= \frac{1}{2}\,\big(\vec{F}_{c}(\tau_i)\,\vec{D}_2-\vec{d}_2(\tau_i)\big)\abs{C_i},
\end{aligned}
\end{equation}
Note that the discrete values of $\mathfrak{P}^{\mathrm{h}}$, $\vec{P}^{\mathfrak{n},{\mathrm{h}}}$ and $\vec{P}^{\mathfrak{m},{\mathrm{h}}}$, follows in a straightforward manner from \eqref{eq:new:sys:matrix_very_condense}, where we have made use of $\mathfrak{p}^{\mathrm{h}} = \sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\,\mathfrak{p}_{A}$.



\begin{comment}

For the matrix material, we have to solve
\begin{equation}\label{eq:pdvADis2}
\begin{aligned}
\int\limits_{\Omega_0}\vec{P}^{\mathrm{h}}\,\nabla R^A\,\text{d}V - \int\limits_{\Omega_0}R^A\,\vec{B}^{\mathrm{h}}_{ext}\,\text{d}V -
\int\limits_{\Gamma^{\sigma}}R^A\,\vec{T}^{\mathrm{h}}_{ext}\,\text{d}A +&\\
\int\limits_{\mathfrak{C}_0}\left[R^A\,\bar{\vec{\mu}}^{\mathrm{h}} + \frac{1}{2}\,\ten{\Sigma}^{\mathrm{h}}\,\ten{P}_{12}\,\nabla R^A\right]\abs{C}\d s +
\sum_{i=1,n}\left[R^A\,\bar{\vec{\mu}}^{i^\mathrm{h}} + \frac{1}{2}\,\vec{\Sigma}^{i^\mathrm{h}}\,\vec{P}^{12}\,\nabla R^A\right]\,\abs{A_i}
 &= \vec{0},
\end{aligned}
\end{equation}
for every node $A$ and for both Greville points $i = 1,\,n$. Additionally, at every collocation point $\tau_i$ we solve the balance and constitutive equations
\begin{equation}\label{eq:beamDis}
\begin{aligned}
\vec{0} &= \left[\mathfrak{n}^{\mathrm{h}}(\tau_i)\right]^{\prime} + \bar{\tilde{\vec{n}}}(\tau_i) + \bar{\vec{\mu}}^{\mathrm{h}}(\tau_i)\,\abs{C_i}, \\
\vec{0} &= \left[\mathfrak{m}^{\mathrm{h}}(\tau_i)\right]^{\prime} + \left[\tilde{\vec{\varphi}}^{\mathrm{h}}(\tau_i)\right]^{\prime}\times\mathfrak{n}^{\mathrm{h}}(\tau_i) + 
\bar{\tilde{\vec{m}}}(\tau_i) + \axl\left(\ten{\Sigma}^{\mathrm{h}}(\tau_i)\,\ten{P}_{12}(\tau_i)\,\fib{\vec{R}}\tp(\tau_i)\right)\abs{C_i},
\end{aligned}
\end{equation}
and
\begin{equation}\label{eq:beamDis2}
\begin{aligned}
\vec{0} &= \tilde{\vec{R}}(\tau_i)\,\frac{\partial\tilde{\Psi}}{\partial\vec{\Gamma}}\left(\vec{\Gamma}(\tau_i),\vec{K}(\tau_i)\right)-\mathfrak{n}^{\mathrm{h}}(\tau_i),\\
\vec{0} &=  \tilde{\vec{R}}(\tau_i)\,\frac{\partial\tilde{\Psi}}{\partial\vec{K}}\left(\vec{\Gamma}(\tau_i),\vec{K}(\tau_i)\right)-\mathfrak{m}^{\mathrm{h}}(\tau_i) ,\\
0 &= \mathfrak{q}^{\mathrm{h}}(\tau_i)\cdot\mathfrak{q}^{\mathrm{h}}(\tau_i) - 1\\
\end{aligned}
\end{equation}
along with
\begin{equation}\label{eq:disc:constraints}
\begin{aligned}
\vec{0} &= \left(\vec{\varphi}^{\mathrm{h}}_{i} - \tilde{\vec{\varphi}}^{\mathrm{h}}(\tau_i)\right)\abs{C_i},\\
\vec{0} &= \frac{1}{2}\,\big(\vec{F}_{c}(\tau_i)\,\vec{D}_1-\vec{d}_1(\tau_i)\big)\abs{C_i},\\
\vec{0} &= \frac{1}{2}\,\big(\vec{F}_{c}(\tau_i)\,\vec{D}_2-\vec{d}_2(\tau_i)\big)\abs{C_i},
\end{aligned}
\end{equation}
excluding the endpoints on the line, which we take into account via
\begin{equation}\label{eq:disc:constraints2}
\begin{aligned}
\vec{0} &= \frac{1}{2}\,\big(\vec{F}_{c}(\tau_s)\,\vec{D}_1-\vec{d}_1(\tau_s)\big)\abs{A_s},\\
\vec{0} &= \frac{1}{2}\,\big(\vec{F}_{c}(\tau_s)\,\vec{D}_2-\vec{d}_2(\tau_s)\big)\abs{A_s},
\end{aligned}
\end{equation}
where $s$ denotes the first and last Greville point.

%\rev{Factor $\abs{C}$ can be omitted by scaling both sides. }

\paragraph{Reduced system.}
The condensed system as presented in \eqref{eq:condensedCompact} reads 
\begin{equation}\label{eq:red2}
\begin{aligned}
\int\limits_{\Omega_0}\vec{P}^{\mathrm{h}}\,\nabla R^A\,\text{d}V - &\int\limits_{\Omega_0}R^A\,\vec{B}^{\mathrm{h}}_{ext}\,\text{d}V -
\int\limits_{\Gamma^{\sigma}}R^A\,\vec{T}^{\mathrm{h}}_{ext}\,\text{d}A +\\
&\int\limits_{\mathfrak{C}_0}\mathfrak{P}^{\mathrm{h}}\,:\,\nabla^2R^A + (\vec{P}^{\mathfrak{n},{\mathrm{h}}}+\vec{P}^{\mathfrak{m},{\mathrm{h}}})\,\nabla R^A - 
R^A\,\bar{\tilde{\vec{n}}}^{\mathrm{h}} \d s = \vec{0},
\end{aligned}
\end{equation}
evaluated at every node $A$. Additionally, we enforce at every Greville point \eqref{eq:beamDis2} supplemented by \eqref{eq:disc:constraints}. Note that the discrete values of $\mathfrak{P}^{\mathrm{h}}$, $\vec{P}^{\mathfrak{n},{\mathrm{h}}}$ and $\vec{P}^{\mathfrak{m},{\mathrm{h}}}$, follows in a straightforward manner from \eqref{eq:new:sys:matrix_very_condense}, where $\mathfrak{p}^{\mathrm{h}} = \sum\limits_{A\in\mathcal{J}}\tilde{R}^{A}\,\mathfrak{p}_{A}$ has to be taken into account and at the endpoint constraints we substitute $\mathfrak{n} = \abs{A_s}\,\bar{\vec{\mu}}^s$ and $\mathfrak{m} = \abs{A_s}\,\tilde{\vec{\mu}}_\tau^s$, supplemented by \eqref{eq:disc:constraints2}.

\end{comment}


\paragraph{Discrete reduction scheme.}
Within the Newton-Raphson iteration, we have to solve at every step
\begin{equation}\label{eq:newton}
\begin{bmatrix}
\vec{K}_{\vec{\varphi}\vec{\varphi}} & \vec{K}_{\vec{\varphi}\tilde{\vec{\varphi}}} & 
\vec{K}_{\vec{\varphi}\mathfrak{n}} & \vec{K}_{\vec{\varphi}\mathfrak{m}} & 
\vec{K}_{\vec{\varphi}\mathfrak{q}} & \vec{K}_{\vec{\varphi}\mathfrak{p}} \\
\vec{K}_{\tilde{\vec{\varphi}}\vec{\varphi}} & -\ten{I}_{\tilde{\vec{\varphi}}\tilde{\vec{\varphi}}} & \vec{0} & \vec{0} & \vec{0} & \vec{0} \\
\vec{0} & \vec{K}_{\mathfrak{n}\tilde{\vec{\varphi}}} &
\ten{I}_{\mathfrak{n}\mathfrak{n}} & \vec{0} & \vec{K}_{\mathfrak{n}\mathfrak{q}} & \vec{0} \\
\vec{0} & \vec{0} & \vec{0} & \ten{I}_{\mathfrak{m}\mathfrak{m}} & \vec{K}_{\mathfrak{m}\mathfrak{q}} & \vec{0} \\
\vec{K}_{\mathfrak{q}\vec{\varphi}} & \vec{0} & \vec{0} & \vec{0} & \vec{K}_{\mathfrak{q}\mathfrak{q}} & \vec{0}\\
\vec{K}_{\mathfrak{p}\vec{\varphi}} & \vec{0} & \vec{0} & \vec{0} & \vec{K}_{\mathfrak{p}\mathfrak{q}} & \vec{0}
\end{bmatrix}
\begin{bmatrix}
\Delta\vec{\varphi}\\
\Delta\tilde{\vec{\varphi}}\\
\Delta\mathfrak{n}\\
\Delta\mathfrak{m}\\
\Delta\mathfrak{q}\\
\Delta\mathfrak{p}
\end{bmatrix} =
\begin{bmatrix}
\vec{R}_{\vec{\varphi}}\\
\vec{R}_{\tilde{\vec{\varphi}}}\\
\vec{R}_{\mathfrak{n}}\\
\vec{R}_{\mathfrak{m}}\\
\vec{R}_{\mathfrak{q}}\\
\vec{R}_{\mathfrak{p}}
\end{bmatrix},
\end{equation}
where we have made use of \eqref{eq:simpleMat}. Here, $\vec{R}_{\vec{\varphi}}$ correlates to \eqref{eq:red2}, $\vec{R}_{\tilde{\vec{\varphi}}}$ to \eqref{eq:disc:constraints}$_1$, $\vec{R}_{\mathfrak{n}}$ to \eqref{eq:beamDis2}$_1$, $\vec{R}_{\mathfrak{m}}$ to \eqref{eq:beamDis2}$_2$, $\vec{R}_{\mathfrak{q}}$ and $\vec{R}_{\mathfrak{p}}$ to \eqref{eq:beamDis2}$_3$ and \eqref{eq:disc:constraints}$_2$. Note that $\vec{R}_{\mathfrak{q}}$ and $\vec{R}_{\mathfrak{p}}$ consists of seven equations per beam node (i.e. Greville point), as \eqref{eq:beamDis2}$_3$ is a scalar and \eqref{eq:disc:constraints}$_2$ and \eqref{eq:disc:constraints}$_3$ are in total six constraints. Note that we omit the endpoint constraints for the sake of a clear presentation. Next, we solve the second, third and fourth line in \eqref{eq:newton}
\begin{equation}\label{eq:reduction1}
\Delta\tilde{\vec{\varphi}} = \vec{K}_{\tilde{\vec{\varphi}}\vec{\varphi}}\,\Delta\vec{\varphi}-\vec{R}_{\tilde{\vec{\varphi}}},\quad
\Delta\mathfrak{n} = \vec{R}_{\mathfrak{n}}-\vec{K}_{\mathfrak{n}\tilde{\vec{\varphi}}}\,\Delta\tilde{\vec{\varphi}}-\vec{K}_{\mathfrak{n}\mathfrak{q}}\,\Delta\mathfrak{q},\quad
\Delta\mathfrak{m} = \vec{R}_{\mathfrak{m}}-\vec{K}_{\mathfrak{m}\mathfrak{q}}\,\Delta\mathfrak{q},
\end{equation}
and obtain
\begin{equation}\label{eq:newton3}
\begin{bmatrix}
\vec{K}_{\vec{\varphi}\vec{\varphi}}+\bar{\vec{K}}_{\vec{\varphi}\tilde{\vec{\varphi}}}\,\vec{K}_{\tilde{\vec{\varphi}}\vec{\varphi}} & 
\bar{\vec{K}}_{\vec{\varphi}\mathfrak{q}} & \vec{K}_{\vec{\varphi}\mathfrak{p}} \\
\vec{K}_{\mathfrak{q}\vec{\varphi}} & \vec{K}_{\mathfrak{q}\mathfrak{q}} & \vec{0} \\
\vec{K}_{\mathfrak{p}\vec{\varphi}} & \vec{K}_{\mathfrak{p}\mathfrak{q}} & \vec{0}
\end{bmatrix}
\begin{bmatrix}
\Delta\vec{\varphi}\\
\Delta\mathfrak{q}\\
\Delta\mathfrak{p}
\end{bmatrix} =
\begin{bmatrix}
\bar{\vec{R}}_{\vec{\varphi}}+\bar{\vec{K}}_{\vec{\varphi}\tilde{\vec{\varphi}}}\,\vec{R}_{\tilde{\vec{\varphi}}}\\
\vec{R}_{\mathfrak{q}}\\
\vec{R}_{\mathfrak{p}}
\end{bmatrix},
\end{equation}
where $\bar{\vec{K}}_{\vec{\varphi}\tilde{\vec{\varphi}}} = \vec{K}_{\vec{\varphi}\tilde{\vec{\varphi}}}-\vec{K}_{\vec{\varphi}\mathfrak{n}}\,\vec{K}_{\mathfrak{n}\tilde{\vec{\varphi}}} $, $\bar{\vec{K}}_{\vec{\varphi}\mathfrak{q}} = \vec{K}_{\vec{\varphi}\mathfrak{q}}-\vec{K}_{\vec{\varphi}\mathfrak{m}}\,\vec{K}_{\mathfrak{m}\mathfrak{q}} -\vec{K}_{\vec{\varphi}\mathfrak{n}}\,\vec{K}_{\mathfrak{n}\mathfrak{q}}$ and $\bar{\vec{R}}_{\vec{\varphi}} = \vec{R}_{\vec{\varphi}}-\vec{K}_{\vec{\varphi}\mathfrak{m}}\,\vec{R}_{\mathfrak{m}}-\vec{K}_{\vec{\varphi}\mathfrak{n}}\,\vec{R}_{\mathfrak{n}}$. 







==> sections/sec_impoved.tex <==


\section{Updated model}

Let us consider the coupling forces expansion~\eqref{eq:key3}, where instead of~\eqref{eq:key4}, the moments contribution~$\tilde{\vec{\mu}}$ is given by
\begin{equation}\label{eq:new:mu_tilde}
\tilde{\vec{\mu}}(\theta^{\alpha},s) = \ten{\Sigma}(s)\,\vec{N}(\theta^{\alpha}),
\end{equation}
where $\vec{N}=\vec{D}_1\,\cos\theta + \vec{D}_2\,\sin\theta$ is the unit outer normal to the interface in the reference configuration, and~$\ten{\Sigma}$ denotes the interface stress tensor.
Note that $\int_{C(s)}\ten{\Sigma}(s)\,\vec{N}(\theta^{\alpha})\d C = \ten{\Sigma}(s)\int_{C(s)}\,\vec{N}(\theta^{\alpha})\d C = 0$.
Besides, $\tilde{\vec{\mu}}$ has six degrees of freedom.
In particular, denoting $\ten{P}_{12} = \vec{D}_{\alpha}\otimes\vec{D}_{\alpha}$ and $\ten{\mathcal{D}}=\vec{D}_j\otimes\vec{e}_j$, we can write
\begin{equation}\label{eq:new:LM_matrix}
	\ten{\Sigma}\ten{P}_{12} =
	\fib{\vec{R}}\ten{\mathcal{D}}
	\begin{bmatrix}
		\tilde{\mu}_{n,1} + \tilde{\mu}_{n,2} & \tilde{\mu}_{n,3} - \tilde{\mu}_{\tau,3} & 0\\
		\tilde{\mu}_{n,3} + \tilde{\mu}_{\tau,3} & \tilde{\mu}_{n,1} - \tilde{\mu}_{n,2} & 0\\
		-2\tilde{\mu}_{\tau,2} &  2\tilde{\mu}_{\tau,1} & 0
	\end{bmatrix}
	\ten{\mathcal{D}}\tp,
\end{equation}
where $\tilde{\mu}_{n,1}$ is associated to the dilatation of the cross-section, $\tilde{\mu}_{n,2}$ and $\tilde{\mu}_{n,3}$ to the shear, $\tilde{\mu}_{\tau,1}$ and $\tilde{\mu}_{\tau,2}$ to the bending, and $\tilde{\mu}_{\tau,3}$ to the torsion.

\begin{remark}
	Our previous model turns out to be a particular case, where
	one assumes	no shear constraints, that is, $\tilde{\mu}_{n,1}=\tilde{\mu}_{n,2}=0$, or $\sym{\ten{P}_{12}\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}} = \mu_{n,1}\ten{P}_{12}$.
	%	~$\dev{\ten{\Sigma}}=0$.
\end{remark}

\begin{proposition}
	Let $\tilde{\vec{\mu}}_n = \tilde{\mu}_{n,j}\vec{d}_j$
	and $\tilde{\vec{\mu}}_\tau = \tilde{\mu}_{\tau,j}\vec{d}_j = \axl\left(\ten{\Sigma}\ten{P}_{12}\fib{\vec{R}}\tp\right)$.
	Note that it holds the following decomposition:
	\begin{equation}\label{eq:new:prop:decomposition}
	\frac{1}{2}\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}
	=
	\left(\ten{\Id}-\frac{1}{2}\ten{P}_{12}\right)\skew{\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}}\ten{P}_{12}
	+
	\frac{1}{2}\sym{\ten{P}_{12}\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}}.		
	\end{equation}
	Moreover, it can be written as
	\begin{equation}\label{key}
		\frac{1}{2}\ten{\Sigma}\ten{P}_{12} = \left(\ten{\mathcal{P}}_{\alpha}\tilde{\vec{\mu}}_\tau + \ten{\mathcal{Q}}_{\alpha}\tilde{\vec{\mu}}_n\right)\otimes\vec{D}_\alpha,
	\end{equation}
	where
	\begin{align}
		\ten{\mathcal{P}}_1 &= \left(\frac{1}{2}\vec{d}_2\otimes\vec{d}_3 - \vec{d}_3\otimes\vec{d}_2\right), &
		\ten{\mathcal{P}}_2 &= \left(-\frac{1}{2}\vec{d}_1\otimes\vec{d}_3 + \vec{d}_3\otimes\vec{d}_1\right), \\
		\ten{\mathcal{Q}}_1 &= \frac{1}{2}\left(\vec{d}_1\otimes\vec{d}_1 + \vec{d}_1\otimes\vec{d}_2 + \vec{d}_2\otimes\vec{d}_3\right), &
		\ten{\mathcal{Q}}_2 &= \frac{1}{2}\left(\vec{d}_2\otimes\vec{d}_1 - \vec{d}_2\otimes\vec{d}_2 + \vec{d}_1\otimes\vec{d}_3\right).
	\end{align}
\end{proposition}


%\begin{equation}\label{key}
%\begin{aligned}
%\left(\ten{\Id}-\frac{1}{2}\fib{\ten{R}}\ten{P}_{12}\fib{\ten{R}}\tp\right) & \VPTen{\vec{v}}\fib{\ten{R}}\ten{P}_{12} \\
%&=
%\left(\frac{1}{2}\fib{\ten{R}}\ten{P}_{12}\fib{\ten{R}}\tp + \vec{d}_3\otimes\vec{d}_3\right)\VPTen{\vec{d}_{\alpha}}\tp\vec{v}\otimes\vec{D}_{\alpha}
%\\
%&=
%\underbrace{\left(\frac{1}{2}\vec{d}_2\otimes\vec{d}_3 - \vec{d}_3\otimes\vec{d}_2\right)}_{\ten{\mathcal{P}}_1}\vec{v}\otimes\vec{D}_1
%+
%\underbrace{\left(-\frac{1}{2}\vec{d}_1\otimes\vec{d}_3 + \vec{d}_3\otimes\vec{d}_1\right)}_{\ten{\mathcal{P}}_2}\vec{v}\otimes\vec{D}_2
%\\
%&=
%(\vec{v}\cdot\vec{d}_1)\vec{d}_3\otimes\vec{D}_2  - (\vec{v}\cdot\vec{d}_2)\vec{d}_3\otimes\vec{D}_1 + (\vec{v}\cdot\vec{d}_3)\frac{\vec{d}_2\otimes\vec{D}_1-\vec{d}_1\otimes\vec{D}_2}{2}
%\end{aligned}
%\end{equation}
%Besides, according to~\eqref{eq:new:LM_matrix}, we have
%\begin{equation}\label{key}
%\begin{aligned}
%\fib{\ten{R}}\ten{P}_{12} & \sym{\fib{\vec{R}}\tp\ten{\Sigma}}\ten{P}_{12}
%\\
%&=
%\tilde{\mu}_n\left(\vec{d}_1\otimes\vec{D}_1+\vec{d}_2\otimes\vec{D}_2\right)
%+
%\tilde{\mu}_{s,1}\left(\vec{d}_1\otimes\vec{D}_1-\vec{d}_2\otimes\vec{D}_2\right)
%+
%\tilde{\mu}_{s,2}\left(\vec{d}_2\otimes\vec{D}_1+\vec{d}_1\otimes\vec{D}_2\right)
%\\
%&=
%\underbrace{\left(\vec{d}_1\otimes\vec{d}_1 + \vec{d}_1\otimes\vec{d}_2 + \vec{d}_2\otimes\vec{d}_3\right)}_{\ten{\mathcal{Q}}_1}\tilde{\vec{\mu}}^{sym}\otimes\vec{D}_1
%\\
%&+
%\underbrace{\left(\vec{d}_2\otimes\vec{d}_1 - \vec{d}_2\otimes\vec{d}_2 + \vec{d}_1\otimes\vec{d}_3\right)}_{\ten{\mathcal{Q}}_2}\tilde{\vec{\mu}}^{sym}\otimes\vec{D}_2,
%%&=
%%(\tilde{\vec{\mu}}^{sym}\cdot\vec{d}_1)\vec{d}_1\otimes\vec{D}_1
%%+
%%(\tilde{\vec{\mu}}^{sym}\cdot\vec{d}_2\vec{d}_2\otimes\vec{D}_2
%%+
%%(\tilde{\vec{\mu}}^{sym}\cdot\vec{d}_3)\frac{\vec{d}_2\otimes\vec{D}_1+\vec{d}_1\otimes\vec{D}_2}{2}
%%\\
%%&=
%%\underbrace{\left(\vec{d}_1\otimes\vec{d}_1 + \frac{1}{2}\vec{d}_2\otimes\vec{d}_3\right)}_{\ten{\mathcal{Q}}_1}\tilde{\vec{\mu}}^{sym}\otimes\vec{D}_1
%%+
%%\underbrace{\left(\vec{d}_2\otimes\vec{d}_2 + \frac{1}{2}\vec{d}_1\otimes\vec{d}_3\right)}_{\ten{\mathcal{Q}}_2}\tilde{\vec{\mu}}^{sym}\otimes\vec{D}_2,
%\end{aligned}
%\end{equation}

\begin{proof}	
	\begin{equation}\label{key}
	\begin{aligned}
	\left(\ten{\Id}-\frac{1}{2}\ten{P}_{12}\right)\skew{\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}}\ten{P}_{12}
	&=
	\frac{1}{2}\left(\ten{\Id}-\frac{1}{2}\ten{P}_{12}\right)\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}
	-
	\frac{1}{4}\ten{P}_{12}\ten{\Sigma}\tp\fib{\vec{R}}\ten{P}_{12} \\
	&=
	\frac{1}{2}\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}
	-
	\frac{1}{2}\sym{\ten{P}_{12}\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}}.
	\end{aligned}	
	\end{equation}	
\end{proof}

%In particular, it can be decomposed on a spherical part, deviatoric and skew-symmetric parts:
%\begin{equation}\label{key}
%	\ten{\Sigma} = \mu_n\ten{\Id} + \dev{\ten{\Sigma}} + \left[\vec{\mu}_\tau\right]_\times,
%\end{equation}
%where
%\begin{align}\label{key}
%	 \mu_n &= \frac{1}{3}\tr\ten{\Sigma},\\
%	 \dev{\ten{\Sigma}} &= \frac{1}{2}\left(\ten{\Sigma}+\ten{\Sigma}\tp\right)- \mu_n\ten{\Id},\\
%	 \vec{\mu}_\tau &= \axl\ten{\Sigma}.
%\end{align}



With~\eqref{eq:new:mu_tilde}, equation~\eqref{eq:const} rewrites as
\begin{equation}\label{eq:new:Pi_C}
\Pi_{C} = \int\limits_{\mathfrak{C}_0}\left[\bar{\vec{\mu}}\cdot(\vec{x}_{c} -\tilde{\vec{\varphi}})\abs{C} + 
\int\limits_{C(s)} \ten{\Sigma}\,\vec{N}\cdot\big(\vec{F}_{c}-\fib{\vec{R}}\big)\,\vec{N}\,r \d C\right]\d s.
\end{equation}
According to~\eqref{eq:axial_int}, for the second term in~\eqref{eq:new:Pi_C}, it holds
\begin{equation}
\int\limits_{C(s)} \vec{N}\cdot\ten{\Sigma}\tp\big(\vec{F}_{c}-\fib{\vec{R}}\big)\,\vec{N}\ \d C
=
\pi\tr\left(\ten{\Sigma}\tp\big(\vec{F}_{c}-\fib{\vec{R}}\big)\ten{P}_{12}\right),
\end{equation}
which replaces~\eqref{eq:tan1}.
And thus, \eqref{eq:pdvApi3} is replaced with
\begin{equation}
\begin{aligned}
\delta\Pi_C^2
&=
\frac{1}{2}\int\limits_{\mathfrak{C}_0}\left[
\big(\nabla\delta\vec{\varphi}-\left[\delta\vec{\phi}\right]_\times\fib{\vec{R}}\big)\ten{P}_{12}:\ten{\Sigma}
+
\big(\vec{F}_{c}-\fib{\vec{R}}\big)\ten{P}_{12}:\delta\ten{\Sigma}
\right]\abs{C}\d s
\end{aligned}
\end{equation}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Total system.} Eventually, the total system reads:
\begin{equation}
\begin{aligned}
&\int\limits_{\mtx{\Omega}_0} \left[\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}} - \vec{B}_{ext}\cdot\delta\vec{\varphi}\right] \d V	-
\int\limits_{\partial\Omega_{N}} \!\!\vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d S
+\\
&
+
\int\limits_{\mathfrak{C}_0}\left(\vec{\bar{\mu}} \cdot \delta\vec{\mtx{\varphi}}
+
\frac{1}{2}\,\ten{\Sigma}\ten{P}_{12}:\nabla\delta\mtx{\vec{\varphi}} \right) \abs{C}\d s
+\\
&
+
\sum_{s=0,L}\abs{A}\left[\bar{\vec{\mu}}^s\cdot\delta\mtx{\vec{\varphi}}_s
+
\frac{1}{2}\,\ten{\Sigma}^s\ten{P}_{12}: \nabla\delta\mtx{\vec{\varphi}}_s\right] 
= 0.
\end{aligned}
\end{equation}
%Note that the component~$\ten{\Sigma}\vec{d}_3$ does not enter in the matrix equation. 
The beam contributions  yield
\begin{align}
&\int\limits_{\mathfrak{C}_0}\left(
{\mathfrak{n}}^{\prime} + \bar{\tilde{\vec{n}}}
+
\vec{\bar{\mu}}\abs{C}\right)\cdot\delta\vec{\fib{\varphi}}\d s = 0,  
\label{eq:new:sys:loads2}
\\	
&\int\limits_{\mathfrak{C}_0}\biggl({\mathfrak{m}}^{\prime} + \tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}}
+
\bar{\tilde{\vec{m}}}
+
\underbrace{\axl\left(\ten{\Sigma}\ten{P}_{12}\fib{\vec{R}}\tp\right)}_{\tilde{\vec{\mu}}_\tau}\abs{C}\biggr)\cdot\delta\vec{\phi} \d s = 0,
\label{eq:new:sys:moments2}
\end{align}
supplemented by the constitutive equations
\begin{align}
&\int\limits_{\mathfrak{C}_0}\delta{\mathfrak{g}}\cdot\left({\mathfrak{n}} - \fib{\ten{R}}\frac{\partial\tilde{\Psi}(\vec{\Gamma},\vec{K})}{\partial\vec{\Gamma}}\right)\d s = 0,
\label{eq:new:constitutive_n}
\\
&\int\limits_{\mathfrak{C}_0}\delta{\mathfrak{k}}\cdot\left({\mathfrak{m}} - \fib{\ten{R}}\frac{\partial\tilde{\Psi}(\vec{\Gamma},\vec{K})}{\partial\vec{K}}\right)\,\text{d}s = 0,
\label{eq:new:constitutive_m}
\end{align}
the coupling constraints
\begin{align}
&\int\limits_{\mathfrak{C}_0}\delta\vec{\bar{\mu}} \cdot\left(\fib{\vec{\varphi}}-\vec{\mtx{\varphi}}\right)\d s = 0,	
%\label{eq:sys:pi1}
\\
&\int\limits_{\mathfrak{C}_0}
\big(\vec{F}_{c}-\fib{\vec{R}}\big)\ten{P}_{12}:\delta\ten{\Sigma}\d s = 0. \qquad (6\text{ equations})
\label{eq:new:sys:pi3}
\end{align}
and the beam endpoints conditions at $s=0,L$:
\begin{align}
&\mathfrak{n} = \abs{A}\,\bar{\vec{\mu}}^s,
%\label{eq:sys:bc_n}
\\
&\mathfrak{m} = \abs{A}\,\underbrace{\axl\left(\ten{\Sigma}^s\ten{P}_{12}\fib{\vec{R}}\tp\right)}_{\tilde{\vec{\mu}}_\tau^s}.
%\label{eq:sys:bc_m}
%\\
%&\fib{\vec{\varphi}} = \vec{\mtx{\varphi}},	
%%\label{eq:bc1}
%\\
%&\vec{F}_{c}\vec{D}_{\alpha}=\vec{d}_{\alpha}.
%%\label{eq:bc2}
\end{align}

%\begin{remark}
%	Note that in~\eqref{eq:new:sys:moments2}, the spherical part of~$\fib{\vec{R}}\tp\ten{\Sigma}$, $\mu_n\ten{\Id}$, yields zero term, since $\axl\left(\fib{\vec{R}}\ten{P}_{12}\fib{\vec{R}}\tp\right)=0$.
%	That is, pressure produces no moments.
%\end{remark}

\begin{remark}
	Note that the component~$\ten{\Sigma}\vec{D}_3$ does not enter in the system at all, and that $\delta\ten{\Sigma}\,\ten{P}_{12}$, has only $6$ degrees of freedom: three for bending and torsion of the cross-section, one for dilatation and two more for the shear (directions $\vec{D}_{\alpha}$).
	
%	Moreover, for $\delta\ten{\Sigma} = \VPTen{\delta\vec{\mu}_\tau}$ and $\delta\ten{\Sigma} = \delta\mu_n\,\ten{\Id}$, \eqref{eq:new:sys:pi3} respectively reproduces~\eqref{eq:sys:pi2} and ~\eqref{eq:sys:pi3}:
%	\begin{align}\label{key}
%	\int\limits_{\mathfrak{C}_0}
%	\skew{\vec{F}_{c}\ten{P}_{12}\fib{\vec{R}}\tp}:\VPTen{\delta\vec{\mu}_\tau}\d s &= 0,\\
%	\int\limits_{\mathfrak{C}_0}
%	\tr\left[\big(\vec{F}_{c}-\fib{\vec{R}}\big)\ten{P}_{12}\fib{\vec{R}}\tp\right]\delta\mu_n\d s &= 0,
%	\end{align}
%	and deviatoric part gives us two more equations:
%	\begin{align}\label{key}
%	\int\limits_{\mathfrak{C}_0}
%	\left(\vec{d}_{1}\cdot\vec{F}_{c}\vec{D}_{1} - \vec{d}_{2}\cdot\vec{F}_{c}\vec{D}_{2}\right) \,\delta\mu_{dev}^1\d s &= 0,\\	
%	\int\limits_{\mathfrak{C}_0}
%	\left(\vec{d}_{1}\cdot\vec{F}_{c}\vec{D}_{2} + \vec{d}_{2}\cdot\vec{F}_{c}\vec{D}_{1}\right) \,\delta\mu_{dev}^2\d s &= 0.
%	\end{align}
\end{remark}

\begin{remark}
	Note that \eqref{eq:new:sys:pi3} can simply be written down with 6 equations:
	\begin{align}\label{key}
	\int\limits_{\mathfrak{C}_0}
	\big(\vec{F}_{c}\vec{D}_{1}-\vec{d}_{1}\big)\cdot\delta\tilde{\vec{\mu}}_1\d s &= 0,\\
	\int\limits_{\mathfrak{C}_0}
	\big(\vec{F}_{c}\vec{D}_{2}-\vec{d}_{2}\big)\cdot\delta\tilde{\vec{\mu}}_2\d s &= 0.
	\end{align}
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\paragraph{Reduced system.} 
If $\delta\vec{\varphi}\big|_{\mathfrak{C}_0}$ is in $\HS_{\delta\fib{\vec{\varphi}}}(\mathfrak{C}_0)$, then we can condense \eqref{eq:sys:load2} and \eqref{eq:sys:bc_n} to the matrix equation~\eqref{eq:sys:matrix}, which leads after integration by parts to
\begin{equation}\label{eq:new:sys:matrix_condense}
\begin{aligned}
&\int\limits_{\mtx{\Omega}} \left(\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}}- \vec{B}_{ext}\cdot\delta\vec{\varphi}\right) \d V
-
\int\limits_{\partial\Omega_{N}} \!\!\vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d S
+
\int\limits_{\mathfrak{C}_0}\left(\mathfrak{n}\otimes\vec{D}_3 : \nabla\delta\mtx{\vec{\varphi}}
-
\bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}\right)\d s
\\&+
\frac{1}{2}\,\int\limits_{\mathfrak{C}_0}
\ten{\Sigma}\ten{P}_{12}:\nabla\delta\mtx{\vec{\varphi}} \abs{C}\d s
+
\frac{1}{2} \sum_{s=0,L}
\ten{\Sigma}^s\ten{P}_{12}: \nabla\delta\mtx{\vec{\varphi}}_s\,\abs{A}
= 0.
\end{aligned}
\end{equation}
Thus, we have eliminated the set of Lagrange multipliers $\bar{\vec{\mu}}$.
% using \eqref{eq:sys:load}.
To eliminate the Lagrange multipliers~$\ten{\Sigma}$, we have to assume that $\axl\left(\left(\ten{\Id}-\frac{1}{2}\fib{\vec{R}}\ten{P}_{12}\fib{\vec{R}}\tp\right)\nabla\delta\vec{\mtx{\varphi}}\,\ten{P}_{12}\fib{\vec{R}}\tp\right)\in \HS_{\delta\vec{\phi}}$ for all~$\delta\vec{\varphi}\in \HS_{\delta\vec{\varphi}}$.
Then, substituting $\delta\vec{\phi}=\axl\left(\left(\ten{\Id}-\frac{1}{2}\fib{\vec{R}}\ten{P}_{12}\fib{\vec{R}}\tp\right)\nabla\delta\vec{\mtx{\varphi}}\,\ten{P}_{12}\fib{\vec{R}}\tp\right)$ in~\eqref{eq:new:sys:moments2}, we obtain
\begin{multline}
\int\limits_{\mathfrak{C}_0}\ten{\mathcal{P}}_{\alpha}
\left({\mathfrak{m}}^{\prime} + \tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}}+\bar{\tilde{\vec{m}}}\right)
\otimes\vec{D}_{\alpha}
:
\nabla\delta\vec{\mtx{\varphi}}
\d s
+
\\
+
\int\limits_{\mathfrak{C}_0}
\biggl(\frac{1}{2}\ten{\Sigma}\ten{P}_{12}
-
\underbrace{\frac{1}{2}\fib{\vec{R}}\sym{\ten{P}_{12}\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}}}_{\ten{\mathcal{Q}}_{\alpha}\tilde{\vec{\mu}}_n^s\otimes\vec{D}_{\alpha}}\biggr)
:
\nabla\delta\vec{\mtx{\varphi}}
\abs{C}\d s = 0.
\end{multline}
%\begin{multline}
%\int\limits_{\mathfrak{C}_0}
%\fib{\ten{R}}\tp\left({\mathfrak{m}}^{\prime} + \tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}}+\bar{\tilde{\vec{m}}}\right)
%\cdot
%\axl\left(\left(\ten{\Id}-\frac{1}{2}\ten{P}_{12}\right)\fib{\vec{R}}\tp\nabla\delta\vec{\mtx{\varphi}}\,\ten{P}_{12}\right)
%\d s
%+
%\\
%+
%\int\limits_{\mathfrak{C}_0}
%\axl\left(\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}\right)\cdot\axl\left(\left(\ten{\Id}-\frac{1}{2}\ten{P}_{12}\right)\fib{\vec{R}}\tp\nabla\delta\vec{\mtx{\varphi}}\,\ten{P}_{12}\right)
%\abs{C}\d s = 0.
%\end{multline}
%Hence, applying~\eqref{eq:new:prop:decomposition}, we obtain
%\begin{multline}
%\frac{1}{2}\int\limits_{\mathfrak{C}_0}
%\left(\ten{\Id}-\frac{1}{2}\fib{\ten{R}}\ten{P}_{12}\fib{\ten{R}}\tp\right)\VPTen{{\mathfrak{m}}^{\prime} + \tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}}
%+
%\bar{\tilde{\vec{m}}}}
%\fib{\ten{R}}\ten{P}_{12}
%:
%\nabla\delta\vec{\mtx{\varphi}}
%\d s
%+
%\\
%+
%\frac{1}{2}\int\limits_{\mathfrak{C}_0}
%\left(\frac{1}{2}\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}
%-
%\frac{1}{2}\sym{\ten{P}_{12}\fib{\vec{R}}\tp\ten{\Sigma}\ten{P}_{12}}\right):\fib{\ten{R}}\tp\nabla\delta\vec{\mtx{\varphi}}
%\abs{C}\d s = 0.
%\end{multline}
Thus, substitution to~\eqref{eq:new:sys:matrix_condense} and integration by parts yields
\begin{equation}%\label{eq:sys:matrix_condense2}
\begin{aligned}
&\int\limits_{\mtx{\Omega}} \left(\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}}- \vec{B}_{ext}\cdot\delta\vec{\varphi}\right) \d V
-
\int\limits_{\partial\Omega_{N}} \!\!\vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d S
+
\int\limits_{\mathfrak{C}_0}\left(\mathfrak{n}\otimes\vec{D}_3 : \nabla\delta\mtx{\vec{\varphi}}
-
\bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}\right)\d s\\
&
+
\int\limits_{\mathfrak{C}_0}
\left[\ten{\mathcal{P}}_{\alpha}\mathfrak{m}\otimes\vec{D}_\alpha\otimes\vec{D}_3\right]\,\vdots\,\nabla^2\delta\mtx{\vec{\varphi}}
\d s
+ \int\limits_{\mathfrak{C}_0}
\biggl[\ten{\mathcal{P}}_{\alpha}^\prime\mathfrak{m}
-\ten{\mathcal{P}}_{\alpha}\left(\tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}} +\bar{\tilde{\vec{m}}}\right)
\biggl]\otimes\vec{D}_{\alpha}:\nabla\delta\mtx{\vec{\varphi}}\,\d s
\\
&
+ \int\limits_{\mathfrak{C}_0}
\ten{\mathcal{Q}}_{\alpha}\tilde{\vec{\mu}}_n\otimes\vec{D}_{\alpha}:\nabla\delta\vec{\mtx{\varphi}} \abs{C}\d s
+
 \sum_{s=0,L}
\ten{\mathcal{Q}}_{\alpha}\tilde{\vec{\mu}}_n^s\otimes\vec{D}_{\alpha}: \nabla\delta\mtx{\vec{\varphi}}_s\,\abs{A}
= 0,
\end{aligned}
\end{equation}
%Let us note that for all~$\vec{v}$ it holds
%\begin{equation}\label{key}
%\begin{aligned}
%\left(\ten{\Id}-\frac{1}{2}\fib{\ten{R}}\ten{P}_{12}\fib{\ten{R}}\tp\right) & \VPTen{\vec{v}}\fib{\ten{R}}\ten{P}_{12} \\
%&=
%\left(\frac{1}{2}\fib{\ten{R}}\ten{P}_{12}\fib{\ten{R}}\tp + \vec{d}_3\otimes\vec{d}_3\right)\VPTen{\vec{d}_{\alpha}}\tp\vec{v}\otimes\vec{D}_{\alpha}
%\\
%&=
%\underbrace{\left(\frac{1}{2}\vec{d}_2\otimes\vec{d}_3 - \vec{d}_3\otimes\vec{d}_2\right)}_{\ten{\mathcal{P}}_1}\vec{v}\otimes\vec{D}_1
%+
%\underbrace{\left(-\frac{1}{2}\vec{d}_1\otimes\vec{d}_3 + \vec{d}_3\otimes\vec{d}_1\right)}_{\ten{\mathcal{P}}_2}\vec{v}\otimes\vec{D}_2
%\\
%&=
%(\vec{v}\cdot\vec{d}_1)\vec{d}_3\otimes\vec{D}_2  - (\vec{v}\cdot\vec{d}_2)\vec{d}_3\otimes\vec{D}_1 + (\vec{v}\cdot\vec{d}_3)\frac{\vec{d}_2\otimes\vec{D}_1-\vec{d}_1\otimes\vec{D}_2}{2}
%\end{aligned}
%\end{equation}
%Besides, according to~\eqref{eq:new:LM_matrix}, we have
%\begin{equation}\label{key}
%\begin{aligned}
%\fib{\ten{R}}\ten{P}_{12} & \sym{\fib{\vec{R}}\tp\ten{\Sigma}}\ten{P}_{12}
%\\
%&=
%\tilde{\mu}_n\left(\vec{d}_1\otimes\vec{D}_1+\vec{d}_2\otimes\vec{D}_2\right)
%+
%\tilde{\mu}_{s,1}\left(\vec{d}_1\otimes\vec{D}_1-\vec{d}_2\otimes\vec{D}_2\right)
%+
%\tilde{\mu}_{s,2}\left(\vec{d}_2\otimes\vec{D}_1+\vec{d}_1\otimes\vec{D}_2\right)
%\\
%&=
%\underbrace{\left(\vec{d}_1\otimes\vec{d}_1 + \vec{d}_1\otimes\vec{d}_2 + \vec{d}_2\otimes\vec{d}_3\right)}_{\ten{\mathcal{Q}}_1}\tilde{\vec{\mu}}^{sym}\otimes\vec{D}_1
%\\
%&+
%\underbrace{\left(\vec{d}_2\otimes\vec{d}_1 - \vec{d}_2\otimes\vec{d}_2 + \vec{d}_1\otimes\vec{d}_3\right)}_{\ten{\mathcal{Q}}_2}\tilde{\vec{\mu}}^{sym}\otimes\vec{D}_2,
%%&=
%%(\tilde{\vec{\mu}}^{sym}\cdot\vec{d}_1)\vec{d}_1\otimes\vec{D}_1
%%+
%%(\tilde{\vec{\mu}}^{sym}\cdot\vec{d}_2\vec{d}_2\otimes\vec{D}_2
%%+
%%(\tilde{\vec{\mu}}^{sym}\cdot\vec{d}_3)\frac{\vec{d}_2\otimes\vec{D}_1+\vec{d}_1\otimes\vec{D}_2}{2}
%%\\
%%&=
%%\underbrace{\left(\vec{d}_1\otimes\vec{d}_1 + \frac{1}{2}\vec{d}_2\otimes\vec{d}_3\right)}_{\ten{\mathcal{Q}}_1}\tilde{\vec{\mu}}^{sym}\otimes\vec{D}_1
%%+
%%\underbrace{\left(\vec{d}_2\otimes\vec{d}_2 + \frac{1}{2}\vec{d}_1\otimes\vec{d}_3\right)}_{\ten{\mathcal{Q}}_2}\tilde{\vec{\mu}}^{sym}\otimes\vec{D}_2,
%\end{aligned}
%\end{equation}
%where $
%\tilde{\vec{\mu}}^{sym} = \tilde{\mu}_n\vec{d}_1 + \tilde{\mu}_{s,1}\vec{d}_2 + \tilde{\mu}_{s,2}\vec{d}_3
%$.
%%and
%%\begin{equation}\label{key}
%%	\sym{\fib{\vec{R}}\tp\ten{\Sigma}} = \begin{bmatrix}
%%	\tilde{\mu}^{sym}_1 & \tilde{\mu}^{sym}_3\\
%%	\tilde{\mu}^{sym}_3 & \tilde{\mu}^{sym}_2
%%	\end{bmatrix}.
%%\end{equation}
%Then, we obtain after integration by parts and some tedious, but straight forward manipulations
%\begin{equation}\label{eq:new:sys:matrix_condense3}
%\begin{aligned}
%\int\limits_{\mtx{\Omega}} &\left(\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}}- \vec{B}_{ext}\cdot\delta\vec{\varphi}\right) \d V 
%-
%\int\limits_{\partial\Omega_{N}} \!\!\vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d S
%+
%\int\limits_{\mathfrak{C}_0}\left(\mathfrak{n}\otimes\vec{D}_3 : \nabla\delta\mtx{\vec{\varphi}}
%-
%\bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}\right)\d s  \\
%&
%+
%\int\limits_{\mathfrak{C}_0}
%\left[\ten{\mathcal{P}}_{\alpha}\mathfrak{m}\otimes\vec{D}_\alpha\otimes\vec{D}_3\right]\,\vdots\,\nabla^2\delta\mtx{\vec{\varphi}}
%\d s
%+ \int\limits_{\mathfrak{C}_0}
%\biggl[\ten{\mathcal{P}}_{\alpha}^\prime\mathfrak{m}
%-\ten{\mathcal{P}}_{\alpha}\left(\tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}} +\bar{\tilde{\vec{m}}}\right)
%\biggl]\otimes\vec{D}_{\alpha}:\nabla\delta\mtx{\vec{\varphi}}\,\d s
%\\
%&
%+ \frac{1}{2}\,\int\limits_{\mathfrak{C}_0}
%\ten{\mathcal{Q}}_{\alpha}\tilde{\vec{\mu}}^{sym}\otimes\vec{D}_{\alpha}:\nabla\delta\vec{\mtx{\varphi}} \abs{C}\d s
%+
%\frac{1}{2} \sum_{s=0,L}
%\ten{\mathcal{Q}}_{\alpha}\tilde{\vec{\mu}}^{sym}_s\otimes\vec{D}_{\alpha}: \nabla\delta\mtx{\vec{\varphi}}_s\,\abs{A}
%= 0,
%\end{aligned}.
%\end{equation}
Let us now introduce $\vec{\eta}(s)$ satisfying
\begin{align}\label{key}
	\vec{\eta}^\prime + \tilde{\vec{\mu}}_n &= 0, \\
	\vec{\eta}(0) =\tilde{\vec{\mu}}_n^0, \quad & \vec{\eta}(L) = \tilde{\vec{\mu}}_n^L.
\end{align}
\rev{Why is it possible ?}

Eventually, the final condensed system writes:
\begin{equation}\label{eq:new:sys:matrix_very_condense}
\begin{aligned}
\int\limits_{\mtx{\Omega}} &\left(\drv{\mtx{\Psi}}{\ten{\mtx{F}}}:\nabla\delta\vec{\mtx{\varphi}}- \vec{B}_{ext}\cdot\delta\vec{\varphi}\right) \d V 
-
\int\limits_{\partial\Omega_{N}} \!\!\vec{T}_{ext}\cdot\delta\vec{\mtx{\varphi}} \d S
+
\int\limits_{\mathfrak{C}_0}\left(\mathfrak{n}\otimes\vec{D}_3 : \nabla\delta\mtx{\vec{\varphi}}
-
\bar{\tilde{\vec{n}}} \cdot \delta\mtx{\vec{\varphi}}\right)\d s  \\
&
+
\int\limits_{\mathfrak{C}_0}
\left[\left(\ten{\mathcal{P}}_{\alpha}\mathfrak{m}+\ten{\mathcal{Q}}_{\alpha}\vec{\eta}\right)\otimes\vec{D}_\alpha\otimes\vec{D}_3\right]\,\vdots\,\nabla^2\delta\mtx{\vec{\varphi}}
\d s
\\
&+
\int\limits_{\mathfrak{C}_0}
\biggl[\ten{\mathcal{P}}_{\alpha}^\prime\mathfrak{m}
+ \ten{\mathcal{Q}}_{\alpha}^\prime\vec{\eta}
-\ten{\mathcal{P}}_{\alpha}\left(\tilde{\vec{\varphi}}^{\prime}\times{\mathfrak{n}} +\bar{\tilde{\vec{m}}}\right)
\biggl]\otimes\vec{D}_{\alpha}:\nabla\delta\mtx{\vec{\varphi}}\,\d s
= 0,
\end{aligned}.
\end{equation}
supplemented with constitutive equations~\eqref{eq:new:constitutive_n}-\eqref{eq:new:constitutive_m} and coupling constraints
\begin{align}\label{key}
\int\limits_{\mathfrak{C}_0}
\big(\vec{F}_{c}\vec{D}_{1}-\vec{d}_{1}\big)\cdot\delta\tilde{\vec{\mu}}_1\d s &= 0,\\
\int\limits_{\mathfrak{C}_0}
\big(\vec{F}_{c}\vec{D}_{2}-\vec{d}_{2}\big)\cdot\delta\tilde{\vec{\mu}}_2\d s &= 0.
\end{align}

Here, we now obtain an explicit representation for the third order stress tensor introduced in \eqref{eq:secondGradient} as
\begin{equation}
\mathfrak{P} = \left(\ten{\mathcal{P}}_{\alpha}\mathfrak{m}+\ten{\mathcal{Q}}_{\alpha}\vec{\eta}\right)\otimes\vec{D}_\alpha\otimes\vec{D}_3 \; \delta_{\fib{\vec{\varphi}}_0(\mathfrak{C}_0)}(\X),
\end{equation}
which emanates from the condensation of the moment equation of the beams. Note that this term directly depends on the resultant contact torque, derived from, e.g. \eqref{eq:simpleMat}, which is written in terms of the second and the polar moment of area, respectively.
Above, $\delta_{\fib{\vec{\varphi}}_0(\mathfrak{C}_0)}(\X)$ stands for the line Dirac delta function on~$\fib{\vec{\varphi}}_0(\mathfrak{C}_0)$.

\rev{Why we have a special notation for $[0,L]$ and nothing for $\fib{\vec{\varphi}}_0([0,L])$ ? }
